Milestones in Autonomous Driving and Intelligent Vehicles: Survey of Surveys

Interest in autonomous driving (AD) and intelligent vehicles (IVs) is growing at a rapid pace due to the convenience, safety, and economic benefits. Although a number of surveys have reviewed research achievements in this field, they are still limited in specific tasks, lack of systematic summary and research directions in the future. Here we propose a Survey of Surveys (SoS) for total technologies of AD and IVs that reviews the history, summarizes the milestones, and provides the perspectives, ethics, and future research directions. To our knowledge, this article is the first SoS with milestones in AD and IVs, which constitutes our complete research work together with two other technical surveys. We anticipate that this article will bring novel and diverse insights to researchers and abecedarians, and serve as a bridge between past and future.

==> body/bib.tex <==


\small\bibliographystyle{IEEEtran}
%\biboptions{sort&compress}
\bibliography{body/mylib.bib}

==> body/bib_old.tex <==
%\begin{thebibliography}{1}

\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,mylib}

%%%survey%%%
publisher={IEEE}
@article{survey_1,
  title={Survey on artificial intelligence for vehicles},
  author={Li, Jun and Cheng, Hong and Guo, Hongliang and Qiu, Shaobo},
  journal={Automotive Innovation},
  volume={1},
  number={1},
  pages={2--14},
  year={2018},
  publisher={Springer}
}

\bibitem{survey_Deep_Multi-modal}
Feng, D., Haase-Schütz, C., Rosenbaum, L., Hertlein, H., Glaeser, C., Timm, F., ... & Dietmayer, K. (2020). Deep multi-modal object detection and semantic segmentation for autonomous driving: Datasets, methods, and challenges. IEEE Transactions on Intelligent Transportation Systems, 22(3), 1341-1360.

%%%dataset%%%
\bibitem{dataset_KITTI}
Geiger, A., Lenz, P., & Urtasun, R. (2012, June). Are we ready for autonomous driving? the kitti vision benchmark suite. In 2012 IEEE conference on computer vision and pattern recognition (pp. 3354-3361). IEEE.

\bibitem{dataset_seg_ADE20K}
Zhou, B., Zhao, H., Puig, X., Xiao, T., Fidler, S., Barriuso, A., & Torralba, A. (2019). Semantic understanding of scenes through the ade20k dataset. International Journal of Computer Vision, 127(3), 302-321.

\bibitem{dataset_seg_VOC}
Everingham, M., Van Gool, L., Williams, C. K., Winn, J., & Zisserman, A. (2010). The pascal visual object classes (voc) challenge. International journal of computer vision, 88(2), 303-338.

\bibitem{dataset_seg_CityScape}
Zhou, B., Zhao, H., Puig, X., Xiao, T., Fidler, S., Barriuso, A., & Torralba, A. (2019). Semantic understanding of scenes through the ade20k dataset. International Journal of Computer Vision, 127(3), 302-321.

\bibitem{dataset_seg_Mapillary_Vistas}
Neuhold, G., Ollmann, T., Rota Bulo, S., & Kontschieder, P. (2017). The mapillary vistas dataset for semantic understanding of street scenes. In Proceedings of the IEEE international conference on computer vision (pp. 4990-4999).

\bibitem{dataset_NYUv2}
Silberman, N., Hoiem, D., Kohli, P., & Fergus, R. (2012, October). Indoor segmentation and support inference from rgbd images. In European conference on computer vision (pp. 746-760). Springer, Berlin, Heidelberg.

%%%localization%%%
\bibitem{loca_1}
Kuutti S ,  Fallah S ,  Katsaros K , et al. A Survey of the State-of-the-Art Localization Techniques and Their Potentials for Autonomous Vehicle Applications[J]. IEEE Internet of Things Journal, 2018:829-846.

\bibitem{loca_2}
Liang L ,  Ming Y ,  Bing W , et al. An overview on sensor map based localization for automated driving[C]// Urban Remote Sensing Event. IEEE, 2017.

\bibitem{loca_3}
Wang Y ,  Zhang W . A Survey of Simultaneous Localization and Mapping on Unstructured Lunar Complex Environment[J]. Journal of Zhengzhou University(Engineering Science), 2018.

\bibitem{loca_4}
Luo Q , Y Cao, Liu J , et al. Localization and Navigation in Autonomous Driving: Threats and Countermeasures[J]. IEEE Wireless Communications, 2019, 26(4):38-45.

\bibitem{loca_5}
Debeunne C ,  Vivet D . A Review of Visual-LiDAR Fusion based Simultaneous Localization and Mapping[J]. Sensors, 2020, 20(7):2068.

\bibitem{loca_6}
Singandhupe A ,  La H M . A Review of SLAM Techniques and Security in Autonomous Driving[C] 2019 Third IEEE International Conference on Robotic Computing (IRC). IEEE, 2019.

\bibitem{loca_7}
Takleh T ,  Bakar N A ,  Rahman S A , et al. A Brief Survey on SLAM Methods in Autonomous Vehicle[J]. International Journal of Engineering & Technology, 2018, 7(4):38-43.

\bibitem{loca_8}
Gao B ,  Lang H ,  Ren J . Stereo Visual SLAM for Autonomous Vehicles: A Review[C]// 2020 IEEE International Conference on Systems, Man, and Cybernetics (SMC). IEEE, 2020.

\bibitem{loca_9}
Wong K ,  Gu Y ,  Kamijo S . Mapping for Autonomous Driving: Opportunities and Challenges[J]. IEEE Intelligent Transportation Systems Magazine, 2020, PP(99).

\bibitem{loca_10}
Jonnavithula N ,  Lyu Y ,  Zhang Z . LiDAR Odometry Methodologies for Autonomous Driving: A Survey[J].  2021.

\bibitem{loca_11}
Guo H ,  D  Cao,  Hong C , et al. Vehicle dynamic state estimation: state of the art schemes and perspectives[J]. IEEE/CAA Journal of Automatica Sinica, 2018, 5(002):418-431.

\bibitem{loca_12}
Chehri A ,  Quadar N ,  Saadane R . Survey on localization methods for autonomous vehicles in smart cities[C]// the 4th International Conference. 2019.

\bibitem{loca_14}
Leurent E . A Survey of State-Action Representations for Autonomous Driving. 

\bibitem{loca_15}
Chen S ,  Liu B ,  Feng C , et al. 3D Point Cloud Processing and Learning for Autonomous Driving: Impacting Map Creation, Localization, and Perception[J]. IEEE Signal Processing Magazine, 2021, 38(1):68-86.

\bibitem{loca_16}
G. Bresson, Z. Alsayed, L. Yu and S. Glaser,” Simultaneous Localization and Mapping: A Survey of Current Trends in Autonomous Driving,” IEEE Transactions on Intelligent Vehicles,pp. 194-220, 2017.

\bibitem{loca_17}C. Gentner, T. Jost, W. Wang, S. Zhang, A. Dammann and U.C.Fiebig,” Multipath Assisted Positioning with Simultaneous Localization and Mapping,” IEEE Transactions on Wireless Communications, pp. 1536-1276, 2016.

\bibitem{loca_18}
K.-H. Jo and J. Lee, "Multi-robot cooperative localization with optimally fused information of odometer and gps," in International Conference on Control, Automation and Systems 2007, 2007.

\bibitem{loca_19}
C. Cadena, L. Carlone, H. Carrillo, Y. Latif, D. Scaramuzza, J. Neira,I. Reid, and J. J. Leonard. Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age. IEEETrans. on Robotics, 32(6):1309–1332, Dec 2016.

\bibitem{loca_20}
Frank Steinbrücker, Jürgen Sturm, and Daniel Cremers. Real-time visual odometry from dense rgb-d images. In 2011 IEEE International Conference on Computer Vision Workshops (ICCV Workshops), pages719–722. IEEE, 2011.

\bibitem{loca_21}
Christian Kerl, Jürgen Sturm, and Daniel Cremers. Robust odometry estimation for rgb-d cameras. In 2013 IEEE International Conferenceon Robotics and Automation, pages 3748–3754. IEEE, 2013.

\bibitem{loca_22}
Newcombe, R.A.; Lovegrove, S.J.; Davison, A.J. DTAM: Dense tracking and mapping in real-time.In Proceedings of the 2011 International Conference on Computer Vision, Barcelona, Spain, 6–13 November 2011; pp. 2320–2327.

\bibitem{loca_23}
Engel, J.; Schöps, T.; Cremers, D. LSD-SLAM: Large-scale direct monocular SLAM. In Proceedings of theEuropean Conference on Computer Vision, Zurich, Switzerland, 6–12 September 2014; pp. 834–849.

\bibitem{loca_24}
Forster, C.; Pizzoli, M.; Scaramuzza, D. SVO: Fast semi-direct monocular visual odometry. In Proceedings of the 2014 IEEE International Conference on Robotics and Automation (ICRA), Hong Kong, China,31 May–7 June 2014; pp. 15–22.

\bibitem{loca_25}
Engel, J.; Koltun, V.; Cremers, D. Direct sparse odometry. IEEE Trans. Pattern Anal. Mach. Intell. 2017,40, 611–625. [CrossRef]

\bibitem{loca_26}
Wang, R.; Schworer, M.; Cremers, D. Stereo DSO: Large-scale direct sparse visual odometry withstereo cameras. In Proceedings of the IEEE International Conference on Computer Vision, Venice, Italy,22–29 October 2017; pp. 3903–3911.

\bibitem{loca_27}
E. Eade and T. Drummond, “Scalable Monocular SLAM,” in IEEE Computer Society Conference on Computer Vision and Pattern Recognition, vol. 1, 2006, pp. 469–476.

\bibitem{loca_28}
D. Chetverikov, D. Svirko, D. Stepanov, and P. Krsek, “The trimmed iterative closest point algorithm,” in Object recognition supported by user interaction for service robots, vol. 3. IEEE, 2002, pp. 545–548.

\bibitem{loca_29}
A. Segal, D. Haehnel, and S. Thrun, “Generalized-icp.” in Robotics: science and systems, vol. 2, no. 4. Seattle, WA, 2009, p. 435. 

\bibitem{loca_30}
S. Bouaziz, A. Tagliasacchi, and M. Pauly, “Sparse iterative closest point,” in Computer graphics forum, vol. 32, no. 5. Wiley Online Library, 2013, pp. 113–123. 

\bibitem{loca_31}
A. L. Pavlov, G. W. Ovchinnikov, D. Y. Derbyshev, D. Tsetserukou, and I. V. Oseledets, “Aa-icp: Iterative closest point with anderson acceleration,” in 2018 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2018, pp. 3407–3412. 

\bibitem{loca_32}
S. A. Parkison, L. Gan, M. G. Jadidi, and R. M. Eustice, “Semantic iterative closest point through expectation-maximization.” in BMVC, 2018, p. 280.

\bibitem{loca_33}
C. Choy, W. Dong, and V. Koltun, “Deep global registration,” in Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 2020, pp. 2514–2523.

\bibitem{loca_34}
X. Chen, A. Milioto, E. Palazzolo, P. Giguere, J. Behley, and C. Stachniss, “Suma++: Efficient lidar-based semantic slam,” in 2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). IEEE, 2019, pp. 4530–4537.

\bibitem{loca_35}
X. Zheng and J. Zhu, “Efficient lidar odometry for autonomous driving,” arXiv preprint arXiv:2104.10879, 2021.

\bibitem{loca_36}
J. Zhang and S. Singh, “Loam: Lidar odometry and mapping in realtime.” in Robotics: Science and Systems, vol. 2, no. 9, 2014.

\bibitem{loca_37}
T. Shan and B. Englot, “Lego-loam: Lightweight and groundoptimized lidar odometry and mapping on variable terrain,” in 2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). IEEE, 2018, pp. 4758–4765

\bibitem{loca_38}
Q. M. Thomas, O. Wasenmuller, and D. Stricker, “Delio: Decoupled ¨ lidar odometry,” in 2019 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2019, pp. 1549–1556.

\bibitem{loca_39}
S. Lee, C. Kim, S. Cho, S. Myoungho, and K. Jo, “Robust 3- dimension point cloud mapping in dynamic environment using pointwise static probability-based ndt scan-matching,” IEEE Access, vol. 8, pp. 175 563–175 575, 2020.

\bibitem{loca_40}
Shan T ,  Englot B ,  Ratti C , et al. LVI-SAM: Tightly-coupled Lidar-Visual-Inertial Odometry via Smoothing and Mapping[J].  2021.

\bibitem{loca_41}
Lin J ,  Zheng C ,  Xu W , et al. R2LIVE: A Robust, Real-time, LiDAR-Inertial-Visual tightly-coupled state Estimator and mapping[J].  2021.

\bibitem{loca_42}
Tong, Qin, Peiliang, et al. VINS-Mono: A Robust and Versatile Monocular Visual-Inertial State Estimator[J]. IEEE Transactions on Robotics, 2018.

\bibitem{loca_43}
Hao L ,  Li H ,  Zhang Q , et al. LMVI-SLAM: Robust Low-Light Monocular Visual-Inertial Simultaneous Localization and Mapping[C]// 2019 IEEE International Conference on Robotics and Biomimetics (ROBIO). IEEE, 2019.

\bibitem{loca_44}
Zuo X ,  Geneva P ,  Lee W , et al. LIC-Fusion: LiDAR-Inertial-Camera Odometry[J]. IROS, 2019.

\bibitem{loca_45}
S. W. Chen, G. V. Nardari, E. S. Lee, C. Qu, X. Liu, R. A. F. Romero, and V. Kumar, “Sloam: Semantic lidar odometry and mapping for forest inventory,” IEEE Robotics and Automation Letters, vol. 5, no. 2, pp. 612–619, 2020.

\bibitem{loca_46}
Elhousni M ,  Huang X . A Survey on 3D LiDAR Localization for Autonomous Vehicles[C]// 2020 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2020.

\bibitem{loca_47}
C. Cadena, L. Carlone, H. Carillo, Y. Latif, D. Scaramuzza, J.Neira, I. Reid and J. J. Leonard,” Past, Present and Future of Samultaneous Localization and Mapping: Toward the Robust Perception Age,” IEEE Transactions on Robotics, pp. 1309-1332, 2016. 

\bibitem{loca_48}
X. Xie, Y. Yu, X. Lin and C. Sun,” An EKF SLAM Algorithm for Mobile Robot with Sensor Bias Estimation,” 32nd Youth Academic Annual Conference of Chinese Association of Automation (YAC),pp. 281-285, 2017. 

\bibitem{loca_49}
S. Thrun and J. J. Leonard, “Simultaneous localization and mapping,” in Springer Handbook of Robotics. New York, NY, USA: Springer -Verlag, 2008, pp. 871 –889.

\bibitem{loca_50}
Sun F, Zhou Y, Li C, et al. Research on active SLAM with fusion of monocular vision and laser range data[C]. Jinan: In IEEE World Congress on Intelligent Control and Automation, 2010: 6550–6554.

\bibitem{loca_51}
Arandjelovic R, Gronat P, Torll A, et al. NetVLAD: CNN architecture for weakly supervised place recognition[C]. New York: In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, 2016: 5297-5307

\bibitem{loca_52}
én M, García S, Barea R, et al. A Multi-Sensorial Simultaneous Localization and Mapping (SLAM) System for Low-Cost Micro Aerial Vehicles in GPS-Denied Environments[J]. Sensors, 2017, 17(4): 802-829

\bibitem{loca_53}
Graeter J, Wilczynski A, Lauer M. Limo: Lidar-monocular visual odometry[C]. In IEEE/RSJ International Conference on Intelligent Robots and Systems. Madrid, Spain, 2018: 7872–7879

\bibitem{loca_54}
Shin Y S, Park Y S, Kim A. Direct visual SLAM using sparse depth for camera-lidar system[C]. Australia: In IEEE International Conference on Robotics and Automation Brisbane, 2018: 1–8.

\bibitem{loca_55}
De Silva V, Roche J, Kondoz A. Fusion of LiDAR and camera sensor data for environment sensing in driverless vehicles[J]. arXiv2018, arXiv: 1710.06230.

\bibitem{loca_56}
M. Magnusson, ‘‘The three-dimensional normal-distributions transform—An efficient representation for registration, surface analysis, and loop detection,’’ Ph.D. dissertation, Graduate School Robot. Automat. Process Control, Örebro Univ., Örebro, Sweden, 2009

\bibitem{loca_57}
M. Magnusson, A. Nuchter, C. Lorken, A. J. Lilienthal, and J. Hertzberg,‘‘Evaluation of 3D registration reliability and speed—A comparison of ICP and NDT,’’ in Proc. IEEE Int. Conf. Robot. Autom., May 2009,pp. 3907–3912.

\bibitem{loca_58}
‘‘A 3-D scan matching using improved 3-D normal distributions transform for mobile robotic mapping,’’ in Proc. IEEE/RSJ Int. Conf. Intell. Robots Syst., Oct. 2006, pp. 3068–3073.

%%%perception_scene%%%

\bibitem{scene_FCN}
Long, J., Shelhamer, E., & Darrell, T. (2015). Fully convolutional networks for semantic segmentation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 3431-3440).

\bibitem{scene_segnet}
Badrinarayanan, V., Kendall, A., & Cipolla, R. (2017). Segnet: A deep convolutional encoder-decoder architecture for image segmentation. IEEE transactions on pattern analysis and machine intelligence, 39(12), 2481-2495.

\bibitem{scene_dilated}
Yu, F., & Koltun, V. (2015). Multi-scale context aggregation by dilated convolutions. arXiv preprint arXiv:1511.07122.

\bibitem{scene_DeepLabv1}
Chen, L. C., Papandreou, G., Kokkinos, I., Murphy, K., & Yuille, A. L. (2014). Semantic image segmentation with deep convolutional nets and fully connected crfs. arXiv preprint arXiv:1412.7062.

\bibitem{scene_DeepLabv2}
Chen, L. C., Papandreou, G., Kokkinos, I., Murphy, K., & Yuille, A. L. (2017). Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs. IEEE transactions on pattern analysis and machine intelligence, 40(4), 834-848.

\bibitem{scene_RefineNet}
Lin, G., Milan, A., Shen, C., & Reid, I. (2017). Refinenet: Multi-path refinement networks for high-resolution semantic segmentation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 1925-1934).

\bibitem{scene_PSP}
Zhao, H., Shi, J., Qi, X., Wang, X., & Jia, J. (2017). Pyramid scene parsing network. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 2881-2890).

\bibitem{scene_DeepLabv3}
Chen, L. C., Papandreou, G., Schroff, F., & Adam, H. (2017). Rethinking atrous convolution for semantic image segmentation. arXiv preprint arXiv:1706.05587.

\bibitem{scene_Unet}
Ronneberger, O., Fischer, P., & Brox, T. (2015, October). U-net: Convolutional networks for biomedical image segmentation. In International Conference on Medical image computing and computer-assisted intervention (pp. 234-241). Springer, Cham.

\bibitem{scene_Unet}
Ronneberger, O., Fischer, P., & Brox, T. (2015, October). U-net: Convolutional networks for biomedical image segmentation. In International Conference on Medical image computing and computer-assisted intervention (pp. 234-241). Springer, Cham.

\bibitem{scene_Unet++}
Zhou, Z., Rahman Siddiquee, M. M., Tajbakhsh, N., & Liang, J. (2018). Unet++: A nested u-net architecture for medical image segmentation. In Deep learning in medical image analysis and multimodal learning for clinical decision support (pp. 3-11). Springer, Cham.

\bibitem{scene_OCRNet}
Yuan, Y., Chen, X., & Wang, J. (2020, August). Object-contextual representations for semantic segmentation. In European conference on computer vision (pp. 173-190). Springer, Cham.

\bibitem{scene_OCNet}
Yuan, Y., Huang, L., Guo, J., Zhang, C., Chen, X., & Wang, J. (2018). Ocnet: Object context network for scene parsing. arXiv preprint arXiv:1809.00916.

\bibitem{scene_multi_scale_attention}
Tao, A., Sapra, K., & Catanzaro, B. (2020). Hierarchical multi-scale attention for semantic segmentation. arXiv preprint arXiv:2005.10821.

\bibitem{scene_boundary_aware_segmentation}
Borse, S., Wang, Y., Zhang, Y., & Porikli, F. (2021). Inverseform: A loss function for structured boundary-aware segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 5901-5911).

\bibitem{scene_intrinsic_relevance}
Cai, Y., Dai, L., Wang, H., & Li, Z. (2021). Multi-target pan-class intrinsic relevance driven model for improving semantic segmentation in autonomous driving. IEEE Transactions on Image Processing, 30, 9069-9084.

\bibitem{scene_Naive_student}
Chen, L. C., Lopes, R. G., Cheng, B., Collins, M. D., Cubuk, E. D., Zoph, B., ... & Shlens, J. (2020, August). Naive-student: Leveraging semi-supervised learning in video sequences for urban scene segmentation. In European Conference on Computer Vision (pp. 695-714). Springer, Cham.

\bibitem{scene_unsupervised_domain}
Erkent, Ö., & Laugier, C. (2020). Semantic segmentation with unsupervised domain adaptation under varying weather conditions for autonomous vehicles. IEEE Robotics and Automation Letters, 5(2), 3580-3587.

\bibitem{scene_Warp_Refine_Propagation}
Ganeshan, A., Vallet, A., Kudo, Y., Maeda, S. I., Kerola, T., Ambrus, R., ... & Gaidon, A. (2021). Warp-Refine Propagation: Semi-Supervised Auto-labeling via Cycle-consistency. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 15499-15509).

\bibitem{scene_Mask_RCNN}
He, K., Gkioxari, G., Dollár, P., & Girshick, R. (2017). Mask r-cnn. In Proceedings of the IEEE international conference on computer vision (pp. 2961-2969).

\bibitem{scene_HTC}
Chen, K., Pang, J., Wang, J., Xiong, Y., Li, X., Sun, S., ... & Lin, D. (2019). Hybrid task cascade for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 4974-4983).

\bibitem{scene_Explicit}
Xu, W., Wang, H., Qi, F., & Lu, C. (2019). Explicit shape encoding for real-time instance segmentation. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 5168-5177).

\bibitem{scene_Yolact}
Bolya, D., Zhou, C., Xiao, F., & Lee, Y. J. (2019). Yolact: Real-time instance segmentation. In Proceedings of the IEEE/CVF international conference on computer vision (pp. 9157-9166).

\bibitem{scene_Blendmask}
Chen, H., Sun, K., Tian, Z., Shen, C., Huang, Y., & Yan, Y. (2020). Blendmask: Top-down meets bottom-up for instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 8573-8581).

\bibitem{scene_Centermask}
Lee, Y., & Park, J. (2020). Centermask: Real-time anchor-free instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 13906-13915).

\bibitem{scene_Embedmask}
Ying, H., Huang, Z., Liu, S., Shao, T., & Zhou, K. (2019). Embedmask: Embedding coupling for one-stage instance segmentation. arXiv preprint arXiv:1912.01954.

\bibitem{scene_Mask_encoding}
Zhang, R., Tian, Z., Shen, C., You, M., & Yan, Y. (2020). Mask encoding for single shot instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 10226-10235).

\bibitem{scene_Conditional}
Tian, Z., Shen, C., & Chen, H. (2020, August). Conditional convolutions for instance segmentation. In European conference on computer vision (pp. 282-298). Springer, Cham.

\bibitem{scene_Solov2}
Wang, X., Zhang, R., Kong, T., Li, L., & Shen, C. (2020). Solov2: Dynamic and fast instance segmentation. Advances in Neural information processing systems, 33, 17721-17732.

\bibitem{scene_Ssap}
Gao, N., Shan, Y., Wang, Y., Zhao, X., Yu, Y., Yang, M., & Huang, K. (2019). Ssap: Single-shot instance segmentation with affinity pyramid. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 642-651).

\bibitem{scene_Polytransform}
Liang, J., Homayounfar, N., Ma, W. C., Xiong, Y., Hu, R., & Urtasun, R. (2020). Polytransform: Deep polygon transformer for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 9131-9140).

\bibitem{scene_Look_closer_to_segment_better}
Tang, C., Chen, H., Li, X., Li, J., Zhang, Z., & Hu, X. (2021). Look closer to segment better: Boundary patch refinement for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 13926-13935).

\bibitem{scene_Scaling_wide}
Chen, L. C., Wang, H., & Qiao, S. (2020). Scaling wide residual networks for panoptic segmentation. arXiv preprint arXiv:2011.11675.

\bibitem{scene_Panoptic_segmentation}
Kirillov, A., He, K., Girshick, R., Rother, C., & Dollár, P. (2019). Panoptic segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 9404-9413).

\bibitem{scene_Panoptic_segmentation_joint}
De Geus, D., Meletis, P., & Dubbelman, G. (2018). Panoptic segmentation with a joint semantic and instance segmentation network. arXiv preprint arXiv:1809.02110.

\bibitem{scene_Panoptic_FPN}
Kirillov, A., Girshick, R., He, K., & Dollár, P. (2019). Panoptic feature pyramid networks. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 6399-6408).

\bibitem{scene_AUNet}
Li, Y., Chen, X., Zhu, Z., Xie, L., Huang, G., Du, D., & Wang, X. (2019). Attention-guided unified network for panoptic segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 7026-7035).

\bibitem{scene_UPNet}
Xiong, Y., Liao, R., Zhao, H., Hu, R., Bai, M., Yumer, E., & Urtasun, R. (2019). Upsnet: A unified panoptic segmentation network. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 8818-8826).

\bibitem{scene_Panoptic_FCN}
Li, Y., Zhao, H., Qi, X., Wang, L., Li, Z., Sun, J., & Jia, J. (2021). Fully convolutional networks for panoptic segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 214-223).

\bibitem{scene_Panoptic_SegFormer}
Li, Z., Wang, W., Xie, E., Yu, Z., Anandkumar, A., Alvarez, J. M., ... & Lu, T. (2022). Panoptic SegFormer: Delving deeper into panoptic segmentation with transformers. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 1280-1289).

\bibitem{scene_Improving_panoptic_segmentation}
Porzi, L., Bulo, S. R., & Kontschieder, P. (2021). Improving panoptic segmentation at all scales. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 7302-7311).

\bibitem{scene_TASC}
Li, J., Raventos, A., Bhargava, A., Tagawa, T., & Gaidon, A. (2018). Learning to fuse things and stuff. arXiv preprint arXiv:1812.01192.

\bibitem{scene_Axial_deeplab}
Wang, H., Zhu, Y., Green, B., Adam, H., Yuille, A., & Chen, L. C. (2020, August). Axial-deeplab: Stand-alone axial-attention for panoptic segmentation. In European Conference on Computer Vision (pp. 108-126). Springer, Cham.

\bibitem{scene_Depth_completion}
Uhrig, J., Schneider, N., Schneider, L., Franke, U., Brox, T., & Geiger, A. (2017, October). Sparsity invariant cnns. In 2017 international conference on 3D Vision (3DV) (pp. 11-20). IEEE.

\bibitem{scene_Sparse_and_dense_data_with_cnns}
Jaritz, M., De Charette, R., Wirbel, E., Perrotton, X., & Nashashibi, F. (2018, September). Sparse and dense data with cnns: Depth completion and semantic segmentation. In 2018 International Conference on 3D Vision (3DV) (pp. 52-60). IEEE.

\bibitem{scene_Hms_net}
Huang, Z., Fan, J., Cheng, S., Yi, S., Wang, X., & Li, H. (2019). Hms-net: Hierarchical multi-scale sparsity-invariant network for sparse depth completion. IEEE Transactions on Image Processing, 29, 3429-3441.

\bibitem{scene_Uncertainty_aware_cnns}
Eldesokey, A., Felsberg, M., Holmquist, K., & Persson, M. (2020). Uncertainty-aware cnns for depth completion: Uncertainty from beginning to end. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 12014-12023).

\bibitem{scene_Dfinenet}
Zhang, Y., Nguyen, T., Miller, I. D., Shivakumar, S. S., Chen, S., Taylor, C. J., & Kumar, V. (2019). Dfinenet: Ego-motion estimation and depth refinement from sparse, noisy depth input with rgb guidance. arXiv preprint arXiv:1903.06397.

\bibitem{scene_From_depth_what_can_you_see}
Lu, K., Barnes, N., Anwar, S., & Zheng, L. (2020). From depth what can you see? Depth completion via auxiliary image reconstruction. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 11306-11315).

\bibitem{scene_Confidence_propagation}
Eldesokey, A., Felsberg, M., & Khan, F. S. (2019). Confidence propagation through cnns for guided sparse depth regression. IEEE transactions on pattern analysis and machine intelligence, 42(10), 2423-2436.

\bibitem{scene_Uncertainty_driven_loss}
Zhu, Y., Dong, W., Li, L., Wu, J., Li, X., & Shi, G. (2021). Robust depth completion with uncertainty-driven loss functions. arXiv preprint arXiv:2112.07895.

\bibitem{scene_Depth_normal_constraints}
Xu, Y., Zhu, X., Shi, J., Zhang, G., Bao, H., & Li, H. (2019). Depth completion from sparse lidar data with depth-normal constraints. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 2811-2820).

\bibitem{scene_Self_supervised_sparse_to_dense}
Ma, F., Cavalheiro, G. V., & Karaman, S. (2019, May). Self-supervised sparse-to-dense: Self-supervised depth completion from lidar and monocular camera. In 2019 International Conference on Robotics and Automation (ICRA) (pp. 3288-3295). IEEE.

\bibitem{scene_Geometry_Aware_Embedding}
Du, W., Chen, H., Yang, H., & Zhang, Y. (2022). Depth Completion using Geometry-Aware Embedding. arXiv preprint arXiv:2203.10912.

\bibitem{scene_Joint_2d_3d}
Chen, Y., Yang, B., Liang, M., & Urtasun, R. (2019). Learning joint 2d-3d representations for depth completion. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 10023-10032).

\bibitem{scene_Adaptive_context_aware}
Zhao, S., Gong, M., Fu, H., & Tao, D. (2021). Adaptive context-aware multi-modal network for depth completion. IEEE Transactions on Image Processing, 30, 5264-5276.

\bibitem{scene_Penet}
Hu, M., Wang, S., Li, B., Ning, S., Fan, L., & Gong, X. (2021, May). Penet: Towards precise and efficient image guided depth completion. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 13656-13662). IEEE.

\bibitem{scene_Learning_guided}
Tang, J., Tian, F. P., Feng, W., Li, J., & Tan, P. (2020). Learning guided convolutional network for depth completion. IEEE Transactions on Image Processing, 30, 1116-1129.

\bibitem{scene_RigNet}
Yan, Z., Wang, K., Li, X., Zhang, Z., Xu, B., Li, J., & Yang, J. (2021). RigNet: Repetitive image guided network for depth completion. arXiv preprint arXiv:2107.13802.

\bibitem{scene_SemAttNet}
Nazir, D., Liwicki, M., Stricker, D., & Afzal, M. Z. (2022). SemAttNet: Towards Attention-based Semantic Aware Guided Depth Completion. arXiv preprint arXiv:2204.13635.

\bibitem{scene_Dynamic_spatial_propagation}
Lin, Y., Cheng, T., Zhong, Q., Zhou, W., & Yang, H. (2022). Dynamic spatial propagation network for depth completion. arXiv preprint arXiv:2202.09769.

%%% scene_depth_estimation%%%
\bibitem{scene_Deepstereo}
lynn, J., Neulander, I., Philbin, J., & Snavely, N. (2016). Deepstereo: Learning to predict new views from the world's imagery. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 5515-5524).

\bibitem{scene_NASD}
Kusupati, U., Cheng, S., Chen, R., & Su, H. (2020). Normal assisted stereo depth estimation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 2189-2199).

\bibitem{scene_Indoor_scene_structure_analysis}
Zhuo, W., Salzmann, M., He, X., & Liu, M. (2015). Indoor scene structure analysis for single image depth estimation. In Proceedings of the IEEE Conference on Computer Vision and Pattern recognition (pp. 614-622).

\bibitem{scene_Depth_map_prediction}
Eigen, D., Puhrsch, C., & Fergus, R. (2014). Depth map prediction from a single image using a multi-scale deep network. Advances in neural information processing systems, 27.

\bibitem{scene_Semi_supervised_deep_learning}
Kuznietsov, Y., Stuckler, J., & Leibe, B. (2017). Semi-supervised deep learning for monocular depth map prediction. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 6647-6655).

\bibitem{scene_Unsupervised_cnn}
Garg, R., Bg, V. K., Carneiro, G., & Reid, I. (2016, October). Unsupervised cnn for single view depth estimation: Geometry to the rescue. In European conference on computer vision (pp. 740-756). Springer, Cham.

\bibitem{scene_Refinedmpl}
Vianney, J. M. U., Aich, S., & Liu, B. (2019). Refinedmpl: Refined monocular pseudolidar for 3d object detection in autonomous driving. arXiv preprint arXiv:1911.09712.

\bibitem{scene_Multi_scale_continuous_crfs}
Xu, D., Ricci, E., Ouyang, W., Wang, X., & Sebe, N. (2017). Multi-scale continuous crfs as sequential deep networks for monocular depth estimation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 5354-5362).

\bibitem{scene_Pad_Net}
Xu, D., Ouyang, W., Wang, X., & Sebe, N. (2018). Pad-net: Multi-tasks guided prediction-and-distillation network for simultaneous depth estimation and scene parsing. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 675-684).

\bibitem{scene_Transformer_based_attention}
Yang, G., Tang, H., Ding, M., Sebe, N., & Ricci, E. (2021). Transformer-based attention networks for continuous pixel-wise prediction. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 16269-16279).

\bibitem{scene_P3Depth}
Patil, V., Sakaridis, C., Liniger, A., & Van Gool, L. (2022). P3Depth: Monocular Depth Estimation with a Piecewise Planarity Prior. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 1610-1621).

\bibitem{scene_DORN}
Fu, H., Gong, M., Wang, C., Batmanghelich, K., & Tao, D. (2018). Deep ordinal regression network for monocular depth estimation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 2002-2011).

\bibitem{scene_Multidepth}
Liebel, L., & Körner, M. (2019, October). Multidepth: Single-image depth estimation via multi-task regression and classification. In 2019 IEEE Intelligent Transportation Systems Conference (ITSC) (pp. 1440-1447). IEEE.

\bibitem{scene_HGR}
Zhang, Z., Xu, C., Yang, J., Tai, Y., & Chen, L. (2018). Deep hierarchical guidance and regularization learning for end-to-end depth estimation. Pattern Recognition, 83, 430-442.

\bibitem{scene_SDNet}
Ochs, M., Kretz, A., & Mester, R. (2019, September). SDNet: Semantically guided depth estimation network. In German conference on pattern recognition (pp. 288-302). Springer, Cham.

\bibitem{scene_Pattern_affinitive_propagation_across_depth}
Zhang, Z., Cui, Z., Xu, C., Yan, Y., Sebe, N., & Yang, J. (2019). Pattern-affinitive propagation across depth, surface normal and semantic segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 4106-4115).

\bibitem{scene_From_big_to_small}
Lee, J. H., Han, M. K., Ko, D. W., & Suh, I. H. (2019). From big to small: Multi-scale local planar guidance for monocular depth estimation. arXiv preprint arXiv:1907.10326.

\bibitem{scene_Enforcing_geometric_constraints}
Yin, W., Liu, Y., Shen, C., & Yan, Y. (2019). Enforcing geometric constraints of virtual normal for depth prediction. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 5684-5693).

\bibitem{scene_BANet}
Aich, S., Vianney, J. M. U., Islam, M. A., & Liu, M. K. B. (2021, May). Bidirectional attention network for monocular depth estimation. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 11746-11752). IEEE.

\bibitem{scene_3D_packing}
Guizilini, V., Ambrus, R., Pillai, S., Raventos, A., & Gaidon, A. (2020). 3d packing for self-supervised monocular depth estimation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 2485-2494).

\bibitem{scene_monodepth2}
Godard, C., Mac Aodha, O., Firman, M., & Brostow, G. J. (2019). Digging into self-supervised monocular depth estimation. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 3828-3838).

\bibitem{scene_Gcndepth}
Masoumian, A., Rashwan, H. A., Abdulwahab, S., Cristiano, J., & Puig, D. (2021). Gcndepth: Self-supervised monocular depth estimation based on graph convolutional network. arXiv preprint arXiv:2112.06782.

\bibitem{scene_Unsupervised_monocular_depth_estimation}
Godard, C., Mac Aodha, O., & Brostow, G. J. (2017). Unsupervised monocular depth estimation with left-right consistency. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 270-279).

\bibitem{scene_Self_supervised_monocular_depth_estimation}
Klingner, M., Termöhlen, J. A., Mikolajczyk, J., & Fingscheidt, T. (2020, August). Self-supervised monocular depth estimation: Solving the dynamic object problem by semantic guidance. In European Conference on Computer Vision (pp. 582-600). Springer, Cham.

\bibitem{scene_Dipe}
Jiang, H., Ding, L., Sun, Z., & Huang, R. (2020, October). Dipe: Deeper into photometric errors for unsupervised learning of depth and ego-motion from monocular videos. In 2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS) (pp. 10061-10067). IEEE.

\bibitem{scene_MLDA_Net}
Song, X., Li, W., Zhou, D., Dai, Y., Fang, J., Li, H., & Zhang, L. (2021). MLDA-Net: Multi-level dual attention-based network for self-supervised monocular depth estimation. IEEE Transactions on Image Processing, 30, 4691-4705.

\bibitem{scene_Multimodal_scale_consistency}
Chawla, H., Varma, A., Arani, E., & Zonooz, B. (2021, May). Multimodal scale consistency and awareness for monocular self-supervised depth estimation. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 5140-5146). IEEE.

\bibitem{scene_Channel_Wise_Attention_Based_Network}
Yan, J., Zhao, H., Bu, P., & Jin, Y. (2021, December). Channel-Wise Attention-Based Network for Self-Supervised Monocular Depth Estimation. In 2021 International Conference on 3D Vision (3DV) (pp. 464-473). IEEE.

\bibitem{scene_Transformers_in_Self_Supervised_Monocular_Depth_Estimation}
Varma, A., Chawla, H., Zonooz, B., & Arani, E. (2022). Transformers in Self-Supervised Monocular Depth Estimation with Unknown Camera Intrinsics. arXiv preprint arXiv:2202.03131.

\bibitem{scene_SideRT}
Shu, C., Chen, Z., Chen, L., Ma, K., Wang, M., & Ren, H. (2022). SideRT: A Real-time Pure Transformer Architecture for Single Image Depth Estimation. arXiv preprint arXiv:2204.13892.

\bibitem{scene_DepthFormer}
Li, Z., Chen, Z., Liu, X., & Jiang, J. (2022). DepthFormer: Exploiting Long-Range Correlation and Local Information for Accurate Monocular Depth Estimation. arXiv preprint arXiv:2203.14211.



%%%%HDmap%%%
\bibitem{HDmap_79}
M. Javanmardi et al., “Towards high-definition 3D urban mapping: Road feature-based registration of mobile mapping systems and aerial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017.

\bibitem{HDmap_80}
K. Wong, E. Javanmardi, M. Javanmardi, and S. Kamijo, “Estimating autonomous vehicle localization error using 2D geographic information,” ISPRS Int. J. Geo-Inform., vol. 8, no. 6, p. 288, 2019.

\bibitem{HDmap_34}
M. Javanmardi et al., “Towards high-definition 3D urban mapping:Road feature-based registration of mobile mapping systems and aer-
ial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017. 

\bibitem{HDmap_54}
M. Javanmardi et al., “Towards high-definition 3D urban mapping:Road feature-based registration of mobile mapping systems and aer-
ial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017.
%%%planning%%%
\bibitem{planning_1}
Katrakazas, M. Quddus, W. Chen, and L. Deka, “Real-time motion planning methods for autonomous on-road driving: State-of-the-art and future research directions,” {\it{Transportation Research Part C: Emerging Technologies}}, vol. 60, pp. 416 - 442, 2015.
\bibitem{planning_2}
Paden, B., Čáp, M., Yong, S. Z., Yershov, D., & Frazzoli, E. (2016). A survey of motion planning and control techniques for self-driving urban vehicles. {\it{IEEE Transactions on intelligent vehicles}}, 1(1), 33-55.
\bibitem{planning_3}
L. Claussmann, M. Revilloud, D. Gruyer, et al., “A review of motion planning for highway autonomous driving,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 21, no. 5, pp. 1826–1848, 2020.
\bibitem{planning_4}
H. Bast, D. Delling, A. Goldberg, et al., Route planning in transportation networks, in Algorithm Engineering. Cham, Switzerland: Springer, 2016, pp. 19–80.
\bibitem{planning_5}
D. Delling, P. Sanders, D. Schultes, and D. Wagner, “Engineering route planning algorithms,” in Algorithmics of Large and Complex Networks. Springer, 2009, pp. 117–139.
\bibitem{planning_6}
B. Li, Z. Yin, Y. Ouyang, et al.,  "Online trajectory replanning for sudden environmental changes during automated parking: A parallel stitching method," {\it{IEEE Transactions on Intelligent Vehicles}}, 2022.
\bibitem{planning_7}
Y. Huang, H. Ding, Y. Zhang, et al., A motion planning and tracking framework for autonomous vehicles based on artificial potential field elaborated resistance network approach. {\it{IEEE Transactions on Industrial Electronics}}, 67(2), 1376-1386, 2019.
\bibitem{planning_8}
Hoel, C. J., Driggs-Campbell, K., Wolff, K., Laine, L., & Kochenderfer, M. J. (2019). Combining planning and deep reinforcement learning in tactical decision making for autonomous driving. {\it{IEEE transactions on intelligent vehicles}}, 5(2), 294-305.
\bibitem{planning_9}
M. Montemerlo, J. Becker, S. Bhat, et al., (2008). Junior: The stanford entry in the urban challenge. {\it{Journal of Field Robotics}}, 25(9), 569-597.
\bibitem{planning_10}
Y. Liu, X. Hu, G. Chen, et al., Review of end-to-end motion planning for autonomous driving with visual perception.{\it{ Journal of Image and Graphics}}, 26(01): 49-66. 2021.
\bibitem{planning_11}
Rehder, E., Quehl, J., & Stiller, C. (2017, September). Driving like a human: Imitation learning for path planning using convolutional neural networks. {\it{In International Conference on Robotics and Automation Workshops}} (pp. 1-5).
\bibitem{planning_12}
Chen, L., Hu, X., Tian, W., Wang, H., Cao, D., & Wang, F. Y. (2018). Parallel planning: A new motion planning framework for autonomous driving. {\it{IEEE/CAA Journal of Automatica Sinica}}, 6(1), 236-246.
\bibitem{planning_13}
Zhang, X., Jiang, Y., Lu, Y., & Xu, X. (2022). A Receding-Horizon Reinforcement Learning Approach for Kinodynamic Motion Planning of Autonomous Vehicles. {\it{IEEE Transactions on Intelligent Vehicles}}.
\bibitem{planning_14}
Kendall, A., Hawke, J., Janz, D., Mazur, P., Reda, D., Allen, J. M., ... & Shah, A. (2019, May). Learning to drive in a day. {\it{In 2019 International Conference on Robotics and Automation (ICRA)}} (pp. 8248-8254). IEEE.
\bibitem{planning_15}
Aradi, S. (2020). Survey of deep reinforcement learning for motion planning of autonomous vehicles. {\it{IEEE Transactions on Intelligent Transportation Systems}}. vol. 23, no. 2, pp. 740 - 759.
\bibitem{planning_16}
B. Li, T. Acarman, Y. Zhang, et al., “Optimization-based trajectory planning for autonomous parking with irregularly placed obstacles: A lightweight iterative framework,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, 2021.
\bibitem{planning_17}
D. Dolgov, S. Thrun, M. Montemerlo, and J. Diebel, “Path planning for autonomous vehicles in unknown semi-structured environments,” Int. {\it{Journal of Robotics Research}}, vol. 29, no. 5, pp. 485–501, 2010.
\bibitem{planning_18}
Fassbender, D., Heinrich, B. C., & Wuensche, H. J. (2016, October). Motion planning for autonomous vehicles in highly constrained urban environments. In 2016 {\it{IEEE/RSJ international conference on intelligent robots and systems (IROS)}} (pp. 4708-4713). IEEE.
\bibitem{planning_19}
W. Xu, J. Pan, J. Wei, and J. M. Dolan, “Motion planning under uncertainty for on-road autonomous driving,” In Proc. 2014 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 2507–2512, 2014.
\bibitem{planning_20}
M. McNaughton, C. Urmson, J. M. Dolan, and J. Lee, “Motion planning for autonomous driving with a conformal spatiotemporal lattice,” In Proc. 2011 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 4889–4895, 2011.
\bibitem{planning_21}
H. Fan, F. Zhu, C. Liu, et al., “Baidu Apollo EM motion planner,” arXiv preprint, available at https://arxiv.org/abs/1807.08048, 2018.
\bibitem{planning_22}
X. Li, Z. Sun, D. Cao, et al., “Real-time trajectory planning for autonomous urban driving: framework, algorithms, and verifications,” {\it{IEEE/ASME Transactions on Mechatronics}}, vol. 21, no. 2, pp. 740–753, 2016.
\bibitem{planning_23}H. Bai, S. Cai, N. Ye, et al., (2015, May). Intention-aware online POMDP planning for autonomous driving in a crowd. In 2015 {\it{ieee international conference on robotics and automation (icra)}} (pp. 454-460). IEEE.
\bibitem{planning_24}
Ye, N., Somani, A., Hsu, D., & Lee, W. S. (2017). DESPOT: Online POMDP planning with regularization. {\it{Journal of Artificial Intelligence Research}}, 58, 231-266.
\bibitem{planning_25}
K. Kondak, and G. Hommel, “Computation of time-optimal movements for autonomous parking of non-holonomic mobile platforms,” In Proc. 2001 {\it{IEEE International Conference on Robotics and Automation}}, vol. 3, pp. 2698–2703, 2001.
\bibitem{planning_26}
X. Zhang, A. Liniger, A. Sakai, and F. Borrelli, “Autonomous parking using optimization-based collision avoidance,” In Proc. 2018 {\it{IEEE Conference on Decision and Control}}, pp. 4327–4332, 2018.
\bibitem{planning_27}
J. Chen, W. Zhan, and M. Tomizuka, “Autonomous driving motion planning with constrained iterative LQR,” {\it{IEEE Transactions on Intelligent Vehicles}}, vol. 4, no. 2, pp. 244–254, 2019.
\bibitem{planning_28}
A. Liniger, A. Domahidi, and M. Morari, “Optimization-based autonomous racing of 1:43 scale RC cars”, {\it{Optimal Control Applications and Methods}}, pp. 628–647, 2015.
\bibitem{planning_29}
B. Li, Y. Ouyang, L. Li and Y. Zhang, "Autonomous driving on curvy roads without reliance on Frenet frame: A cartesian-based trajectory planning method," {\it{IEEE Transactions on Intelligent Transportation Systems}}, doi: 10.1109/TITS.2022.3145389.
\bibitem{planning_30}
W. Lim, S. Lee, M. Sunwoo, et al., “Hierarchical trajectory planning of an autonomous car based on the integration of a sampling and an optimization method,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 19, no. 2, pp. 613–626, 2018.
\bibitem{planning_31}
Scheffe, P., Henneken, T. M., Kloock, M., & Alrifaee, B. (2022). Sequential convex programming methods for real-time optimal trajectory planning in autonomous vehicle racing. {\it{IEEE Transactions on Intelligent Vehicles}}.
\bibitem{planning_32}
Miller, C., Pek, C., & Althoff, M. (2018, June). Efficient mixed-integer programming for longitudinal and lateral motion planning of autonomous vehicles. In 2018 {\it{IEEE Intelligent Vehicles Symposium (IV)}} (pp. 1954-1961). IEEE.
\bibitem{planning_33}
Claussmann, L., Revilloud, M., & Glaser, S. (2019, May). Simulated annealing-optimized trajectory planning within non-collision nominal intervals for highway autonomous driving. In 2019 {\it{International Conference on Robotics and Automation (ICRA)}} (pp. 5922-5928). IEEE.
\bibitem{planning_34}
Quinlan, S., & Khatib, O. (1993, May). Elastic bands: Connecting path planning and control. In [1993] {\it{Proceedings IEEE International Conference on Robotics and Automation}} (pp. 802-807). IEEE.
\bibitem{planning_35}
Rösmann, C., Hoffmann, F., & Bertram, T. (2017). Integrated online trajectory planning and optimization in distinctive topologies. {\it{Robotics and Autonomous Systems}}, 88, 142-153.
\bibitem{planning_36}
Hang, P., Lv, C., Huang, C., Cai, J., Hu, Z., & Xing, Y. (2020). An integrated framework of decision making and motion planning for autonomous vehicles considering social behaviors. {\it{IEEE transactions on vehicular technology}}, 69(12), 14458-14469.
\bibitem{planning_37}
Gu, T., Atwood, J., Dong, C., Dolan, J. M., & Lee, J. W. (2015, September). Tunable and stable real-time trajectory planning for urban autonomous driving. In 2015 {\it{IEEE/RSJ international conference on intelligent robots and systems (IROS)}} (pp. 250-256). IEEE.
\bibitem{planning_38}
D. Le, Z. Liu, J. Jin, K. Zhang, and B. Zhang, “Historical improvement optimal motion planning with model predictive trajectory optimization for on-road autonomous vehicle,” In Proc. 45th {\it{Annual Conference of IEEE Industrial Electronics Society}}, pp. 5223–5230, 2019.
\bibitem{planning_39}
Park, J., Karumanchi, S., & Iagnemma, K. (2015). Homotopy-based divide-and-conquer strategy for optimal trajectory planning via mixed-integer programming. {\it{IEEE Transactions on Robotics}}, 31(5), 1101-1115.
\bibitem{planning_40}
J. Ziegler, P. Bender, T. Dang, et al., “Trajectory planning for Bertha — A local, continuous method,” In Proc. 2014 {\it{IEEE Intelligent Vehicles Symposium (IV)}}, pp. 450–457, 2014.
\bibitem{planning_41}
Dubins, L. E. (1957). On curves of minimal length with a constraint on average curvature, and with prescribed initial and terminal positions and tangents. {\it{American Journal of mathematics}}, 79(3), 497-516.
\bibitem{planning_42}
Reeds, J., & Shepp, L. (1990). Optimal paths for a car that goes both forwards and backwards. {\it{Pacific journal of mathematics}}, 145(2), 367-393.
\bibitem{planning_43}
M. Werling, J. Ziegler, S. Kammel, et al., “Optimal trajectory generation for dynamic street scenarios in a Frenet frame,” In Proc. 2010 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 987–993, 2010.
\bibitem{planning_44}
Patten, W. N., Wu, H. C., & Cai, W. (1994). Perfect parallel parking via Pontryagin's principle. J. Dyn. Sys., Meas., Control. Dec 1994, 116(4): 723-728.
\bibitem{planning_45}
Y. Kuwata, J. Teo, G. Fiore, et al., “Real-time motion planning with applications to autonomous urban driving,” {\it{IEEE Transactions on Control Systems Technology}}, vol. 17, no. 5, pp. 1105–1118, 2009.
\bibitem{planning_46}
Y. Zhang, H. Chen, S. Waslander, et al., “Hybrid trajectory planning for autonomous driving in highly constrained environments,” {\it{IEEE Access}}, vol. 6, pp. 32800–32819, 2018.
\bibitem{planning_47}
M. Rufli, and R. Siegwart, “On the design of deformable input-/ state-lattice graphs,” In Proc. 2010 {\it{IEEE International Conference on Robotics and Automation}}, pp. 3071–3077, 2010.
\bibitem{planning_48}
Bergman, K., Ljungqvist, O., & Axehill, D. (2020). Improved path planning by tightly combining lattice-based path planning and optimal control. {\it{IEEE Transactions on Intelligent Vehicles}}, 6(1), 57-66.
\bibitem{planning_49}
Liu, C., Zhan, W., & Tomizuka, M. (2017, June). Speed profile planning in dynamic environments via temporal optimization. In 2017 {\it{IEEE Intelligent Vehicles Symposium (IV)}} (pp. 154-159). IEEE.
\bibitem{planning_50}
L. Ma, J. Xue, K. Kawabata, et al., “Efficient sampling-based motion planning for on-road autonomous driving,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 16, no. 4, pp. 1961–1976, 2015.
\bibitem{planning_51}
Tian, F., Zhou, R., Li, Z., Li, L., Gao, Y., Cao, D., & Chen, L. (2022). Trajectory planning for autonomous mining trucks considering terrain constraints. {\it{IEEE Transactions on Intelligent Vehicles}}, 6(4), 772-786.
\bibitem{planning_52}
Müller, J., & Buchholz, M. (2019, October). A risk and comfort optimizing motion planning scheme for merging scenarios. In 2019 {\it{IEEE Intelligent Transportation Systems Conference (ITSC)}} (pp. 3155-3161). IEEE.
\bibitem{planning_53}
Hubmann, C., Schulz, J., Becker, M., Althoff, D., & Stiller, C. (2018). Automated driving in uncertain environments: Planning with interaction and uncertain maneuver prediction. {\it{IEEE transactions on intelligent vehicles}}, 3(1), 5-17.
\bibitem{planning_54}
Andersen, H., Alonso-Mora, J., Eng, Y. H., Rus, D., & Ang, M. H. (2019). Trajectory optimization and situational analysis framework for autonomous overtaking with visibility maximization. {\it{IEEE Transactions on Intelligent Vehicles}}, 5(1), 7-20.
\bibitem{planning_55}
Pek, C., & Althoff, M. (2020). Fail-safe motion planning for online verification of autonomous vehicles using convex optimization. {\it{IEEE Transactions on Robotics}}, 37(3), 798-814.


%%%%%%system%%%%%%%%%%%
\bibitem{system_1}
Liu, Liangkai, et al. "Computing systems for autonomous driving: State of the art and challenges." IEEE Internet of Things Journal 8.8 (2020): 6469-6486.
\bibitem{system_2}
Muller, Urs, et al. "Off-road obstacle avoidance through end-to-end learning." Advances in neural information processing systems 18 (2005). 
\bibitem{system_3}
Kendall, Alex, et al. "Learning to drive in a day." 2019 International Conference on Robotics and Automation (ICRA). IEEE, 2019.
\bibitem{system_4}
Liu, Shaoshan, et al. "Edge computing for autonomous driving: Opportunities and challenges." Proceedings of the IEEE 107.8 (2019): 1697-1716.
\bibitem{system_5}
Lin, Shih-Chieh, et al. "The architectural implications of autonomous driving: Constraints and acceleration." Proceedings of the Twenty-Third International Conference on Architectural Support for Programming Languages and Operating Systems. 2018.
\bibitem{system_6}
Liu, Shaoshan, et al. "Computer architectures for autonomous driving." Computer 50.8 (2017): 18-25.
\bibitem{system_7}
Wu, Tianze, et al. "Oops! It's Too Late. Your Autonomous Driving System Needs a Faster Middleware." IEEE Robotics and Automation Letters 6.4 (2021): 7301-7308.
\bibitem{system_8}
Yeong, De Jong, et al. "Sensor and sensor fusion technology in autonomous vehicles: A review." Sensors 21.6 (2021): 2140.
\bibitem{system_9}
Jagannadha, Pavan Kumar Datla, et al. "Special session: in-system-test (IST) architecture for Nvidia drive-AGX platforms." 2019 IEEE 37th VLSI Test Symposium (VTS). IEEE, 2019. 
\bibitem{system_10}
Boppana, Vamsi, et al. "UltraScale+ MPSoC and FPGA families." 2015 IEEE Hot Chips 27 Symposium (HCS). IEEE, 2015. 
\bibitem{system_11}
Jouppi, Norman P., et al. "Ten lessons from three generations shaped google’s tpuv4i: Industrial product." 2021 ACM/IEEE 48th Annual International Symposium on Computer Architecture (ISCA). IEEE, 2021.
\bibitem{system_12}
Hildebrand, Dan. "An Architectural Overview of QNX." USENIX Workshop on Microkernels and Other Kernel Architectures. 1992.
\bibitem{system_13}
Hambarde, Prasanna, Rachit Varma, and Shivani Jha. "The survey of real time operating system: RTOS." 2014 International Conference on Electronic Systems, Signal Processing and Computing Technologies. IEEE, 2014. Wu, Tianze, et al. 
\bibitem{system_14}
Wu, Tianze, et al. "Oops! It's Too Late. Your Autonomous Driving System Needs a Faster Middleware." IEEE Robotics and Automation Letters 6.4 (2021): 7301-7308. 
\bibitem{system_15}
Quigley, Morgan, et al. "ROS: an open-source Robot Operating System." ICRA workshop on open source software. Vol. 3. No. 3.2. 2009.
\bibitem{system_16}
DiLuoffo, Vincenzo, William R. Michalson, and Berk Sunar. "Robot Operating System 2: The need for a holistic security approach to robotic architectures." International Journal of Advanced Robotic Systems 15.3 (2018): 1729881418770011.
\bibitem{system_17}
Fayazbakhsh, Mohammad Ali, and Majid Bahrami. "Comprehensive modeling of vehicle air conditioning loads using heat balance method." SAE technical paper 2013 (2013): 1507.
\bibitem{system_18}
Farrington, Rob, and John Rugh. Impact of vehicle air-conditioning on fuel economy, tailpipe emissions, and electric vehicle range. No. NREL/CP-540-28960. National Renewable Energy Lab.(NREL), Golden, CO (United States), 2000.
\bibitem{system_19}
Fayyad, Jamil, et al. "Deep learning sensor fusion for autonomous vehicle perception and localization: A review." Sensors 20.15 (2020): 4220.
\bibitem{system_20}
Wang, Zhangjing, Yu Wu, and Qingqing Niu. "Multi-sensor fusion in automated driving: A survey." Ieee Access 8 (2019): 2847-2868.
\bibitem{system_21}
Marti, Enrique, et al. "A review of sensor technologies for perception in automated driving." IEEE Intelligent Transportation Systems Magazine 11.4 (2019): 94-108.
\bibitem{system_22}
Badue, Claudine, et al. "Self-driving cars: A survey." Expert Systems with Applications 165 (2021): 113816.
\bibitem{system_23}
Li, Ying, et al. "Deep learning for lidar point clouds in autonomous driving: A review." IEEE Transactions on Neural Networks and Learning Systems 32.8 (2020): 3412-3432.
\bibitem{system_24}
Wang, Dingkang, Connor Watkins, and Huikai Xie. "MEMS mirrors for LiDAR: a review." Micromachines 11.5 (2020): 456.
\bibitem{system_25}
Hsu, Ching-Pai, et al. "A review and perspective on optical phased array for automotive LiDAR." IEEE Journal of Selected Topics in Quantum Electronics 27.1 (2020): 1-16.
\bibitem{system_26}
Elhousni, Mahdi, and Xinming Huang. "A survey on 3d lidar localization for autonomous vehicles." 2020 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2020.
\bibitem{system_27}
Royo, Santiago, and Maria Ballesta-Garcia. "An overview of lidar imaging systems for autonomous vehicles." Applied Sciences 9.19 (2019): 4093.
\bibitem{system_28}
Van Nam, Dinh, and Kim Gon-Woo. "Solid-state LiDAR based-SLAM: A concise review and application." 2021 IEEE International Conference on Big Data and Smart Computing (BigComp). IEEE, 2021.
\bibitem{system_29}
Cui, Yaodong, et al. "Deep learning for image and point cloud fusion in autonomous driving: A review." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_30}
Van Brummelen, Jessica, et al. "Autonomous vehicle perception: The technology of today and tomorrow." Transportation research part C: emerging technologies 89 (2018): 384-406.
\bibitem{system_31}
Fayyad, Jamil, et al. "Deep learning sensor fusion for autonomous vehicle perception and localization: A review." Sensors 20.15 (2020): 4220.
\bibitem{system_32}
Debeunne, César, and Damien Vivet. "A review of visual-LiDAR fusion based simultaneous localization and mapping." Sensors 20.7 (2020): 2068.
\bibitem{system_33}
Zhou, Taohua, et al. "MMW radar-based technologies in autonomous driving: A review." Sensors 20.24 (2020): 7283.
\bibitem{system_34}
Wei, Zhiqing, et al. "MmWave Radar and Vision Fusion for Object Detection in Autonomous Driving: A Review." Sensors 22.7 (2022): 2542.
\bibitem{system_35}
Ma, Dingyou, et al. "Joint radar-communication strategies for autonomous vehicles: Combining two key automotive technologies." IEEE signal processing magazine 37.4 (2020): 85-97.
\bibitem{system_36}
Saponara, Sergio, Maria Sabrina Greco, and Fulvio Gini. "Radar-on-chip/in-package in autonomous driving vehicles and intelligent transport systems: Opportunities and challenges." IEEE Signal Processing Magazine 36.5 (2019): 71-84.
\bibitem{system_37}
Javadi, S. Hamed, and Alfonso Farina. "Radar networks: A review of features and challenges." Information fusion 61 (2020): 48-55.
\bibitem{system_38}
Mousazadeh, Hossein. "A technical review on navigation systems of agricultural autonomous off-road vehicles." Journal of Terramechanics 50.3 (2013): 211-232.
\bibitem{system_39}
Jing, Hao, et al. "Integrity Monitoring of GNSS/INS Based Positioning Systems for Autonomous Vehicles: State-of-the-Art and Open Challenges." IEEE Transactions on Intelligent Transportation Systems (2022). 
\bibitem{system_40}
Rosique, Francisca, et al. "A systematic review of perception system and simulators for autonomous vehicles research." Sensors 19.3 (2019): 648.
\bibitem{system_41}
Mohammed, Abdul Sajeed, et al. "The perception system of intelligent ground vehicles in all weather conditions: a systematic literature review." Sensors 20.22 (2020): 6532.
\bibitem{system_42}
Xing, Yang, et al. "Advances in vision-based lane detection: algorithms, integration, assessment, and perspectives on ACP-based parallel vision." IEEE/CAA Journal of Automatica Sinica 5.3 (2018): 645-661.
\bibitem{system_43}
Zhang, Hao, et al. "Image fusion meets deep learning: A survey and perspective." Information Fusion 76 (2021): 323-336.
\bibitem{system_44}
Kedem, Benjamin, Victor De Oliveira, and Michael Sverchkov. "Statistical data fusion." (2017).
\bibitem{system_45}
Berrio, Julie Stephany, et al. "Camera-LIDAR integration: Probabilistic sensor fusion for semantic mapping." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_46}
Sasiadek, J. Z., and P. Hartana. "Sensor data fusion using Kalman filter." Proceedings of the Third International Conference on Information Fusion. Vol. 2. IEEE, 2000.
\bibitem{system_47}
https://www.bsigroup.com/globalassets/localfiles/en-gb/cav/cav-standards-roadmap/cav-standards-roadmap-2022.pdf.
\bibitem{system_48}
Gao, Yu, Yunfeng Ai, Bin Tian, Long Chen, Jian Wang, Dongpu Cao, and Fei-Yue Wang. "Parallel end-to-end autonomous mining: An IoT-oriented approach." IEEE Internet of Things Journal 7, no. 2 (2019): 1011-1023.
\bibitem{system_49}
Hájnik, Ambróz, Veronika Harantová, and Alica Kalašová. "Use of electromobility and autonomous vehicles at airports in Europe and worldwide." Transportation Research Procedia 55 (2021): 71-78.
\bibitem{system_50}
Uhlemann, Elisabeth. "Autonomous Vehicles Have Entered the Off-Road Market [Connected and Automated Vehicles]." IEEE Vehicular Technology Magazine 16.2 (2021): 15-19.
\bibitem{system_51}
Van Meldert, Bram, and Liesje De Boeck. "Introducing autonomous vehicles in logistics: a review from a broad perspective." FEB Research Report KBI_1618 (2016).
\bibitem{system_52}
Omeiza, Daniel, et al. "Explanations in autonomous driving: A survey." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_53}
Zablocki, Éloi, et al. "Explainability of vision-based autonomous driving systems: Review and challenges." arXiv preprint arXiv:2101.05307 (2021).
\bibitem{system_54}Atakishiyev, Shahin, et al. "Explainable Artificial Intelligence for Autonomous Driving: A Comprehensive Overview and Field Guide for Future Research Directions." arXiv preprint arXiv:2112.11561 (2021).

@article{paden2016survey,
  title={A survey of motion planning and control techniques for self-driving urban vehicles},
  author={Paden, Brian and {\v{C}}{\'a}p, Michal and Yong, Sze Zheng and Yershov, Dmitry and Frazzoli, Emilio},
  journal={IEEE Transactions on intelligent vehicles},
  volume={1},
  number={1},
  pages={33--55},
  year={2016},
  publisher={IEEE}
}

@inproceedings{prediction1,
  title={Desire: Distant future prediction in dynamic scenes with interacting agents},
  author={Lee, Namhoon and Choi, Wongun and Vernaza, Paul and Choy, Christopher B and Torr, Philip HS and Chandraker, Manmohan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={336--345},
  year={2017}
}
@inproceedings{prediction2,
  title={Probabilistic prediction of vehicle semantic intention and motion},
  author={Hu, Yeping and Zhan, Wei and Tomizuka, Masayoshi},
  booktitle={2018 IEEE Intelligent Vehicles Symposium (IV)},
  pages={307--313},
  year={2018},
  organization={IEEE}
}
@inproceedings{prediction3,
  title={Fast and furious: Real time end-to-end 3d detection, tracking and motion forecasting with a single convolutional net},
  author={Luo, Wenjie and Yang, Bin and Urtasun, Raquel},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={3569--3577},
  year={2018}
}

@ARTICLE{Kalman1,
  author={Guo, Ge and Zhao, Shijie},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={3D Multi-Object Tracking with Adaptive Cubature Kalman Filter for Autonomous Driving}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TIV.2022.3158419}}
  
@ARTICLE{Kalman2,
  author={Bahramgiri, Mojtaba and Nooshabadi, Saeid and Olutomilayo, Kunle and Fuhrmann, Daniel},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Automotive Radar-Based Hitch Angle Tracking Technique for Trailer Backup Assistant Systems}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TIV.2022.3144896}}
  
@ARTICLE{Kalman3,
  author={Xie, Zhenming and Jeon, Woongsun and Rajamani, Rajesh},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Low-Density Lidar Based Estimation System for Bicycle Protection}, 
  year={2021},
  volume={6},
  number={1},
  pages={67-77},
  doi={10.1109/TIV.2020.3010728}}
  
@ARTICLE{graph1,
  author={Lv, Hui and Liu, Chao and Zhao, Xiaowei and Xu, Chunyan and Cui, Zhen and Yang, Jian},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Lane Marking Regression From Confidence Area Detection to Field Inference}, 
  year={2021},
  volume={6},
  number={1},
  pages={47-56},
  doi={10.1109/TIV.2020.3009366}}
  


@ARTICLE{graph3,
  author={Zhao, Chengfeng and Fu, Chen and Dolan, John M. and Wang, Jun},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={L-Shape Fitting-Based Vehicle Pose Estimation and Tracking Using 3D-LiDAR}, 
  year={2021},
  volume={6},
  number={4},
  pages={787-798},
  doi={10.1109/TIV.2021.3078619}}
  
@ARTICLE{TrackingNetwork1,
  author={Zhu, Yabin and Li, Chenglong and Tang, Jin and Luo, Bin},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Quality-Aware Feature Aggregation Network for Robust RGBT Tracking}, 
  year={2021},
  volume={6},
  number={1},
  pages={121-130},
  doi={10.1109/TIV.2020.2980735}}
  
@ARTICLE{TrackingNetwork2,
  author={Hoffmann, João Eduardo and Tosso, Hilkija Gaïus and Santos, Max Mauro Dias and Justo, João Francisco and Malik, Asad Waqar and Rahman, Anis Ur},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Real-Time Adaptive Object Detection and Tracking for Autonomous Vehicles}, 
  year={2021},
  volume={6},
  number={3},
  pages={450-459},
  doi={10.1109/TIV.2020.3037928}}
  
@inproceedings{TrackingLSTM1,
  title={Online multi-target tracking using recurrent neural networks},
  author={Milan, Anton and Rezatofighi, S Hamid and Dick, Anthony and Reid, Ian and Schindler, Konrad},
  booktitle={Thirty-First AAAI conference on artificial intelligence},
  year={2017}
}

@inproceedings{TrackingLSTM2,
  title={Probabilistic vehicle trajectory prediction over occupancy grid map via recurrent neural network},
  author={Kim, ByeoungDo and Kang, Chang Mook and Kim, Jaekyum and Lee, Seung Hi and Chung, Chung Choo and Choi, Jun Won},
  booktitle={2017 IEEE 20th International Conference on Intelligent Transportation Systems (ITSC)},
  pages={399--404},
  year={2017},
  organization={IEEE}
}



% human-machine
\bibitem{human-machine_1}Hasenjäger, Martina, Martin Heckmann, and Heiko Wersing. "A survey of personalization for advanced driver assistance systems." IEEE Transactions on Intelligent Vehicles 5.2 (2019): 335-344.
\bibitem{human-machine_2}Xing, Yang, Chen Lv, Dongpu Cao, and Peng Hang. "Toward human-vehicle collaboration: Review and perspectives on human-centered collaborative automated driving." Transportation research part C: emerging technologies 128 (2021): 103199.
\bibitem{human-machine_3}Wang, Wenshuo, and Ding Zhao. "Evaluation of lane departure correction systems using a regenerative stochastic driver model." IEEE Transactions on Intelligent Vehicles 2.3 (2017): 221-232.
\bibitem{human-machine_4}Chen, Wuwei, et al. "Human–machine shared control for lane departure assistance based on hybrid system theory." Control Engineering Practice 84 (2019): 399-407.
\bibitem{human-machine_5}Althoff, Matthias, Sebastian Maierhofer, and Christian Pek. "Provably-correct and comfortable adaptive cruise control." IEEE Transactions on Intelligent Vehicles 6.1 (2020): 159-174.
\bibitem{human-machine_6}Utriainen, Roni, Markus Pöllänen, and Heikki Liimatainen. "The safety potential of lane keeping assistance and possible actions to improve the potential." IEEE Transactions on Intelligent Vehicles 5.4 (2020): 556-564.
\bibitem{human-machine_7}Lal, Saroj KL, and Ashley Craig. "A critical review of the psychophysiology of driver fatigue." Biological psychology 55.3 (2001): 173-194.
\bibitem{human-machine_8}Xing, Yang, et al. "Driver lane change intention inference for intelligent vehicles: framework, survey, and challenges." IEEE Transactions on Vehicular Technology 68.5 (2019): 4377-4390.
\bibitem{human-machine_9}Hu, Zhongxu, et al. "Data-driven estimation of driver attention using calibration-free eye gaze and scene features." IEEE Transactions on Industrial Electronics 69.2 (2021): 1800-1808.
\bibitem{human-machine_10}Marquart, Gerhard, Christopher Cabrall, and Joost de Winter. "Review of eye-related measures of drivers’ mental workload." Procedia Manufacturing 3 (2015): 2854-2861.
\bibitem{human-machine_11}Zepf, Sebastian, et al. "Driver emotion recognition for intelligent vehicles: A survey." ACM Computing Surveys (CSUR) 53.3 (2020): 1-30.
\bibitem{human-machine_12}Kashevnik, Alexey, et al. "Driver distraction detection methods: A literature review and framework." IEEE Access 9 (2021): 60063-60076.
\bibitem{human-machine_13}Balandong, Rodney Petrus, et al. "A review on EEG-based automatic sleepiness detection systems for driver." Ieee Access 6 (2018): 22908-22919.
\bibitem{human-machine_14}Xing, Yang, Chen Lv, Yifan Zhao, Yahui Liu, Dongpu Cao, and Sadahiro Kawahara. "Pattern recognition and characterization of upper limb neuromuscular dynamics during driver-vehicle interactions." Iscience 23, no. 9 (2020): 101541.
\bibitem{human-machine_15}Zhongxu Hu, et al. Review and Perspectives on Driver Digital Twin and Its Enabling Technologies for Intelligent Vehicles. IEEE Trans. on Intelligent Vehicles. 2022.
\bibitem{human-machine_16}Du, Na, et al. "Predicting driver takeover performance in conditionally automated driving." Accident Analysis & Prevention 148 (2020): 105748.
\bibitem{human-machine_17}Weaver, Bradley W., and Patricia R. DeLucia. "A systematic review and meta-analysis of takeover performance during conditionally automated driving." Human factors (2020): 0018720820976476.
\bibitem{human-machine_18}Louw, Tyron, et al. "Driver inattention during vehicle automation: How does driver engagement affect resumption of control?." 4th International Conference on Driver Distraction and Inattention (DDI2015), Sydney: proceedings. ARRB Group, 2015.
\bibitem{human-machine_19}Salubre, Kevin Joel, and Dan Nathan-Roberts. "Takeover request design in automated driving: a systematic review." Proceedings of the Human Factors and Ergonomics Society Annual Meeting. Vol. 65. No. 1. Sage CA: Los Angeles, CA: SAGE Publications, 2021.
\bibitem{human-machine_20}Eriksson, Alexander, and Neville A. Stanton. "Takeover time in highly automated vehicles: noncritical transitions to and from manual control." Human factors 59.4 (2017): 689-705.
\bibitem{human-machine_21}Hu, Zhongxu, et al. "Driver Anomaly Quantification for Intelligent Vehicles: A Contrastive Learning Approach with Representation Clustering." IEEE Transactions on Intelligent Vehicles (2022).
\bibitem{human-machine_22}Lv, Chen, et al. "Human–Machine Collaboration for Automated Driving Using an Intelligent Two‐Phase Haptic Interface." Advanced Intelligent Systems 3.4 (2021): 2000229.
\bibitem{human-machine_23}Jing, Peng, et al. "The Determinants behind the Acceptance of Autonomous Vehicles: A Systematic Review." Sustainability 12.5 (2020): 1719.
\bibitem{human-machine_24}Olaverri-Monreal, Cristina. "Promoting trust in self-driving vehicles." Nature Electronics 3.6 (2020): 292-294.
\bibitem{human-machine_25}Choi, Jong Kyu, and Yong Gu Ji. "Investigating the importance of trust in adopting an autonomous vehicle." International Journal of Human-Computer Interaction 31.10 (2015): 692-702.
\bibitem{human-machine_26}Dikmen, Murat, and Catherine Burns. "Trust in autonomous vehicles: The case of tesla autopilot and summon." 2017 IEEE International Conference on Systems, Man, and Cybernetics (SMC). IEEE, 2017.
\bibitem{human-machine_27}Ayoub, Jackie, et al. "From manual driving to automated driving: A review of 10 years of autoui." Proceedings of the 11th International Conference on Automotive User Interfaces and Interactive Vehicular Applications. 2019.
\bibitem{human-machine_28}Liu, Weimin, et al. "A Literature Review on Additional Semantic Information Conveyed from Driving Automation Systems to Drivers through Advanced In-Vehicle HMI Just Before, During, and Right After Takeover Request." International Journal of Human–Computer Interaction (2022): 1-21.
\bibitem{human-machine_29}Politis, Ioannis, et al. "Designing autonomy in cars: A survey and two focus groups on driving habits of an inclusive user group, and group attitudes towards autonomous cars." International Conference on Applied Human Factors and Ergonomics. Springer, Cham, 2017.
\bibitem{human-machine_30}Benderius, Ola, Christian Berger, and Victor Malmsten Lundgren. "The best rated human–machine interface design for autonomous vehicles in the 2016 grand cooperative driving challenge." IEEE Transactions on intelligent transportation systems 19.4 (2017): 1302-1307.
\bibitem{human-machine_31}Bengler, Klaus, et al. "From HMI to HMIs: Towards an HMI Framework for Automated Driving." Information 11.2 (2020): 61.
\bibitem{human-machine_32}Wulf, Felix, et al. "Recommendations supporting situation awareness in partially automated driver assistance systems." IEEE Transactions on Intelligent Transportation Systems 16.4 (2014): 2290-2296.
\bibitem{human-machine_33}Richardson, Natalie Tara, et al. "Conceptual design and evaluation of a human machine interface for highly automated truck driving." 2018 IEEE intelligent vehicles symposium (IV). IEEE, 2018.
\bibitem{human-machine_34}Chen, Danjue, et al. "Towards vehicle automation: Roadway capacity formulation for traffic mixed with regular and automated vehicles." Transportation research part B: methodological 100 (2017): 196-221.
\bibitem{human-machine_35}Benderius, Ola, Christian Berger, and Victor Malmsten Lundgren. "The best rated human–machine interface design for autonomous vehicles in the 2016 grand cooperative driving challenge." IEEE Transactions on intelligent transportation systems 19.4 (2017): 1302-1307.
\bibitem{human-machine_36}Zandi, Babak, et al. "International study on the importance of communication between automated vehicles and pedestrians." Transportation research part F: traffic psychology and behaviour 74 (2020): 52-66.
\bibitem{human-machine_37}	Hu, Z., et al. "Toward human-centered automated driving: a novel spatiotemporal vision transformer-enabled head tracker. IEEE Vehi Technol Mag 2–9." (2021).
\bibitem{human-machine_38}Rahman, Md Mahmudur, et al. "How the older population perceives self-driving vehicles." Transportation research part F: traffic psychology and behaviour 65 (2019): 242-257. 
\bibitem{human-machine_39}Linkov, Václav, et al. "Human factors in the cybersecurity of autonomous vehicles: Trends in current research." Frontiers in psychology 10 (2019): 995.
\bibitem{human-machine_40}Kong, Qinglei, et al. "Blockchain-based privacy-preserving driver monitoring for maas in the vehicular iot." IEEE Transactions on Vehicular Technology 70.4 (2021): 3788-3799.
\bibitem{human-machine_41}Holstein, Tobias, Gordana Dodig-Crnkovic, and Patrizio Pelliccione. "Ethical and social aspects of self-driving cars." arXiv preprint arXiv:1802.04103 (2018).

%\end{thebibliography}

==> body/methodology.tex <==
\section{Methodology}

\begin{figure*}
\centering  %图片全局居中
\includegraphics[width=18cm]{picture/methodology/framework.png}

\caption{The structure of autonomous driving with the function, methodology and application scenes}
\label{fig:structure}
\end{figure*}

We divide the methodology into eight sub-sections, including perception, planning, control, system, HD map, communication, testing, and human behaviors in AVs (perception, planning, and motion control in Part II). The structure can be seen in Fig. \ref{fig:structure}.

%\input{body/methodology/detection}

%\input{body/methodology/planning}

%\input{body/methodology/control}

\input{body/methodology/system}

\input{body/methodology/communication}

\input{body/methodology/HDmap}

\input{body/methodology/testing}

\input{body/methodology/human-mechine}


==> body/methodology/HDmap.tex <==
\subsection{HD map}

Maps are an integral part of modern autonomous driving. The information from the map supports many functions of autonomous driving, including self-orientation, vehicle control, motion planning, perception and systems management. Broadly speaking, a map is a representation of features of the real world and their locations as objects. It is a symbolic and abstract description of object features (such as buildings, roads and lakes) and non-object concepts (such as air pressure or temperature). The narrow definition of maps is that maps provide information about real-world features or phenomena and their position in 2D or 3D space.

The information provided by HDmap can be divided into three categories: topological information, geometric information and semantic information. Topology information contains connectivity information between geometric features, geometric information contains geometric shape mapping data of objects around vehicles, semantic information shows road speed limit, lane information and road classification, etc.

The data quality of autonomous driving maps consists of five components: 1) accuracy, 2) precision, 3) completeness, 4) consistency, and 5) timeliness. Accuracy is the difference or deviation between the actual value and the mapped value. Precision means the smallest discernible unit of a map. Completeness means the extent to which a map contains all real-world features, which is measured by omission (missing data) and redundancy (presence of too much data). Consistency also refers to the extent to which logical rules of data structure, attributes, and relationships are followed. Timeliness means the time between map creation and use.

In order to increasing data quality, Wong and Ellul\cite{HDmap_81}proposed geometry-based metrics as part of fitness assessment for 3D maps. Javanmardi et al.\cite{HDmap_79} defined four criteria to evaluate the vehicle location capability of maps, from the view of layout, feature adequacy, presentation quality and local similarity. Murphy and Pao\cite{HDmap_82} proposed a method for detecting unmapped or mismapped roads and parking lots in the context of map matching, resulting to a system that is more robust and can even correct errors in the underlying map. From a similar but alternative perspective, Yang and Huang\cite{HDmap_80} studied how to make autonomous vehicle systems more resistant to malicious attacks on their sensors.

==> body/methodology/communication.tex <==
\subsection{\textbf{Communication}}
As a powerful extension of the perception capabilities of autonomous driving and intelligent vehicles, the communication of intelligent vehicles not only involves the vehicles themselves, but also involves a variety of infrastructure and technical elements of transportation, communication, and other systems, and is a focused area for the integration and convergence of automotive, transportation, communication, information, and other industries. Vehicular communication technology originated from academic research and demonstration projects conducted in Europe and the United States at the end of the 20th century that focused on vehicle-to-vehicle (V2V) and vehicle-to-infrastructure (V2I) communications, which was known as vehicular ad-hoc network (VANET) \cite{hartenstein2008tutorial} or vehicular network at that time. With the development of the novel information and communication technologies, the connection and cooperation of all elements in transportation systems has been further strengthened to form a connected and cooperative autonomous driving, the concept of VANET was extended to the Internet of vehicles and it has gained wide attention due to its supporting role for industries such as intelligent transportation and autonomous driving.

%\cite{weiss2011v2x,abboud2016interworking}
%\cite{jiang2008ieee,chen2020vision}

With the expansion of the concept, the vehicular communication technology has evolved from the VANET that connects vehicles and infrastructure to the vehicle-to-everything (V2X) \cite{abboud2016interworking} that connects various elements of the transportation system such as vehicles, infrastructures, pedestrians and clouds. Specifically, V2X contains two types of technologies, dedicated short range communication (DSRC) standardized by IEEE and cellular V2X (C-V2X) standardized by the 3rd Generation Partnership Project (3GPP) \cite{chen2020vision}. In terms of communication methods, V2X communication can be subdivided into V2V, V2I, vehicle-to-pedestrian (V2P), and vehicle-to-cloud/network (V2C/N) communication. Therefore, vehicular networks can realize real-time and efficient information interaction among pedestrians, vehicles, infrastructures, and clouds, and support the massive data transmission of autonomous driving and intelligent vehicles.

\subsubsection{\textbf{Standardization of V2X Communication}}
To achieve efficient communication and interaction between heterogeneous vehicles, it is necessary to establish unified protocols and standards covering from the physical layer to the application layer. As mentioned above, based on different radio access technologies, there are two major types of V2X communication standards, namely DSRC and C-V2X. In this section, we briefly present the status and development of these two types of standards.

%\cite{weiss2011v2x,abboud2016interworking,kenney2011dedicated}
%\cite{eichler2007performance,survey_communication_7}

\textbf{\textit{1.1 DSRC}}: 
Strictly speaking, DSRC is a radio access technology for vehicular communication, but it is also used to broadly refer to vehicular communication based on this radio access technology. Currently, the technology is relatively mature, and several organizations for standardization, such as IEEE, Society of Automotive Engineers (SAE), and European Telecommunications Standards Institute (ETSI), have worked on DSRC-related standards \cite{abboud2016interworking}. Here we take the standard of the United States as an example to describe its standardization. In the United States, IEEE has developed the IEEE 802.11p and IEEE 1609 standards for the 5.9 GHz spectrum and formed the WAVE protocol stack \cite{uzcategui2009wave}. IEEE 802.11p is a communication protocol expanded from the IEEE 802.11 standard to support vehicular communication in a mobility environment \cite{survey_communication_7}. The IEEE 1609 protocol family is a high-level protocol for WAVE, including 1609.1, 1609.2, 1609.3, 1609.4, etc. \cite{teixeira2014vehicular,dibaei2022investigating}. Specifically, 1609.1 is a standard on resource management at the application layer of WAVE, 1609.2 defines secure message formats and their processing, 1609.3 defines routing and transport services, and 1609.4 mainly provides a communication standard for multi-channel cooperation. It is worth noting that the Federal Communications Commission (FCC) has already reallocated the 70 MHz dedicated spectrum for DSRC in 2019 and dedicated 20 MHz of that band for C-V2X technology. In 2020, the FCC added another 10 MHz to the previous proposal, formally allocating 30 MHz of spectrum to C-V2X communications and dropping support for DSRC communications \cite{fcc2020use}.

\textbf{\textit{1.2 C-V2X}}
The standardization of C-V2X technology by 3GPP can be divided into two phases, LTE-V2X and NR-V2X, which complement each other and are designed with forwarding and backward compatibility considerations \cite{gyawali2021challenges}. C-V2X mainly includes two types of communication methods, cellular mobile communication (using Uu interface) and sidelink communication (using PC5 interface) \cite{hasan2020securing}.
The standardization of LTE-V2X was initially completed in 3GPP Release 14, and its main application scenario was safety-oriented services for intelligent driving assistance. Release 15 enhanced the LTE-V2X technology and supported some enhanced applications of vehicular communication. To support the requirements of advanced V2X services and autonomous driving, 3GPP Release 16 and 17 carried out research on NR-V2X and enhanced the PC5 and Uu interfaces based on 5G NR, and the related standards are frozen now \cite{chen2020vision}.
LTE-V2X, based on 4G cellular communication, is the first C-V2X communication technology, which defines the basic architecture and technical principle of C-V2X combining cellular mobile communication and sidelink communication methods \cite{chen2016lte}.
NR-V2X, based on 5G communication, is an evolutionary version of LTE-V2X. It follows the system architecture and key technical principles of combining the Uu and PC5 interfaces defined in LTE-V2X. Meanwhile, to support a series of enhanced V2X services such as platooning, extended sensors, and remote driving for the future, NR-V2X is enhanced with novel technologies of 5G NR on the PC5 interface to provide higher data rate, low latency, and ultra reliable communication services. In terms of key technologies, NR-V2X supports unicast and multicast communication modes in addition to broadcast, and adaptive improvements have been made to resource allocation and synchronization mechanisms \cite{naik2019ieee}.

\subsubsection{\textbf{Innovative Studies of Vehicular Communication}}
Facing the stringent requirements of intelligent vehicles and autonomous driving for vehicular communication, researchers have proposed improvements and optimizations for the existing vehicular communication methods in several research directions of communication and networks \cite{ahmed2018cooperative}. In this part, we briefly present innovative studies for vehicular communication in terms of the physical layer, media access control, routing, and security.

\textbf{\textit{2.1 Physical Layer}}:
The physical layer is one of the important parts that affect the performance of vehicular communication, which enables the transmission of vehicle and traffic data through radio channels \cite{liang2017vehicular}. Currently, OFDM is the major modulation technology in vehicular communication \cite{wang2019networking}, thus many studies are devoted to optimizing orthogonal frequency division multiplexing (OFDM) parameters to ensure reliable and efficient data transmission \cite{arslan2017effects}. In addition, facing the requirement of data rate for communication in autonomous driving and intelligent vehicles, millimeter-wave communication \cite{ghafoor2020millimeter} and visible light communication (VLC) \cite{memedi2021vehicular} in the vehicular environment have become emerging research directions.

\textbf{\textit{2.2 Congestion Control}}:
Since the bandwidth of vehicular communication is limited, with large-scale deployment of vehicles, the access of massive terminals can lead to channel congestion and cause delay or even failure of data transmission \cite{paranjothi2020survey}. Congestion control avoids the congestion in the channel and improves the stability and reliability of data transmission through power-based, rate-based, hybrid, priority-based, and cross-layer approaches \cite{rashmi2021survey}.

\textbf{\textit{2.3 Resource Allocation}}:
Facing the dynamic channel access and multi-user interference caused by the high mobility of massive vehicles, vehicular communication maximizes the system performance by optimizing the allocation of resources such as channels, bandwidth, and transmit power \cite{ahmed2018cooperative}. For DSRC, various studies have proposed schemes such as medium access control (MAC) parameter allocation, channel allocation, and rate allocation \cite{noor2022survey}. For C-V2X, resources are efficiently utilized through centralized schemes based on clustering, cloud computing, non-orthogonal multiple access (NOMA) and semi-persistent scheduling, and distributed schemes based on location, sensing, and enhanced randomization \cite{le2021comprehensive}. In addition, machine learning, especially deep reinforcement learning, as a powerful analytical technique for complex problems, has become an important scheme for resource allocation and optimization \cite{nguyen2021drl}.

\textbf{\textit{2.4 Routing}}:
In vehicular communication, the range of one-hop communication between vehicles and other units (vehicles or infrastructure) is limited, so routing is needed to achieve long-distance data interaction between vehicles and vehicles or roadside infrastructures \cite{jeong2021comprehensive}. However, facing the frequently changing topology and unstable connections caused by the high-speed movement of vehicles, the traditional routing methods in wireless communication are no longer applicable \cite{ksouri2022towards,xia2021comprehensive}. Therefore, many studies have proposed enhanced routing schemes in vehicular communication to achieve efficient and stable data exchange, which include position-based, topology-based, geocast-based, broadcast-based, and cluster-based routing protocols \cite{wang2019networking,sun2021applications}. Various routing protocols improve the quality of service (QoS) of vehicular communication by optimizing the delay, distance, reliability, energy consumption, or security of routing \cite{belamri2021survey}. In addition, with the development of machine learning, learning-based routing protocols have also attracted more attention \cite{kayarga2021study}.


%\cite{sun2021applications,hasan2020securing}
%\cite{gyawali2021challenges,alladi2022comprehensive}
%\cite{sheikh2019survey,farooq2021survey,gyawali2021challenges}
%\cite{alladi2022comprehensive,dibaei2022investigating,talpur2022machine}

\textbf{\textit{2.5 Security}}: Intelligent vehicles interact with traffic systems through vehicular communication to improve driving safety and traffic efficiency \cite{hasan2020securing}. In this environment, attacks such as replay attacks, man-in-the-middle attacks, impersonation attacks, spoofing attacks, and malicious third-party attacks threaten the information security and even driving safety of vehicles \cite{gyawali2021challenges}. Therefore, facing the security requirements of vehicular communication, various studies prevent malicious attacks in terms of authentication, authorization, confidentiality, data integrity, and availability \cite{farooq2021survey,gyawali2021challenges}. In addition, machine learning-based attack detection and blockchain-based consensus and tamper-proof have become emerging research directions \cite{dibaei2022investigating,talpur2022machine}.

\subsubsection{\textbf{Future Research Directions}}
Vehicular communication realizes the connection and interaction among pedestrians, vehicles, roadside infrastructures, and cloud platforms. With the improvement of communication capability in the future, the vehicular communication system will not only complete the interaction of data but also realize the cooperation among vehicles, roadside infrastructures, and cloud platforms. The potential development directions of vehicular communication are as follows.

\textbf{\textit{3.1 Communication Technology Evolution and Performance Improvement}}:
With the evolution of C-V2X communication, the chips, modules, and terminals based on NR-V2X communication will be gradually commercialized. The application of the novel communication technology will significantly improve the communication performance of the vehicular communication system, and build a large bandwidth, high reliability, and low latency connection between the pedestrian, vehicle, infrastructure, and cloud. Relying on this high-performance communication technology, vehicular communication will no longer be limited to the basic assistant warning scenarios, but will further support the realization of various high-level cooperation and control scenarios, such as remote driving, sensor sharing, platooning, and advanced driving, and promote the intelligent transportation services to the next generation.

\textbf{\textit{3.2 From Data Interaction to Cooperative Intelligence}}:
With the performance improvement of vehicular communication and the development of sensing and computing technology, the function of vehicles and roadside infrastructures will no longer be limited to the reception and dissemination of information, but will further cooperate to complete the sensing, decision-making, and control in the complex traffic environment, thus realizing the highly cooperative operation of the vehicular communication system. In addition to the onboard sensors of intelligent vehicles, roadside infrastructure will deploy cameras, LiDARs, radars, and other devices. With the cooperative capability provided by vehicular communication, the sensing results of each intelligent terminal will be further shared, thus solving the ineffectiveness of perception by individual vehicles caused by low penetration of communication or obstacle occlusion.

\textbf{\textit{3.3 Integration of Communication and Computing}}: 
With the empowerment of vehicular communication, the connectivity and intelligence of vehicles will be further enhanced, resulting in vehicle-infrastructure-cloud connectivity and cooperation in various scenarios. The compute-intensive and latency-sensitive applications in these environments impose stringent requirements on communication rate, transmission reliability, computational real-time, and computing power scheduling. Facing these requirements, the communication and computation of the system can be integrated and resources can be scheduled and allocated cooperatively to support the development of autonomous driving.

==> body/methodology/control.tex <==

\subsection{\textbf{Control}}
Vehicle motion control is an important duty for enhanced driver assistance features. Many control tasks, such as lateral stability control and driving at the limits for accident avoidance, must be considered in the context of a highly automated vehicle. This section summarizes some of the major advancements in automated vehicle control during the previous few years. We will introduce the function of vehicle motion control, provide a comprehensive discussion on control strategies and discuss the state-of-the-art validation methods of control strategies.

\subsubsection{\textbf{Categories of Vehicle Motion Control}} 
We category the vehicle motion control into two sub parts, the longitudinal vehicle control and the lateral vehicle control.
%and the integration of lateral and longitudinal control.

\textbf{\textit{1.1 Longitudinal Vehicle Control}}: Longitudinal control manages the acceleration of the vehicle through the vehicle’s throttle and brake to keep a safe distance behind another vehicle, maintain the desirable velocity on the road and apply the brake as quickly as possible to avoid rear-end collisions in emergencies \cite{nobe2001overview, survey_control_6, smc_4, smc_6, smc_9, smc_10, smc_12, smc_24}.

%\cite{kim1996fuzzy,isermann1995nonlinear}

Longitudinal control strategies have been investigated in various scenarios, including platooning for connected autonomous vehicle (CAV) \cite{gong2016constrained, wei2017dynamic, arefizadeh2018platooning}, speed harmonization \cite{malikopoulos2018optimal, ma2016freeway}, trajectory smoothing \cite{li2018piecewise}, and speed management on signalized arterials \cite{altan2017glidepath, hao2018eco}. Local and string stability are crucial aspects of platoon longitudinal controllers. Local stability refers to a vehicle's capacity to maintain an equilibrium state under the condition of disturbance.  String stability refers to the magnitude of a disturbance that reduces or remains constant as it propagates through a platoon of vehicles. The control strategies for speed harmonization aim to determine the speed policy of the vehicles so that to prevent traffic break-downs and mitigate the loss of highway performance. The fundamental idea of trajectory smoothing is to improve traffic flow stability and efficiency through the longitudinal control strategy of CAV. On signalized arterials, speed management systems aim to adjust signal timing to reduce stops at signalized crossings while smoothing vehicle trajectories. Common longitudinal control strategies include Fuzzy logic \cite{kim1996fuzzy}, Proportional–Integral–Derivative (PID) \cite{choi1996robust}, model predictive control (MPC) \cite{zhou2019distributed}, game theory \cite{huang2019game}, sliding mode control (SMC) \cite{wu2019path}, Fuzzy inference system (FIS) \cite{mar2001anfis}, Lyapunov-based adaptive control approaches \cite{swaroop2001direct}, and AI-approaches \cite{chen2017learning}. The challenges dealing with within the design of the longitudinal control system include string-stable operation with tiny headway, execution of longitudinal split, and join manoeuvres subject to communication limitations \cite{dai2005approach, smc_25}.

%\cite{gong2016constrained, nobe2001overview}
%\cite{falcone2007predictive, kim2014model}
%\cite{tai2002experimental, guo2013adaptive, liu2021super, sun2019nested}

\textbf{\textit{1.2 Lateral Vehicle Control}}: 
Lateral vehicle control systems focus on the vehicle’s position in the lane. The major function of the lateral vehicle control system is to keep the vehicle in the current lane (lane-keeping), drive the vehicle to the adjacent lane (lane change), or avoid collisions with its preceding vehicle \cite{gong2016constrained}. The control tasks for lateral control are to minimize the lateral displacement and the angular error with regard to the reference trajectory \cite{survey_planning_4}. Various linear and nonlinear controllers have been reported in the literature to control the motion of the vehicle including Game theory-based approaches \cite{zhang2019game,yu2018human,talebpour2015modeling}, PID \cite{marino2011nested}, MPC \cite{kim2014model}, $H_\infty$ robust control \cite{ganzelmeier2001robustness, smc_26}, Lyapunov-based adaptive control approaches \cite{choi2000design, netto2004lateral}, Linear Parameter Varying Controllers \cite{huang2005ltv, baslamisli2009gain, besselmann2009autonomous}, SMC \cite{guo2013adaptive, liu2021super, sun2019nested}, Fuzzy logic \cite{guo2012design, arifin2022steering} and deep learning-based approach \cite{eraqi2017end}.

As the lateral control system can change the vehicles’ lane safely and perform evasive manoeuvres, it can offer potential benefits in reducing accidents and enhancing driving safety. However, full implementation of lateral vehicle control remains a real-world difficulty in lance changes and evasive maneuvers. For example, environmental factors such as weather conditions, road curves, and other various disturbances may affect the control performance and a proper lateral control strategy is needed.

%\textbf{Integration of Lateral and Longitudinal Control:}
%To couple characteristics between the lateral and longitudinal dynamics of intelligent vehicles in order to achieve difficult control objectives (e.g. sharp turn at high speed), the research on the design of constructing integrated control laws for lateral and longitudinal motions has attracted the researchers' attention.

%The integrated control of horizontal and lateral motions can be divided into decomposed control and centralized control. Decomposed coordinated control decouples horizontal and lateral dynamics, constructs horizontal and lateral control laws independently, and designs control logic to coordinate the horizontal and lateral dynamics at the same time. For example \cite{rajamani2000demonstration} designs an integrated control system that includes three components: lateral controller, longitudinal controller, and supervisor. The supervisor module is responsible to coordinate the lateral/longitudinal controller by monitoring the vehicle state in real-time.  The centralized coordinated control refers to obtaining the integrated control law by controlling the vehicle's lateral and longitudinal coupling dynamics model directly. \cite{bae2014integrated} presents a systematic design of the integrated control of vehicle lateral and longitudinal motions to maximize the capacity to transfer traction forces longitudinally and laterally in the most efficient way possible. The simulation results show that centralized coordinated control can remove the conventional simplifications on vehicle dynamics and deal with unmatched nonlinear vehicles and overcome the non-linear and strong coupling horizontal and vertical characteristics. However, it highly depends on high-quality hardware support.

%Compared to the independent control design (longitudinal or lateral) mentioned above, only a few such works on integrated control of horizontal and lateral motion have been reported, see game-theoretic approaches \cite{wang2015game,dreves2018generalized}, neural network \cite{naranjo2006acc+,rausch2017learning}, $H_\infty$ robust control \cite{peng2006robust}.

\subsubsection{\textbf{Control Methodology}} 
We introduce severval common methodologies in vehicle control.

\textbf{\textit{2.1 Proportional–Integral–Derivative (PID) Control}}: 
The generic applicability of the PID controller can make it outperform other control approaches to in-vehicle control for intelligent vehicles \cite{choi1996robust, connolly1999longitudinal, smc_7, smc_14, smc_15, smc_16, smc_17, smc_18, smc_19}. A nested PID steering control is developed for lateral control of autonomous vehicles in the condition of unknown route curvature \cite{yu2018human}. PID control has the advantages of simple structures, easy implementation, and no need to know the in-depth knowledge of the behavior of the system. However, PID parameters tuning is challenge and no optimal performance guaranteed. In addition, it is hard for PID controllers to be adaptive and robust to unknown and changeable external environments \cite{huang2017parameterized}.

\textbf{\textit{2.2 Game-theoretic Approaches}}: 
In game theory approaches, the vehicles are regarded as game participants and traffic rules are considered in the respective decision models. The decision models can mimic human behaviors by interacting with surrounding drivers, extract information from the interaction and generate the optimal control strategies, e.g. when and how to change the lane \cite{zhang2019game,yu2018human}. One advantage of the game-theoretical approaches is the consideration of the mutual influence of traffic participants, which can increase the reliability of decision-making. However, the dimension of the game can be highly increased by involving more participants and the high dimensionality of the coupled game system may result in high computational complexity.

\textbf{\textit{2.3 Fuzzy Logic Control}}: 
Similar to PID controller, Fuzzy logic control doesn’t require the mathematical model of the plant allowing the controller to adequately deal with nonlinear vehicle dynamics. Another benefit is their humanoid control actions because of the human-like rules. Using membership functions, the input variables are translated into linguistic variables. The controller's output is determined by fuzzy rules that take the form of "if-then" statements. \cite{cai2009intelligent} presents a neuro-fuzzy controller with the aim to regulate the speed in order to maintain a safe distance with respect to the vehicle in front. \cite{sun2019nested} designs a fuzzy feedback controller to optimize the parameters of membership functions and rules in order to track the reference trajectories under different driving conditions. However, parameter optimization is challenging and fuzzy inference rules with a lot of expert knowledge are also required for fuzzy logic control \cite{guo2012design}.

\textbf{\textit{2.4 Model Predictive Control}}: 
MPC is extremely popular for vehicle control, see longitudinal control \cite{ arefizadeh2018platooning, zhou2019distributed}, lateral control \cite{yu2018human}, and integrated control \cite{8885839}. The principle of MPC is to find a predictive motion solution over a longer horizon period by solving the problem at each sample time and applying the first sequence of actions. In this way, MPC simulates a receding horizon control and changes the solution set to remain accurate to upcoming information \cite{nobe2001overview}. \cite{kim2014model} proposes an MPC-based path tracking controller that incorporates the dynamic characteristics of the steering actuation system to ensure accurate and smooth tracking. The main advantage of MPC algorithms is their ability to consider multiple performance criteria of control efficiency, ride comfort, fuel consumption, and their constraint handling capability on vehicles’ physical limits and safety.  However, they are still inadequate for non-convex and high-complexity issues. Excessive computing difficulties may impede their real-time applications.

\textbf{\textit{2.5 Sliding Mode Control-based Approaches}}: 
SMC offers the capacity to adapt to unknown disturbances and matched uncertainties. A series of path following controllers based on SMC is proposed in \cite{wu2019path, guo2013adaptive} and simulation results show that the SMC controllers are robust to disturbances and provide a proper path tracking performance.  However, the model uncertainties and the disturbances are time-varying in the realistic scenario and the model accuracy greatly influences the control performance. The control performance may be degraded due to the modeling errors \cite{rausch2017learning}.

\textbf{\textit{2.6 Linear Parameter Varying Control}}: 
The LPV controller is a linear controller and has been designed together with predictive control for lateral control \cite{ganzelmeier2001robustness,choi2000design} and integrated system control \cite{gaspar2005design}. This method requires advanced knowledge of a plant model as well as real-time signals from all states during driving. A state observer is required because this is not provided by default.



\textbf{\textit{2.7 AI-guided Driving Policy Learning}}: 
Research on artificial intelligence algorithms is progressing rapidly because of the commonplace of big data. Compared to the traditional control systems, AI-guided vehicle systems do not require any system-level knowledge and have shown great potential to optimize nonlinear systems in complex and dynamic environments \cite{chen2017learning, dai2005approach, samak2011control}. Instead of designing explicit hand-engineered algorithms for lane detection, obstacle detection, path planning, and control law design separately, the AI-guided vehicle systems can combine all efforts within one framework and teach the system to perform well and generalize to new environments through learning \cite{nobe2001overview}. \cite{yu1995road} investigates a road-following system using reinforcement learning. The testing results show that the proposed algorithm can use previous driving experiences to learn how to drive in new environments and improve the road-following performance through online learning. \cite{wang2018reinforcement} uses Deep Q-Network (DQN) to train a vehicle agent to learn automated lane change behaviors. \cite{chae2017autonomous} presents a novel autonomous braking system that uses deep reinforcement learning to intelligently manage the vehicle's velocity when a potential collision is announced. \cite{naranjo2006acc+} investigates an end-to-end controller based on a convolutional neural network (CNN) to provide steering commands without engineering each autopilot component. The AI-guided control strategies are very powerful and their capacity to generalize over a variety of similar scenarios make them fit for minor deviations in the driving conditions \cite{samak2011control}. However, safety validation of these AI-guided systems is very challenging due to the opaque nature of the methods and there is no explanation for failure can be given\cite{smc_30}. In addition, the need for training data may hinder the research of AI-guided systems.

The classic PID and sliding mode control method may fail to adapt to complex environment and unknown disturbances. The MPC and LQR are based on precise mathematical models, the uncertain and nonlinear mathematical model of the vehicle during real-world driving may degrade the control performance, especially in extreme maneuverings. The fuzzy rules of the fuzzy logic systems are based on experience, and there are no qualitative rules to refer to, making them challenging to use in engineering applications. Due to the high dimensionality of the coupled game system, the design of game theory-based control strategies is challenging. The AI-based method requires significant amount of off-line computation and training and more study into interpretability and functional safety validation methodologies for AI-driven cars is needed\cite{smc_29}.



\subsubsection{\textbf{Validation Process}}
To verify vehicle motion control algorithms, a series of testing should be designed for control strategy validation. In terms of testing patterns, the validation type can be divided into simulation studies and experimental tests. Testing in the actual world can be costly in terms of time, labor, and money. Simulation studies, in contrast, are much less expensive, faster, more adaptable and can be used to create scenarios that are difficult to replicate in real life \cite{guo2012design, wang2018reinforcement}. Simulation has become a more dominating approach with the increased accuracy and speed of simulation tool. National instruments' LabVIEW, which is a graphical computing platform, is widely used in the simulation program for testing and measurement \cite{arifin2022steering}. To model vehicle dynamics, the commercial tools Carsim \cite{kim2014model,rausch2017learning,kim2011control} with ADAMS \cite{sun2019nested}, CARLA \cite{del2021autonomous}, PreScan \cite{chae2017autonomous} and Matlab/Simulink \cite{chebly2019coupled} have been utilized by researchers for simulating car behavior.  SCANeR Studio coupled with Matlab/Simulink is used to provide realistic driving conditions for testing of automated vehicle motion controllers \cite{chebly2019coupled}. Microscopic traffic simulation tools VISSIM 10.0 \cite{so2020automated} and AutonoVi-Sim \cite{best2018autonovi} are utilized for modelling traffic situation and implement automated vehicle control. It should be noticed that the model errors should be considered through the verification and validation process and an inaccurate model may result in infeasible evaluation performance.

Some researchers set simulation studies as a first step for performance validation and conduct experimental tests for further validation. In the literature, the experimental tests can be conducted by a small and lightweight vehicle \cite{system_2}, and an on-road vehicle \cite{peng2006robust, sun2019nested,arifin2022steering}. A small and lightweight vehicle is rugged and low-cost and can be carried by a single person for testing in various environmental conditions. In addition, the small and lightweight vehicle can travel at a high speed without the worry of injuring people and property. The main disadvantage is its small payload, which is insufficient to hold the computing power required for computing. On-road vehicles as Fig.  \ref{fig:system_fig_0} in contrast, can validate the control performance in diverse lighting and weather conditions, but the approval of testing such as ethical approval is needed.


%\begin{figure}[!tb]
%    \centering
%    \begin{minipage}{.21\textwidth}
%        \centering
%        \includegraphics[width=0.8\linewidth]{picture/methodology/control_robot.png}
%        \caption{A small and lightweight vehicle The proposed approach}
%        \label{fig:prob1_6_2}
%    \end{minipage}%
%    \begin{minipage}{0.24\textwidth}
%        \centering
%        \includegraphics[width=0.85\linewidth]{picture/methodology/control_car.png}
%        \caption{On-road test vehicle}
%        \label{fig:prob1_6_1}
%    \end{minipage}
%\end{figure}

\begin{figure}
\centering  %图片全局居中
\includegraphics[width=8.5cm]{picture/methodology/autonomous_cars.png}

\caption{The figure shows the appearance of autonomous vehicles. The left vehicle is the test autonomous platform of Xi'an Jiaotong University. The right vehicle is the autonomous mining truck at an open-pi mine in China.}
\label{fig:system_fig_0}
\end{figure}

%In terms of maneuver behaviors, the vehicle motion control strategies can be tested for lane keeping behavior and lane change behavior. Lane keeping and lane change are the two important operations that require and assess the ability and performance of vehicle motion functionalities. The goal of lane keeping is to execute automatic steering to keep the vehicle in the center of the road regardless of changes in traffic conditions. The control system for lane keeping, which involves longitudinal and lateral control, is usually designed to detect any variation between the controlled vehicle and the desirable path. For example, \cite{o1996vehicle} presents an $H_\infty$ lane keeping controller that can work for both curved and straight highways in the presence of uncertain road conditions. \cite{son2014robust} develops a state feedback controller to improve the lane keeping performance on curved roads. Lane changing is a maneuver that allows a fast car to pass a sluggish vehicle and may be seen all over the highway \cite{gaspar2005design,kim2011control,djoudi2020simulation}. Compared to the lane-keeping, lane-change is more challenging to control as its reliability highly relies on driving conditions, surrounding vehicles, traffic signals, and so on \cite{khodayari2010historical}.

%In respect of driving scenarios, the testing environment can be highways \cite{gaspar2005design,kumarawadu2006neuroadaptive}, an urban environment (e.g., local roads, and residential streets) \cite{peng2006robust,huang2017parameterized}, and other areas like parks, playgrounds, front yards, and backyards of a number of suburban homes, and heavily cluttered construction areas \cite{chae2017autonomous}.


==> body/methodology/detection.tex <==
\subsection{\textbf{Perception}}
Perception is a fundamental module for autonomous driving. This module provides surrounding environmental information to the ego-vehicle. As can be seen in Fig. \ref{fig:perception methodology}, perception is divided into localization, object detection, scene understanding, target prediction, and tracking.

\subsubsection{\textbf{Localization}}
Localization is the technology for the driving platform to obtain its own position and attitude. It is an important prerequisite for the planning and control \cite{survey_loca_2,survey_loca_15,local_3,survey_loca_7,survey_loca_8,survey_loca_11,survey_loca_12,survey_loca_5}. Currently, localization strategies are divided into four categories: Global Navigation Satellite System (GNSS) and Inertial Measurement Unit(IMU), visual Simultaneously Localization and Mapping (SLAM), LiDAR SLAM, and visual-LiDAR fusion based SLAM \cite{survey_loca_10,survey_loca_3}.

\textit{\textbf{1.1 GNSS and IMU:}} GNSS \cite{survey_loca_14} is an space-based radio navigation and localization system that can provide users with all-weather, three-dimensional coordinates, velocity and time information on the earth's surface or in near-earth space. IMU\cite{local_17} is composed of three-axis accelerometers and three-axis gyroscopes. By integrating the linear acceleration and angular acceleration from IMU, we can get the localization and posture of vehicles. The advantages of combining of GNSS and IMU are achieving all-weather and large coverage area, but the disadvantages are poor positioning accuracy and slow update frequency\cite{local_35,local_36}.

\textit{\textbf{1.2 Visual SLAM:}} Generally, visual localization analyse and match continuous image frames to obtain pose changes, it belongs to relative localization method. Visual localization algorithms are divided into three categories: monocular, multi-ocular and depth camera. The advantage of visual localization is that the cost of the camera is relatively low, and users would get the image information, without auxiliary equipment\cite{local_48,local_49}. Visual localization also have disadvantages. It is dependent on feature and light greatly. In the image processing, back-part optimization is particularly important. Back-end optimization adopts filter and graph optimization, based on filtering theory and nonlinear optimization theory\cite{local_24,local_25}.

The filter algorithm is based on Bayes' theorem. For autonomous vehicles, the car's sensors get real-time data as the vehicle moves from one position to the next. These data can be used in Bayes' theorem to estimate the probability of the vehicle's next location in the map. Various SLAM algorithms have been derived based on Bayes' theorem, including Extended Kalman Filter (EKF)\cite{local_57}, Unscented Kalman Filter (UKF)\cite{local_18}, Particle Filter (PF)\cite{local_23} and graph SLAM. EKF adds linearization steps, which is performed around the current estimate by first-order Taylor expansion, to the nonlinear model\cite{local_45, survey_loca_13}. The advantage of EKF is that it can process nonlinear models and provide a good reference for closed loop\cite{survey_loca_16}. However, EKF also has weakness, the localization effect get worse as the map becomes larger and more complex \cite{local_26,local_27}. UKF is a nonlinear Kalman filter that does not need to deal with Jacobian matrix. PF relies on particles that can sample states according to their probability density. Some methods are developed to incorporate PF in SLAM, such as DP-SLAM\cite{local_19}, DP-SLAM2.0\cite{local_47} and FastSLAM\cite{local_29}. The basic principle of graph SLAM is to use a matrix containing vehicle state (posture) and map landmark information to find the optimal trajectory of the vehicle in the map \cite{local_51}. As graph SLAM contains the vehicle attitude and the matrix structure of the ground mark in the map, its calculation cost is high \cite{survey_loca_4}.

\textit{\textbf{1.3 LiDAR SLAM:}} LiDAR SLAM uses LiDAR to detect the relative distance between the profile of objects and the carrier. It is not sensitive to light, thus the generated horizontal view is large and precise. However, the generated vertical view's resolution is low. The sparse point cloud can only represent part of the environment features, and it is seriously disturbed by the weather\cite{local_50}. In terms of localization, laser localization is similar to visual localization, the key points of environment features are registered with the map, so as to locate the vehicle in the map. Before localization, LiDAR SLAM needs to collect environment point cloud information in the local area of the prior point cloud map\cite{local_21,local_22,local_31}, then LiDAR SLAM assumes that the current vehicle is located in the area of a particular location. Furthermore, a single frame is obtained by vehicular laser radar point cloud data, LiDAR SLAM matches it with a prior point cloud. If no great changes of environment occurs, LiDAR SLAM can find the best matching sites in the prior point cloud. The coordinates corresponding to this point are the relative coordinates of the vehicle. 

At present, there are several relevant algorithms for LiDAR SLAM, such as Normal Distribution Transformation (NDT) \cite{local_54,local_53} and Iterative Nearest Point (ICP) \cite{local_28,local_29,local_30}. These algorithms evaluate the registration of prior point cloud image and current point cloud data, and then make the matching sites converge through continuous iteration to obtain the optimal result. ICP algorithm can obtain very precise registration effect \cite{survey_loca_4}, without the need for segmentation and feature extraction of the processed point set. However, in the process of searching the corresponding point, the calculation is very large. In addition, ICP is based on the nearest Euclidean point as the corresponding point which may lead to errors.  NDT can directly carry out registration and calculation without passing the characteristics of corresponding points, so the calculation speed is fast. Grid parameters are important in NDT. It needs careful selection of grid parameters, as too large grid parameters lead to low accuracy, while too small grid parameters lead to high memory.

The ICP is the most common method in point cloud registration. A few methods \cite{local_32, local_33} analyzed NDT to replace the ICP. The point representation is converted to a grid, and the mean and covariance of the grid are obtained for matching and comparison in NDT. NDT is proven to be more robust than point-to-point ICP matching. \cite{local_34} proposed an improved version of 3D-NDT matching. \cite{local_56} enhanced the NDT strategy with road marker matching. \cite{local_57} developed a Monte Carlo Localization (MCL) method based on NDT, based on offline static maps and constantly updated short-term maps.

\textit{\textbf{1.4 Visual-LiDAR Fusion Based SLAM:}}In order to solve the shortcomings of visual SLAM and LiDAR SLAM, some researchers believe that the fusion of the two can overcome the shortcomings. In the early stage of research, many studies applied the classical method based on EKF to study the fusion of visual SLAM and LiDAR SLAM\cite{local_20,local_52}. However, this method does not really fuse the data of the two sensors, it only adopts the switching mechanism between the working modes of two sensors. Later, many scholars fused LiDAR data into visual SLAM, using the optimization algorithm of deep completion and Bundle Adjustment (BA). Sun et al. \cite{local_39} proposed an EKF expression based on data association to improve the accuracy of SLAM. Xu et al. \cite{local_40} proposed a SLAM method based on the fusion of EKF RGB-D camera and LiDAR to deal with camera matching failure. When camera matching fails, LiDAR is used to supplement camera 3D point cloud data and generates maps. 

Guillen et al.\cite{local_41} compared the performance of various SLAM algorithms based on EKF on a visual camera integrated with IMU. Existing research results show that adding 2D LiDAR into SLAM system to generate 2.5D map can improve the accuracy of robot pose estimation. However, these feature detection methods, which are independent of measurement space, are still loosely coupled\cite{local_39}. There still exists a gap for the research on tightly coupled EKF vision and LiDAR fusion algorithm. Visual SLAM often ineffectively extracts depth information from feature points, however, that is what LiDAR is good at. In order to overcome the deficiency of single Visual SLAM, researchers tried to fuse LiDAR data into the visual SLAM method. Graeter et al.\cite{local_42} used LiDAR to measure the scene depth, and applied BA optimization algorithm based on visual key frames, to estimate state and construct map based on point cloud projection video frames. Shin et al.\cite{local_43} proposed a method of using LiDAR to obtain sparse depth point clouds for visual SLAM, but since the resolution of the camera is much higher than that of LiDAR, this method will lead to a large number of pixels without depth information. For this reason, De Silva et al. .\cite{local_44} proposed a method to solve the resolution matching problem, Gaussian regression was used to interpolate the missing depth values after calculating the geometric transformation between the two sensors. This approach uses LiDAR to directly initialize the features detected in the image in the same way as using RGB-D sensors.

\subsubsection{\textbf{Object Detection}} The purpose of object detection is to detect the static and dynamic targets in the field of view of the sensors. The results of some detection tasks can be seen in Fig. \ref{fig:3D Object Detection}.

\textit{\textbf{2.1 Lane Detection}} Lane Detection is to recognise the lane in the views of sensors, to assist driving. For universal process, it involves three sections, including the image pre-processing, lane detection and tracking. The propose of image pre-processing, such as Region of Interest (RoI) extraction, inverse perspective mapping, and segmentation, is to reduce the computing cost and eliminate noise. The methods of lane detection and tracking can be divided into the Computer Vision based (CV-based) method and learning-based method.

CV-based methods in lane detection are broadly utilized nowadays, primarily because of its light computing cost and easy reproduction. A morphological top-hat transform is utilized to eliminate the irrelevant objects in the field \cite{object_detection_lane_detection_1, object_detection_lane_detection_2}. After that, the Hough transform is applied to extract the edge pixel of the image and construct the straight lines. However, the disadvantage is that it is hard to detect the curve lines, so a number of researchers have introduced some effective methods on the Hough transform \cite{object_detection_lane_detection_1, object_detection_lane_detection_2}. Some other lines estimation approaches involve the Gaussian Mixture Models (GMM) \cite{object_detection_lane_detection_3}, Random Sample Consensus (RANSAC) \cite{object_detection_lane_detection_4}, Kalman filter \cite{object_detection_lane_detection_5, object_detection_lane_detection_6} in complex scenes.

Learning-based methods can be deployed on abundant scenes but they need a great deal of data to train the network with plenty of parameters. Some researchers attempt to design novel structures such as multiple sub-headers \cite{object_detection_lane_detection_7}, \cite{object_detection_lane_detection_8} and \cite{object_detection_lane_detection_9} to improve the lane detection performance. A light weight model \cite{object_detection_lane_detection_10} and implement method \cite{object_detection_lane_detection_11} are able to relief the high computing cost of the deep neural networks.

\textit{\textbf{2.2 Driving Regions Detection:}} Driving regions detection increases the obstacle information comparing to the lane detection, which offers the base information to obstacle avoidance function and path planning task. We also category this task into the CV-based and learning-based approaches.

Driving regions detection can be converted to lane detection when the road surface is not obscured by obstacles. Otherwise, it can be seen as the combination of lane detection and 2D target detection. When considering driving regions detection as an independent task, it needs to distinguish the road pixel from targets and non-driving regions. The color histogram can meet the requirement and some researchers develop the methods on color \cite{object_detection_driving_region_1} and efficiency \cite{object_detection_driving_region_2} to tackle the poor performance on color varying and low effect of it. Region growth methods \cite{object_detection_driving_region_3, chenlong_tvt} are more robust than the color histogram methods. 

The learning-based methods in driving regions detection are similar with the image segmentation. For machine learning algorithms, features such as the RGB color, Walsh Hadamard , Histogram of Oriented Gridients (HOG), Local Binary Pattern (LBP), Haar, LUV channel, can be extracted by the feature extractors and the classification header, such as Support Vector Machine (SVM), Conditional Random Field (CRF), to obtain the final results. The deep neural network can replace the feature extractors and some improvements, such as employing the large visual regions convolutional kernels \cite{object_detection_driving_region_4}, connection by multiple layers \cite{object_detection_driving_region_5}, to achieve competitive performance. We recommend readers to explore more tricks and novel structures from the research on segmentation task.

\textit{\textbf{2.3 Traffic Sign Detection:}} Traffic signs contain plenty of crucial traffic information, such as road conditions, speed limitations, driving behavior restrictions and other information. We also divide it into CV-based approaches and learning-based approaches. 

For CV-based detection approaches, the conditions for the approximate color composition of traffic signs in a specific region (in a certain country or city) are similar. In the relatively simple original image, better results can be obtained by threshold separation of specific colors, which can be obtained by adopting the color space distribution, segmentation head and the SVM classifier \cite{traffic_sign_1, traffic_sign_2}. Some research develops the methods by introducing extra color channel \cite{traffic_sign_3}, such as NRGB model, the dynamic color threshold \cite{traffic_sign_4}, probability model \cite{traffic_sign_5}, and edge information \cite{traffic_sign_6}. However these approaches are hard to solve the problem caused by the illumination, fading, occlusion and bad weather. Some researchers tried to utilize the appearance \cite{traffic_sign_7}, Hough transform on the triangle \cite{traffic_sign_8}, circular traffic signs \cite{traffic_sign_9} or a coding gradient detection method \cite{traffic_sign_10}, to handle occlusion and conjunction. The shape-based detection method can solve the problem of in-stable result caused by color change, but it has little capability to overcome the problem caused by occlusion and deformation.

The traffic sign recognition algorithm based on machine learning usually uses the sliding window method to traverse the given traffic sign image such as \cite{traffic_sign_11, traffic_sign_12}. \cite{traffic_sign_12} proposed a variant histogram feature of gradient direction, and trained single classifier to detect traffic signs through extreme learning machine. With the continuous research of deep learning algorithm, more and more scholars use deep learning algorithm to detect traffic signs. Readers can regard this classification method as handing feature extraction, including pre-processing and classification \cite{traffic_sign_13, traffic_sign_14, traffic_sign_15, traffic_sign_16, traffic_sign_17}. To extract deeper information, the YOLOv3 \cite{traffic_sign_13} backbone, integrated Space Pyramid Pooling (SPP) layer \cite{traffic_sign_14}, cascaded RCNN network \cite{traffic_sign_15}, depth separable convolution \cite{traffic_sign_16} and clipping strategy \cite{traffic_sign_17} are introduced to achieve the detection accuracy and high inference speed. The deep learning method has a good tolerance for the change of target color and shape, however the problem lies in the huge training data and high requirements for hardware.

\textit{\textbf{2.4 Visual-based 3D Object Detection:}} Visual-based 3D object detection refers to the process of acquiring 3D information (location, dimension and rotation) about all targets in the field from the image. We divided this section into the monocular-based detection and stereo-based detection.

\textit{\textbf{2.4.1 Monocular 3D Object Detection:}} Monocular 3D object detection is widely researched and the accuracy has been improving in recent years. Direct classification and regression methods \cite{CenterNet, M3DRPN}, inheriting from 2D object detection networks \cite{FasterRCNN, M3DRPN}, have straightforward structures but perform poorly due to the ill-posed problem in recovering 3D attributions from single image. There are two main kinds of strategies to solve the shortcoming. 1) some groups \cite{Deep3DBox, MonoPair, Monet3D} introduce the geometric connections between 3D boxes and projected 2D boxes. For example, GS3D \cite{GS3D} decouples the objects into several parts to analyze the surface attributes and mapping relations. Monopair \cite{MonoPair} and Monet3D \cite{Monet3D} consider the relationships between a target and its two nearest targets. 2) When regressing the 3D bounding boxes on the training stage, networks can take into account the local or full depth map \cite{CaDDN, DDMP3D} from stereo vision or LiDAR data. CaDDN \cite{CaDDN} provides a fully differentiable end-to-end approach for combining depth estimation and object detection. DDMP3D \cite{DDMP3D} uses the feature representation of context and depth estimation to achieve promising performance. In addition, Joint3D \cite{Joint3D} and Kinematic3D \cite{Kinematic3D} utilize successive frames as input for training and testing, attempting to analyze the 3D results of each frame independently.

\textit{\textbf{2.4.2 Stereo 3D Object Detection:}} Stereo 3D object detection approaches\cite{Stereo-RCNN, OC-Stereo, ZoomNet, YOLOStereo3D, Disp-RCNN, stereo_system} are inspired by the parallax analysis of binocular vision. In a common scene, the precise depth value can be reckoned through the distance of the binocular centers and the associated pair of pixels. However, this type of method is time-consuming and needs a great deal of computing resource. Disp-RCNN \cite{Disp-RCNN}, OC-Stereo \cite{OC-Stereo}, and ZoomNet \cite{ZoomNet} add segmentation modules paired images from stereo cameras to induce accurate association. YOLOStereo3D \cite{YOLOStereo3D} provides a light-weight model, outperforms a great number of stereo methods based on the complicated disparity convolution operations, and significantly reduces the length of training and testing time.

\begin{figure*}
\centering  %图片全局居中
\includegraphics[width=17cm]{picture/methodology/detection-structure.png}

\caption{The structure of perception methodology}
\label{fig:perception methodology}
\end{figure*}

\textit{\textbf{2.5 LiDAR-based 3D Object Detection:}} LiDAR-based 3D object detection detect targets 3D information from point clouds data captured by LiDARs. We divided this section into the Voxel-wise detection and Point-wise detection.

\textit{\textbf{2.5.1 Voxel-wise Object Detection:}} Voxel-wise object detection methods represent the point cloud features in the Birds Eyes View based (BEV-based) object detection. BEV map is obtained by gridding the LiDAR point cloud and projecting it to the X-Y coordinate plane. After gridding, the resolution can be set manually. Each grid corresponds to one pixel in the feature image or feature vector. As a result, the higher the resolution is, the higher accuracy and computational cost will be, and vice versa.

The structural design of this type of detection network evolves from point cloud segmentation frameworks, such as PointNet \cite{PointNet} and PointNet++ \cite{PointNet++}, which fit the detection task at the input or output side, and its overall architecture needs to balance performance and efficiency. Taking the classic VoxelNet \cite{voxelnet} and PointPillar \cite{pointpillars} as examples, VoxelNet first divides the 3D point cloud into a certain number of voxels, then normalizes the point cloud, and subsequently applies local feature extraction using several Voxel Feature Encoding (VFE) layers to each non-empty voxel. The voxel-wise features are further abstracted by 3D convolutional middle layers (increasing the receptive field and learning the geometric spatial representation), and finally, the object is detected and classified using a Region Proposal Network (RPN) with position regression.

\textit{\textbf{2.5.2 Point-wise Object Detection:}} Point-wise object detection such as \cite{pointrcnn, pvrcnn}, can reduce point cloud information loss without using voxel gridding or sampling. This type of algorithm is also inspired by PointNet. Point-RCNN \cite{pointrcnn} is a two-stage point cloud detection framework. Candidate frames are generated at the first stage, during which semantic segmentation is applied, differentiating between foreground and background. Frames are bounded with every filtered foreground segment to obtain N candidate frames. In the second stage, every candidate frame is rotated and transformed to a proper position, and they will be scored and optimized, resulting in the final result. VoteNet \cite{votenet} is a novel point cloud detection strategy, which extends 2D structures to 3D framework to establish a generic detection framework for point clouds. It basically follows the PointNet++ structure to reduce the information loss in point cloud transformation. VoteNet adopts a simple voting mechanism inspired by the Hough transform to locate the targets' centers instead of the surface, compared with the other traditional point cloud processing networks. The position with the highest votes is determined to the closet to the center. It achieves SOTA 3D target detection performance in both SUN RGB-D \cite{sunrgbd} and ScanNet \cite{scannet} datasets.

\textit{\textbf{2.6 Fusion-based 3D Object Detection:}} LiDARs, radars and cameras are widely deployed in the autonomous driving vehicles for perception task. The combination of these sensors can make the vehicles be robust and full-time detection. However, not all the fusion-based methods outperform the uni-model networks nowadays. There are three reasons for the disadvantage of fusion-based methods. 1) It is challenging for network to fill the gap among different data from multiple kinds of sensors; 2) The system and measurement errors are difficult to eliminate for multiple-model networks; 3)The fusion-based network require more learn-able parameters and that puts a challenge to the network to fit the data. Most researchers propose solutions to handle these difficulties and achieve some competitive outcomes. In this section, we category the fusion-based objection detection task based on the sensors.

\textit{\textbf{2.6.1 Camera and LiDAR:}} Camera and LiDAR are two types of crucial sensors for autonomous driving. The parallel approaches mean the structure share the extracted features after the independent backbones. The sequential methods indict one type of the data is extracted by the other.

MV3D \cite{MV3D} and AVOD \cite{AVOD} utilize the shared 3D anchors on the point cloud and the corresponding images. ContFuse \cite{ContFuse} and MMF \cite{MMF} adopt tightly-coupled fusion approaches with a consecutive fusion layer. 3D-CVF \cote{3D-CVF} introduces a cross-view spatial feature fusion method to fuse the images and point clouds. In addition, EPNet \cite{EPNet} focuses on the point cloud system and projects the images on it with point based strategy on the geometric space.

Compared with parallel approaches, sequential methods are easier because it does not need to consider the joint structure to reduce the gaps between two types data. F-PointNet \cite{F-PointNet} and F-ConvNet \cite{F-ConvNet} attempt to reduce the searching areas by generating 3D bounding boxes within 2D results. PointPainting \cite{PointPainting} outputs semantic information and projects each point on the corresponding point to improve the 3D object detection. CLOCs \cite{CLOCs} fuses the data after the independent extractors and achieve competing result on KITTI \cite{dataset_KITTI}. DVF \cite{DVF} adopts the 2D truth and the point cloud to avoid noise from two tpyes of data.

\textit{\textbf{2.6.2 Camera and Radar:}} Combining the images and data from Radars can effectively reduce the cost and maintain the accuracy. Common methods, such as \cite{object_detection_fusion_3D_cameraradar_1, object_detection_fusion_3D_cameraradar_2}, project radar detection results to the image space and utilize them to boost the object detection accuracy for distant objects. CRF-Net \cite{object_detection_fusion_3D_cameraradar_3} develops the method with vertical presentation.

\textit{\textbf{2.6.3 LiDAR and Radar:}} These type of fusion focuses on the extremely harsh weather condition and distinct targets. RadarNet \cite{RadarNet} fuses radar and LiDAR data via a novel-based early fusion approach. It leverages the radar' long sensing range via an attention-based fusion. MVDNet \cite{MVDNet} generates proposals from two sensors and then fuses region-wise features between multi-modal sensor streams to improve final detection results. ST-MVDNet \cite{ST-MVDNet} develops the structure by enforcing output consistency between a Teacher network and a Student network, and introducing missing modalities to tackle the degeneration problem when one type of data is missing.

\textit{\textbf{2.6.4 Camera, LiDAR and Radar:}} In this fusion type, researchers attempt to design a robust perception system in different weather conditions. \cite{lidar_camera_radar} obtains object detection outputs with a PointNet \cite{PointNet} architecture by projecting the images onto the point cloud directly. Parallel to the previous frame, the point cloud from radar is processed to predict velocity which is then associated with the final detection output. RVF-Net \cite{RVF-Net} fuses all of the data on the input procedure and achieves satisfying results on the nuScenes \cite{nuScenes} data set. 

\textit{\textbf{2.6.5 Others:}} Ultrasonic radar judges the distance of obstacles through the time of sound transmission in the air, and the accuracy can achieves centimeter scale within 5 meters. This sensor is mostly used in autonomous parking scenes. Infrared camera with infrared lamp can capture the infrared spectral characteristics to achieve the effect of night vision imaging. The research on event cameras is one of the hot topics nowadays. Event cameras process data based on pipeline timestamps, rather than processing individual pixels in a frame plane. Because the data has the nature of time sequence, the traditional network structure can not process the data, so how to fuse with other sensors will be one of the research points in the future.

\begin{figure}
\centering  %图片全局居中
\includegraphics[width=9cm]{picture/methodology/Perception_detection.png}

\caption{The crucial tasks in the object detection for autonomous driving. The top-left, top-right, bottom-left, bottom-right figure represents the lane detection, drivable region, traffic sign detection and 3D object detection.}
\label{fig:3D Object Detection}
\end{figure}

In summary, Comparing the 3D object detection results of multiple methodologies on KITTI \cite{dataset_KITTI} /unScenes \cite{nuScenes} data. We summarize: 1) The visual and fusion 3D object detection attracts more and more researchers recently; 2) The point-wise LiDAR-based 3D object detection methods achieve more accurate results but they are time-consuming and hard to regress during the training step. Researchers always estimate their approaches on datasets, for example KITTI, nuScene, Waymo \cite{Waymo}, Cityscape \cite{dataset_seg_CityScape}. To deploy the detection models on intelligent platforms, researchers pay more attention on the sensors deployment (cameras, LiDARs, lasers), calibration, synchronization and annotation. There are multi difficulties: 1) the huge gap between the academic and industrial areas; 2) the limited computing chip; 3) the robust requirements on real world.



\subsubsection{\textbf{Scene Understanding}}
We define the scene understanding in our paper as the multiple outputs for each pixel or point instead of each target. In this section, we divide into three sub sections, segmentation, depth and flow estimation. We only focus on the academic research and applications in the autonomous driving areas.

\textit{\textbf{3.1 Segmentation in Autonomous Driving:}}
The target of semantic segmentation is to partition a scene into several meaningful parts, usually by labeling each pixel in the image with semantics (semantic segmentation) , by simultaneously detecting objects and distinguish each pixel from each object (instance segmentation), or by combining semantic and instance segmentation (panoptic segmentation)\cite{survey_dynamic_20}. The segmentation is one of the crucial tasks in computer vision and researchers evaluate their models on ADE20K \cite{dataset_seg_ADE20K}, Pascal-VOC \cite{dataset_seg_VOC}, CityScape \cite{dataset_seg_CityScape}, etc. However, in autonomous driving scenarios, the classic 3D CV area, it is hard to complete the perception task independently. It is usually involved into the lane detection, driving region detection, visual interface module or combined with point clouds to provide semantic information. We will briefly introduce the general background based on segmentation, and then highlight segmentation research at autonomous driving \cite{smc_31}.

\textit{\textbf{3.1.1 Semantic Segmentation:}} Fully Convolutional Network (FCN) \cite{scene_FCN} is a popular structure for semantic segmentation which adopts convolutional layers to recover the size of output maps. Some work extend FCN by introducing an improved encoder-decoder \cite{scene_segnet}, the dilated convolutions \cite{scene_dilated}, CRFs \cite{scene_DeepLabv1}, atrous spatial pyramid pooling(ASPP) \cite{scene_DeepLabv2}, residual connection \cite{scene_RefineNet}, pyramid pooling module \cite{scene_PSP} and improved ASPP \cite{scene_DeepLabv3}. In addition, above approaches attend to fixed, square context regions because of the pooling and dilation convolution operations. Relational context methods \cite{scene_OCRNet, scene_OCNet} extract the relationship between pixels. Some networks \cite{scene_UNet, scene_Unet++} pursue the high resolution by channel concatenation and skip connection especially in the medical field. In autonomous driving, the semantic segmentation networks may be familiar with the common structures, and researchers should pay more attention to the special categories, occlusion, and evaluate their models on road scenarios data sets \cite{dataset_seg_CityScape, dataset_KITTI, dataset_seg_Mapillary_Vistas}. To achieve SOTA results on data sets, researcher introduce the multiple scale attention mechanism \cite{scene_multi_scale_attention}, boundary-aware segmentation module \cite{scene_boundary_aware_segmentation}. Besides, some research focus on the targets' attributes on roads like considering the intrinsic relevance among the cross class objects \cite{scene_intrinsic_relevance} or semi-supervised segmentation mechanism because of the lack of labeled data on autonomous driving scenarios such as \cite{scene_Naive_student}, \cite{scene_unsupervised_domain}, \cite{scene_Warp_Refine_Propagation}.


\textit{\textbf{3.1.2 Instance Segmentation:}} Instance segmentation is to predict a mask and its corresponding category for each object instance. Early methods \cite{scene_Mask_RCNN, scene_HTC} design architectures to realize both object detection and segmentation missions. Mask-RCNN \cite{scene_Mask_RCNN} extends Faster-RCNN to identify each pixel's category with binary segmentation and pools image features from Region of Interest (RoI) following a Region Proposal Network (RPN). HTC \cite{scene_HTC} proposes an interleaved way to localize boxes and mask pixels. Some researchers develop the base structure by introducing a coefficients network \cite{scene_Explicit}, the IoU score for each mask, and shape priors to refine predictions. Similar with the 2D object detection methods, Some methods \cite{scene_Blendmask, scene_Centermask, scene_Embedmask, scene_Mask_encoding} replace the detectors with
the one-stage structures. Some methods \cite{scene_Solov2, scene_Ssap} attempt to avoid the effect of detection and achieve remarkable performances. To achieve competitive results on autonomous driving data set such as segmentation, researchers focus on the geometric information on 3D space \cite{scene_Polytransform}, boundary recognition \cite{scene_Look_closer_to_segment_better}, combining the semantic segmentation (panoptic segmentation) \cite{scene_Scaling_wide} or intruding multiple frames (video-base) \cite{scene_Naive_student}.

\textit{\textbf{3.1.3 Panoptic Segmentation:}} Panoptic segmentation is proposed to unify pixel-level and instance-level semantic segmentation \cite{scene_Panoptic_segmentation, scene_Panoptic_segmentation_joint}, and some methods \cite{scene_Panoptic_FPN, scene_UPNet} design different branches to regress the semantic and instance results. Panoptic-FCN \cite{scene_Panoptic_FCN} aims to represent and predict foreground things and background stuff in a unified fully convolutional pipeline. Panoptic SegFormer \cite{scene_Panoptic_SegFormer} introduces a concise and effective framework for panoptic segmentation with transformers. For autonomous driving scenarios, TASC \cite{scene_TASC} proposes a new differentiable approach to reduce the gap between the two sub-tasks during training. Axial-DeepLab \cite{scene_Axial_deeplab} builds a stand-alone attention model with global receptive field and a position-sensitive attention layer to capture the positional information with low computational cost. Besides, researchers address the multiple scales on roads by introducing a novel crop-aware bounding box regression loss and a sample approach \cite{scene_Improving_panoptic_segmentation}, and capture the targets' boundary by a combinatorial optimization strategy. These methods achieve competitive results on the task of CityScape \cite{dataset_seg_CityScape} or Mapillary Vistas \cite{dataset_seg_Mapillary_Vistas}.

\textit{\textbf{3.2 Depth Estimation in Autonomous Driving:}}
This type of task is to present the depth information on the camera plane, which is an effective way to enhance the visual-based 3D object detection and a potential bridge to connect the LiDAR and camera.

%{\romannumeral1} \textit{Depth Completion:}
The Depth Completion task is a sub-problem of depth estimation \cite{scene_Depth_completion, smc_5}. In the sparse-to-dense depth completion problem, researchers infer the dense depth map of a 3D scene from a sparse depth map by computational methods or multiple data from sensors. The main difficulties include: 1) the irregularly spaced pattern in the sparse depth, 2) the fusion methods for multiple sensor modalities (optional), 3) the lack of dense pixel-level ground truth for some data and real world (optional).

%Depth-only methods \cite{scene_Depth_completion, scene_Sparse_and_dense_data_with_cnns, scene_Hms_net, scene_Uncertainty_aware_cnns} only take sparse depth as input and output the dense depth map. Although these learning based methods outperform the model based methods, they are computationally expensive and unable to recover the accurate depth value because of the lack of semantic cues from visual data. 

%Multiple data methods supplement extra information into the input and take advantage of complementary features from other modalities. The image can provide rich semantic cues or as the guidance to produce dense maps by self-supervised methods \cite{scene_Dfinenet, scene_Confidence_propagation, scene_Uncertainty_driven_loss, scene_Self_supervised_sparse_to_dense, scene_Geometry_Aware_Embedding, scene_Adaptive_context_aware, scene_SemAttNet, scene_Dynamic_spatial_propagation}. \cite{scene_Self_supervised_sparse_to_dense} utilize a self-supervised network and a pose estimation to recover the scale. Besides, Dfinenet \cite{scene_Dfinenet} supervises the depth and the relative pose between the consecutive frames. \cite{scene_From_depth_what_can_you_see} develops the depth-only methods, which adds an image reconstruction module from sparse depth as an auxiliary task and supervised by the unlabelled gray scale images. \cite{scene_Uncertainty_driven_loss} considers the uneven distribution characteristics in the sparse depth map and the accumulated outliers in the synthesized ground truth. \cite{scene_Depth_normal_constraints, scene_Geometry_Aware_Embedding} introduce the space constricts on the network to guide the dense map output. \cite{scene_Adaptive_context_aware} adopts the graph propagation to obtain the observed context on image plane. \cite{scene_SemAttNet, scene_Dynamic_spatial_propagation} achieve competitive results on KITTI \cite{dataset_KITTI} and NYUv2 \cite{dataset_NYUv2} (indoor) datasets by looking and thinking twice mechanism \cite{scene_RigNet}, attention module \cite{scene_SemAttNet} and non-linear propagation mode \cite{scene_Dynamic_spatial_propagation}.


%{\romannumeral2} \textit{Depth Estimation:}
Depth Estimation is the task of measuring the distance of each pixel relative to the camera. The depth value is extracted from either monocular or stereo images with supervised (the dense map obtained by depth completion) \cite{scene_Indoor_scene_structure_analysis, scene_Depth_map_prediction}, unsupervised \cite{scene_Semi_supervised_deep_learning, scene_Unsupervised_cnn}, LiDAR guidance \cite{scene_Refinedmpl} or stereo computing\cite{scene_Deepstereo, scene_NASD}. Some approaches introduce the CRF module\cite{scene_Multi_scale_continuous_crfs}, multi-tasks structure \cite{scene_Pad_Net}, global extractor\cite{scene_Transformer_based_attention} or the piece-wise planarity prior \cite{scene_P3Depth} to achieve competitive performances in popular benchmarks such as KITTI \cite{dataset_KITTI} and NYUv2 \cite{dataset_NYUv2}. Models are typically evaluated according to a RMS metric \cite{dataset_KITTI}.

For outdoor monocular depth estimation, DORN \cite{scene_DORN} adopts a multi-scale network structure to capture the contextual information. MultiDepth \cite{scene_Multidepth} makes use of depth interval classification as an auxiliary task. HGR \cite{scene_HGR} proposes a hierarchical guidance and regularization learning framework to estimate the depth. SDNet \cite{scene_SDNet} and PAP \cite{scene_Pattern_affinitive_propagation_across_depth} improves the results by utilizing dual independent estimation head involving depth and semantics. \cite{scene_From_big_to_small} designs a novel structure which includes local planar guidance layers at multiple stages. \cite{scene_Enforcing_geometric_constraints} uses the geometric constraints of normal directions determined by randomly sampled three points to improve the depth prediction accuracy. BANet\cite{scene_BANet} introduces bidirectional attention modules which adopt the feed-forward feature maps and incorporate the global information to eliminate ambiguity. Unsupervised methods attract plenty researchers\cite{scene_3D_packing, scene_monodepth2, scene_Unsupervised_monocular_depth_estimation}, which could reduce the requirements on the labeled data and eliminate the over-fit problem. In addition, the pure monocular depth estimation only obtain the relative depth value because of the ill-posed problem, and the stereo guidance methods could obtain the absolute depth value. Some methods \cite{scene_Transformers_in_Self_Supervised_Monocular_Depth_Estimation, scene_DepthFormer} introduce the Transformer structures to achieve the competitive results. The stereo depth estimation methods can be found at the stereo disparity estimation task.


\textit{\textbf{3.3 Flow Estimation in Autonomous Driving}}: Similar with the segmentation and depth estimation tasks, the flow estimation focuses on the image plane and it presents the pixel movement during a data frame. It attracts interest nowadays and its research can be used in the event camera methods.

\textit{\textbf{3.3.1 Optical Flow Estimation:}}
Optical flow refers the pixels' movement on the image system including two directions, the horizontal and vertical. Similar with unsupervised video-based depth estimation, the pixel motion \cite{scene_flownet} can be deduced by minimizing differences between the target and source images. SPyNet \cite{scene_spynet} proposes a lightweight framework which adopts classical spatial-pyramid formulation for optical flow estimation. In addition, it attempts to estimate large displacement movement and accurate sub-pixel flow. PWC-Net \cite{scene_pwcnet} includes three sub-nets, the feature pyramid extractor, warping layer and cost volume layer, to improve the quality of optical flow. 

\textit{\textbf{3.3.2 Scene Flow Estimation:}} Scene flow estimation indicates a 3-dimensional movement field which can be treated as the extension of optical flow. Therefore, it is the combination of optical flow and depth estimation in 3D scenarios. Monocular images are seldom utilized in the holistic training step for scene flow, and the structure takes the binocular videos as input to regress disparity to restore the scale. ISF \cite{scene_isf} is the first work to incorporates deep Convolutional Neural Network (CNN) and variational methods to estimate scene flow. DRISF \cite{scene_drisf} treats the inference step of Gaussian Newton (GN) as a Recurrent Neural Network (RNN) which means it can be trained in an end-to-end method. FD-Net \cite{scene_dfnet} further extends the unsupervised depth estimation \cite{scene_uldepth} and disentangles the full flow into object flow (targets pixels) and rigid flow (background pixels) to assess the characteristics respectively, which is able to avoid the warping ambiguity due to the occlusion and truncation. Competitive Collaboration (CC) \cite{scene_cc} sets the scene flow estimation as a game with three players.Two of them compete for the resource and the last one acts as a moderator. GeoNet \cite{scene_geonet} consists of two modules, a monocular depth with the 6 DoF ego-motion estimation and a residual network to learn the object optical flow.

%\textbf{Stereo Disparity Estimation in Autonomous Driving}: Disparity estimation based on a stereo image pair is a well known problem in computer vision, which can be seen as a fundamental part of the stereo depth estimation. The value of each box in the disparity map represents the pixel distance on the horizontal line between the left and right image from the same point in 3D space. The results of the stereo disparity estimation are similar to the segmentation output and the structure are similarly to the flow estimation, by replacing the subsequent to the simultaneously space adjacent frame.

%CNN based methods have recently achieved competitive results in this task. Researchers adopt a Siamese structure \cite{scene_siam} to match pairs of image patches for disparity estimation. Then the cost volume construction networks have appeared. DispNet \cite{scene_dispnet} regresses the similarities of left-right image features to form a cost volume by 2D convolution operation. GC-Net \cite{scene_gcnet} introduces a concatenation volume to form a 4D cost volume by 3D convolution to reduce the information loss. GwcNet \cite{scene_gwcnet} attempts to combine the above approaches by the group-wise volume. However all the methods are time-consuming for the inference step. The following research including successfully reduce the computational complexity by coarse-to-fine, multi-scales and depth-wise convolution.


%\begin{figure}
%\centering  %图片全局居中
%\includegraphics[width=8.5cm]{picture/methodology/semantic.png}

%\caption{Scene understanding results}
%\label{fig:3D Object Detection}
%\end{figure}


\subsubsection{\textbf{Prediction}}
In order to safely and efficiently navigate in complex traffic scenarios, an autonomous driving framework should be able to predict the way in which the other traffic agents (such as vehicles and pedestrians) will behave in the near future.
Prediction can be defined as probable results according to past perceptions. Let $X_{t}^{i}$ be a vector with the spatial coordinates of agents  $i$ at observation time $t$, with $t\in \left \{ X_{1}^{i},X_{2}^{i}, ... .X_{T_{obs}}^{i}  \right \} $.

\textit{\textbf{4.1 Model-based Approaches:}} These methods predict behaviors of agents, such as changing lanes, turning left and so on. One of the simplest methods to predict the probability distribution of vehicle behavior is the autonomous multiple modals (AMM) algorithms. This algorithm computes the maximum probability trajectory of each agent.

\textit{\textbf{4.2 Data-driven Approaches:}}
These methods are mainly composed of the neural network. After training on the perception dataset, the model makes a prediction of the next behaviour.
DESIRE\cite{prediction1} proposes an encoder-decoder framework that innovatively incorporates the scenario context and the interactions between traffic agents. 
SIMP\cite{prediction2} discretizes the output space, calculates the distribution of the vehicle's destination, and predicts an estimated time of arrival and a spatial offset.
FaF \cite{prediction3} pioneers the unification of detection and short-term motion forecasting based on LiDAR point clouds.

\subsubsection{\textbf{Tracking}}

The tracking problem begins with a sequence of vehicle-mounted sensor data. Depending on if neural network is embedded in the tracking framework, we divide them into the traditional method and the neural network method.


\textit{\textbf{5.1 Tradition Method:}}
The Kalman filter\cite{Kalman1} is a famous algorithm, particularly with regard to tracking agents. Because of the low computational cost, Kalman-based methods\cite{Kalman2}\cite{Kalman3} have quick response time even on low-spec hardware in simple scenarios.

The tracking problem also can be shown as a graph search problem\cite{graph1}.  Compared with Kalman-based methods, The most important advantage of graph-based approach is that it is better for the multi-tracking problems. Most methods\cite{graph2}\cite{graph3} exploit graph-based methods using the min-cost approach to solve tracking problems.

\textit{\textbf{5.2 Neural Network Method:}}
Neural networks have the advantage of being able to learn important and robust features given training data that is relevant and with sufficient quantity.

CNN is widely used in agents tracking. \cite{TrackingNetwork1} handles multi-agent tracking using combinations of values from convolutional layers. \cite{TrackingNetwork2} proposes appropriate filters for information drawn from shallow convolutional layers, achieving the same level of robustness compared with deeper layers or a combination of multiple layers.

One of the most difficult challenges for autonomous driving comes from temporal coherence in tracking task. To solve this problem, one popular approach is to integrate recurrent components into the classifier, which inherently accounts for the context provided by a set of elements from the sequence data. \cite{TrackingLSTM1} uses an LSTM-based classifier to track agents across multiple frames in time. Compared with CNN method, the LSTM-based approach is better suited to remove and reinsert candidate observations particularly when objects leave or reenter the visible area of the scene. In order to generate probabilities for the occurrence of future maneuver instances, \cite{TrackingLSTM2} establishes several maneuver classes and feed maneuver sequences data to LSTM layers.

==> body/methodology/detection_old.tex <==
\subsection{Perception}
%无人驾驶中的感知是指通过各型号传感器对车辆周围的三维环境进行定量测量，广义的感知包括车辆定位，目标检测与追踪，目标预测等子环节。在学术领域还有驾驶场景的深度补全、深度估计、光流估计、场景流估计，这些研究由室内机器人的环境感知任务发展而来，但是就当下的量产无人驾驶车辆而言少见基于上述研究的成果引入，其原因分析有二：其一，上述任务多基于视觉相机或深度相机采集的数据，但当今的无人驾驶车辆仍然以激光雷达为主要传感器。其二，上述任务不仅考虑了目标还考虑了背景，这无疑增加了计算单元的开销，这对以嵌入式设备或域控制器为处理核心的智能车辆提出了更高的挑战。因此本文没有涉及上述任务的综述，感兴趣的读者可以从这些文章找到这些领域在无人驾驶学术研究中的成果。

The perception in unmanned driving refers to the quantitative measurement of the three-dimensional environment around the vehicle by various types of sensors. The generalized perception includes vehicle positioning, target detection and tracking, target prediction and other sub-links. In the academic field, there are also driving scene depth completion, depth estimation, optical flow estimation and scene flow estimation. These studies are developed from the environment perception task of indoor robots. However, for the current mass production of unmanned vehicles, there are few results introduced based on the above research. First, most of these missions are based on data collected by vision cameras or depth cameras, but today's driverless vehicles still use lidar as their primary sensor. Second, the above tasks not only consider the target but also consider the background, which undoubtedly increases the overhead of the computing unit, which presents a higher challenge to the intelligent vehicle with embedded devices or domain controllers as the processing core. Therefore, there is no overview of the above tasks in this paper, but interested readers can find achievements in academic research in these areas

%(2)目标检测，无人驾驶中的目标检测可以分成对静态场景的检测和对动态目标的检测。对静态场景的检测包含车道线检测、可行驶区域和交通标志识别，低阶无人驾驶系统会通过上述的任务实现车道保持、变更速度等行为，高阶无人驾驶则会结合高精度地图融合其他任务进行精准地自主驾驶。对动态目标的检测包含对车辆、行人等全部交通参与者的位态检测，我们按照处理数据的不同划分成视觉检测、点云检测和融合检测。无人驾驶属于典型的3D任务，因此除某些任务无需3D检测外（例如交通标志识别），我们将主要关注3D目标检测而非2D目标检测。

\textit{A.2 Object  Detection} 

Target detection Target detection in unmanned driving can be divided into static scene detection and dynamic target detection. The detection of static scenes includes lane line detection, drivable areas and traffic sign recognition. The low-order unmanned system will realize lane keeping and speed change behaviors through the above tasks, while the high-order unmanned system will integrate other tasks with high-precision map for accurate autonomous driving. Detection of dynamic targets includes configuration detection of all traffic participants such as vehicles and pedestrians, which can be divided into visual detection, point cloud detection and fusion detection according to different data processing. Unmanned driving is a typical 3D task, so we will focus on 3D target detection rather than 2D target detection except for some tasks that do not require 3D detection (such as traffic sign recognition).

% 车道线检测方法分为两种：一种是传统算法，主要基于边缘特征或者是图像分割，通过图像预处理，特征提取等方式与卡尔曼滤波器等算法结合，在识别出车道线后采用后处理的方式形成最终的车道。然而这种传统方法易受到光照变化，行驶车辆，道路破损等干扰，导致效果欠佳。近年来，深度学习方法利用网络模型自动学习目标特征，具有较强的泛化能力，可以有效提高目标检测的准确率。得益于卷积神经网络的强大特征提取能力，性能也在不断提升。

%基于视觉的车道线检测任务一般包括三个主要流程，即图像预处理、车道检测与车道跟踪。其中预处理阶段最常见的程序包括感兴趣区域（region of interest，ROI）选择、去噪声和模糊、逆透视映射（inverse perspective mapping，IPM）、分割和边缘统计等。在完成预处理之后即可进行车道的检测，一般会先对车道的特征，比如边缘或颜色等进行提取，然后利用这些特征确定车道线的位置。在成功检测到车道线之后，可以使用跟踪算法，比如卡尔曼滤波器和粒子滤波器对车道进行细化与预测。

% 基于传统方法图像处理的车道线检测方法一般应用于结构化道路上。首先对输入图像进行感兴趣区域选择和去除无关元素，常用的处理方法是顶帽变换（Top-Hat Transform, 用于去除图像中的非车道标志。	一旦输入图像经过预处理，就可以提取车道特征，例如颜色和边缘特征，因此可以基于这些特征进行检测。Hough变换算法利用边缘像素图像，是以往研究中应用最广泛的车道检测算法之一。然而，该方法设计用于在开始时检测直线，在曲线车道检测中效率不高。通常可以基于模型拟合技术（如随机样本一致性（RANSAC））检测曲线车道。RANSAC通过递归测试模型拟合分数来拟合车道模型，以找到最佳模型参数。因此，它具有很强的处理异常特征的能力。最后，在车道成功检测后，可以使用卡尔曼滤波器或粒子滤波器等跟踪算法跟踪车道位置，以改进检测结果并以更有效的方式预测车道位置。

具体来说，Kang[Road lane segmentation using dynamic programming for active safety vehicles]使用Sobel算子检测车道边缘特征，并沿垂直方向将道路图像划分为多个子区域; Suddamalla[A novel algorithm of lane detection addressing varied scenarios of curved and dashed lanemarks]等人使用像素强度和边缘信息检测曲线和直线车道，并使用自适应阈值技术提取车道标记;



基于视觉的车道检测可以大致分为两类：基于特征的车道检测[9]−[19]


和基于模型的[20]−[29]。基于特征的方法依赖于车道标记特征的检测，如车道颜色、纹理和边缘。例如，在[9]中，使用Sobel算子检测噪声车道边缘特征，并沿垂直方向将道路图像划分为多个子区域。Suddamalla等人使用像素强度和边缘信息检测曲线和直线车道，并使用自适应阈值技术提取车道标记【10】。为了消除数字图像中的摄像机透视失真并提取真实的车道特征，可以通过透视变换有效地检测车道标线。Collado等人创建了道路图像的鸟瞰图，并提出了一种基于空间车道特征和Hough变换算法的自适应车道检测和分类方法【11】。文献[12]中使用了IPM和基于车道特征的聚类粒子滤波方法相结合的方法来估计多条车道。作者声称，如果在上下文中使用强lane模型，则鲁棒性较差，并且他们仅使用弱模型进行粒子滤波跟踪。除了使用彩色图像，还可以使用其他颜色格式的图像检测车道。颜色格式转换背后的一般思想是，黄色和白色车道标记可以在其他颜色域中更加清晰，因此对比度会增加。在[13]中，在车道假设阶段，使用扩展的边缘连接算法检测车道边缘。在车道验证步骤中，使用YUV格式的车道像素、边缘方向和车道标记宽度来选择候选的边缘链接对。在【14】中，使用无监督自适应分类器识别车道。彩色图像首先转换为HSV格式以增加对比度。然后，利用基于亮度值的阈值法对二值特征图像进行处理。虽然在某些正常情况下，颜色变换有助于车道检测，但它不稳定，处理阴影和照明变化的能力有限[4]。Borkar等人提出了一种分层方法来检测夜间车道【15】。采用时间模糊技术降低视频噪声，并基于自适应局部阈值方法生成二值图像。另一种域算法（LANA）中的车道查找表示频域中的车道特征【16】。该算法在频域中捕获车道强度和方向，并使用可变形模板检测车道标线。结果表明，LANA在各种条件下都具有较强的鲁棒性。在[17]中，介绍了一种时空车道检测算法。通过积累过去帧中的某些行像素生成一系列时空图像，并对合成图像应用Hough变换检测车道。在文献[18]中，基于车道梯度幅度特征和改进的Hough变换，设计了基于FPGA和DSP的实时车道检测系统。Ozgunalp和Dahnoun提出了一种改进的车道检测特征图[19]。首先利用边缘方向确定车道方向直方图，然后根据估计的车道方向对特征地图进行改进和移位。一般来说，基于特征的方法具有更好的计算效率，并且能够在车道标线清晰时准确检测车道。然而，由于假设了太多的约束，例如车道颜色和形状，这些方法的缺点包括与基于模型的方法相比，处理阴影和低可见性条件的鲁棒性较差
传统的基于图像处理的方法较大程度的依赖了车道线的颜色、形状等特征，这种方法在车道线被遮挡、污染的情况下鲁棒性较差。


%随着机器学习的发展，许多机器学习算法在计算机视觉任务中显示出巨大的优势，并且与传统方法相比，检测和识别性能显著提高。卷积神经网络是目标识别研究中最常用的方法之一。与传统的图像处理方法相比，通过使用卷积神经网络模型，车道线检测精度从80%左右显著提高到90%以上。卷积神经网络使用多个卷积核对输入进行特征提取。组成卷积核的每个元素都对应一个权重系数和一个偏差量（bias vector），类似于一个前馈神经网络的神经元（neuron）。卷积层内每个神经元都与前一层中位置接近的区域的多个神经元相连，区域的大小取决于卷积核的大小，被称为“感受野” 。卷积核在工作时，会有规律地扫过输入特征，在感受野内对输入特征做矩阵元素乘法求和并叠加偏差量[1]：其中， 表示第 层提取的特征图， 和 分别表示第 层特征的尺寸和通道数。 ， 和 是卷积层参数，对应卷积核大小、卷积步长（stride）和填充（padding）层数。基于机器学习的方法一般采用多层卷积网络对输入图像进行特征提取。然后将特征送入全连接网络（Fully Connected Neural Network，FCNN）得到输出。网络的输出一般有两类，一类是离散的分类结果，指示图像是否包含车道线。如果检测到车道线，则输出第二类结果，即对车道线位置和方向的连续估计。也有研究采用编码器-解码器结构实现车道线检测，此类方法将编码器提取到的特征送入由多层上采样层组成的解码器中，生成与输入相同大小的图像，输出仅包含车道线的二值图。随着生成对抗网络在计算机视觉中的应用，也有研究使用生成对抗网络进行车道线检测。生成对抗网络包含一个生成器和一个鉴别器，生成器一般采用编码器-解码器结构，鉴别器负责判断生成图像的真伪。通过引入生成对抗损失函数让生成器和鉴别器相互博弈来达到更好的检测效果。通过生成对抗网络得到的车道线一般比仅用编码器-解码器结构的网络更加精确。


\textbf{Lane detection} methods are divided into two types: one is the traditional algorithm, which is mainly based on edge features or image segmentation. Through image preprocessing, feature extraction and other methods combined with kalman filter and other algorithms, the final lane is formed by post-processing after identifying lane lines. However, this traditional method is prone to interference such as light changes, driving vehicles and road damage, resulting in poor results. In recent years, deep learning methods use network models to automatically learn target features and have strong generalization ability, which can effectively improve the accuracy of target detection. Thanks to the powerful feature extraction capability of convolutional neural network, its performance is also improving

Lane detection tasks based on vision generally include three main processes, that is, image preprocessing, lane detection and lane tracking. In the pre-processing stage, the most common programs include region of interest (ROI) selection, noise and blur removal, Inverse Perspective Mapping (IPM), segmentation and edge statistics, etc. Lane detection can be carried out after the completion of the pretreatment. Generally, features of the lane, such as edge or color, will be extracted first, and then the position of the lane line will be determined by using these features. After the lane lines are successfully detected, tracking algorithms such as Kalman filter and particle filter can be used to refine and predict the lane.

Lane line detection methods based on traditional image processing generally use edge extraction method to detect lane lines on structured roads. Firstly, the input image is selected for the region of interest and irrelevant elements are removed. The commonly used processing method is top-hat Transform, which is used to remove non-lane signs in the image. In morphology, top-hat Transform is an operation to extract small elements and details from a given image. The formula is where and respectively represent the images before and after the top hat transformation, represent the open operation, and represent the structure element of the top hat operation. The top hat transformation will remove objects larger than the structure element in the image, so as to delete non-lane signs such as turning signs and road text. After removing irrelevant elements, this method extracts the edge information of the image, and then uses Hough transform to find the straight lines in the edge graph. Hough transform is a method to find straight lines or curves in 2d pixels by using the global properties of images. The principle of Hough transform is to map the image space to the parameter space and convert the curves in the image space to the corresponding reference points in the parameter space. Its main advantage is that it is less affected by noise and curve discontinuities. After all the lines in the image are obtained, the final lane lines are obtained by clustering and denoising according to the slope and other features of the lines. The traditional image processing method relies on the color and shape of the lane lines to a large extent, and this method has poor robustness when the lane lines are blocked and polluted.


With the development of machine learning, many machine learning algorithms show great advantages in computer vision tasks, and their detection and recognition performance is significantly improved compared with traditional methods. Convolutional neural network is one of the most commonly used methods in object recognition. Compared with traditional image processing methods, the accuracy of lane line detection is improved from about 8\% to more than 90\% by using convolutional neural network model. Convolutional neural network uses multiple convolution check inputs for feature extraction. Each element of the convolution kernel corresponds to a weight coefficient and a bias vector, similar to neuron of a feedforward neural network. Each neuron in the convolution layer is connected to multiple neurons in the region with similar positions in the previous layer, and the size of the region depends on the size of the convolution kernel, known as the "receptive field". When the convolution kernel is working, it will regularly sweep the input features, multiply and sum the matrix elements of the input features in the receptive field, and add up the deviation [1] : where, represents the feature graph extracted at the first layer, and represents the size and channel number of the features at the first layer respectively. , and are convolution layer parameters, corresponding to the convolution kernel size, stride and padding layers. Multi-layer convolutional networks are generally used to extract features from input images based on machine learning. Then the features are sent into the Fully Connected Neural Network (FCNN) to get the output. The output of the network generally has two types. One is the discrete classification result, indicating whether the image contains lane lines. If lane lines are detected, the second type of result is output, which is the continuous estimation of the position and direction of lane lines. There are also studies using encoder-decoder structure to achieve lane line detection. In this method, the features extracted from the encoder are fed into a decoder composed of multiple up-sampling layers to generate images of the same size as the input, and the output contains only a binary graph of lane lines. Along with the application of generative adversarial network in computer vision, there are also researches on lane detection using generative adversarial network. The generative adversance network consists of a generator and a discriminator. The generator usually adopts encoder-decoder structure, and the discriminator is responsible for judging the authenticity of the generated image. The generator and discriminator play game with each other to achieve better detection effect by introducing generative adversarial loss function. Lane lines obtained by generating adversarial networks are generally more accurate than those obtained by encoder-decoder networks alone.


%交通标志检测与识别系统是无人驾驶系统中一个重要的组成部分,通过对道路上交通标志的准确识别,将识别结果反馈给上层行车控制策略系统,车辆根据行车策略做出相应的反应,提高道路安全性,更好地辅助无人驾驶系统。

\texbf{traffic sign detection} The traffic sign detection and recognition system is an important part of the unmanned driving system. Through the accurate identification of traffic signs on the road, the identification results will be fed back to the upper driving control strategy system, and the vehicle will respond accordingly according to the driving strategy to improve road safety and better assist the unmanned driving system.

%基于视觉的3D目标检测
\texbf{visual 3D object detection} The traffic sign detection and recognition system is an important part of the unmanned driving system. Through the accurate identification of traffic signs on the road, the identification results will be fed back to the upper driving control strategy system, and the vehicle will respond accordingly according to the driving strategy to improve road safety and better assist the unmanned driving system.

%基于激光的3D目标检测是指通过激光雷达捕获的点云数据进行目标3D属性的检测。由于点云本身包含了有效点的空间位置，如果该点位于目标表面即可以认为大致了解到了目标所在的位置信息，因此基于点云的3D目标检测相较于视觉3D检测在精度上有更好的表现。

\textbf{point cloud based object detection} Laser-based 3D target detection refers to the detection of 3D target attributes through point cloud data captured by lidar. Since point cloud itself contains the spatial position of effective points, if the point is located on the target surface, it can be considered that the location information of the target is roughly understood. Therefore, 3D target detection based on point cloud has better performance in accuracy compared with visual 3D detection.

%基于融合的3D目标检测
\textbf{visual and point cloud fusion 3D object detection} abc
 
%(3)目标追踪 目标跟踪是目标检测在时间轴上的延续，获得连续时间序列一系列的目标检测结果后，可关联不同时刻下的检测结果是否属于同一目标，并推算目标运动速度、加速度等不可直接观测的微分运动信息，甚至于预测目标未来时刻的运动状态。
(3) target tracking target tracking is a continuation of target detection on the timeline, obtain continuous time series after series of target detection results, can be associated with different times of the test results are belong to the same goal, and the estimation of target motion velocity and acceleration can not be directly observed, such as differential motion information, and even predict target motion state of the future time.

%(4)预测 目标跟踪是目标检测在时间轴上的延续，获得连续时间序列一系列的目标检测结果后，可关联不同时刻下的检测结果是否属于同一目标，并推算目标运动速度、加速度等不可直接观测的微分运动信息，甚至于预测目标未来时刻的运动状态。
(4) Prediction

==> body/methodology/human-mechine.tex <==
\subsection{Human Behaviors in Autonomous Vehicles}

Human behaviors and human factor issues are important topics for autonomous vehicles, as they determine the widespread acceptance of autonomous vehicles. Modelling and understanding human behaviors can also contribute to the establishment of mutual understanding and mutual trust between humans and vehicles. However, human is a highly complex system, and a unified human behavior modeling framework still need to be investigated further \cite{human-machine_1}. In this section, the human behavior and human factor issues will be discussed according to the level of autonomy (SAE J3016) as the differences in human behavior can be significant \cite{human-machine_2, smc_21}. 

\subsubsection{\textbf{Driver Assistance and Partial Driving Automation (L1-L2)}}
On L1 or L2 automated driving vehicles (ADVs), human drivers are still inside the vehicle control loop and suppose to drive (mental drive) even if the feet or hands are off the pedals and steering wheel. In this case, the human driver can benefit from a series of advanced driver assistance systems (ADAS) such as lane departure warning (LDW) \cite{human-machine_3}, lane departure assistant (LDA) \cite{human-machine_4}, adaptive cruise control (ACC) \cite{human-machine_5}, and lane-keeping assistance (LKA) \cite{human-machine_6}, etc. To provide accurate assistance to the human drivers, several popular research areas were developed, including fatigue (muscle/mental)/drowsiness detection \cite{human-machine_7}, driver intention inference \cite{human-machine_8}, attention \cite{human-machine_9}, workload \cite{human-machine_10}, emotion \cite{human-machine_11}, and distractions \cite{human-machine_12}. Such assistance systems usually can be separated into two fundamental groups, which are physical (physiological)-behavior and psychological behavior-based methods. 

%Specifically, physical-behaviors are usually related to vehicle interaction and control, distractions and drowsiness behaviors, etc. Common physiological signals include gaze, head, facial, body, hand, foot, speech, brain dynamics (Electroencephalogram, EEG), and neuromuscular dynamics (electromyogram, EMG) \cite{human-machine_13, human-machine_14}. These signals usually can measure the driver's physical state directly. On the other hand, driver psychological behaviors, such as attention, intention, emotion, mental distraction, mental workload, and mental fatigue, reflect the driver's mental cognitive states about the driving task, which cannot be detected and measured directly. Therefore, the most common approach for inferring cognitive driver states is using measurable physiological signals as model inputs and inferring the mental states by building a representation learning-based model \cite{human-machine_15}. 

\subsubsection{\textbf{Conditional Driving Automation (L3)}}
On L3 ADVs, a human driver can further engage in secondary tasks, and long-term monitoring is no longer required. The human driver is only required to be present and capable of taking over the control at any time, especially if an emergency occurs due to system malfunction and surrounding context uncertainty. However, one of the famous drawbacks of L3 automation is the human driver cannot guarantee to provide quality and safe take-over control especially facing the time-constrained decision-making situation \cite{human-machine_16}. Therefore, the most widely studied points for L3 regarding human factors issues are the design of take-over control algorithms, resuming control and smooth switching of the control authority \cite{human-machine_17}. 
%Both driver and vehicle are allowed to raise the take-over request. While, when the vehicle raises the take-over request to the human driver, things can be much more challenging. For instance, it was shown that drivers’ responses to the resumption of control could be less controlled and more aggressive compared to when they were in manual control \cite{human-machine_18}. Also, drivers can easily be distracted, and long-term monitoring can lead to a higher mental workload compared to manual driving \cite{human-machine_19}. They cannot guarantee that they will be able to take over the vehicle quickly and safely, especially encountering critical situations, due to the loss of situation awareness and skill degradation caused by long-term automated driving \cite{human-machine_20}. Most of these studies rely on a better understanding of human behaviors, such as driver distraction and attention recognition \cite{human-machine_21}, as well as neuromuscular dynamic modeling for alert and assistance \cite{human-machine_22}. 

\subsubsection{\textbf{High/Fully Driving Automation (L4-L5)}}
With higher-level automation, human drivers are no longer expected to maintain a proper situation awareness level in case to control the vehicle when necessary. However, complex issues can arise as well, one of which is how humans understand and partner with the autonomous system. To enable the acceptance and behavior adaptation to the higher-level ADVs, driver trust should be developed. 

Driver trust is currently a major reason for the generalization and commercialization of automated driving vehicles. As shown in \cite{human-machine_23}, human trust in the AVs largely depends on the automation's driving performance considering the safety, comfortability, predictability, and ethical response to critical situations. A recent study \cite{human-machine_24} supported that the initial introduction of self-driving cars will cause unexpected reactions and situations, which may affect the level of trust the public has in the new technique. Choi et al. surveyed 552 drivers on their attitudes toward automated driving; it was shown that trust in autonomy is the most dominant factor \cite{human-machine_25}. According to an investigation of 162 Tesla drivers on their trust in Autopilot and Summon systems \cite{human-machine_26}, it was found that high levels of initial trust in the systems could be established if an excellent introduction to the system capability is provided, and the frequency of system usage will increase over time, regardless of whether participants experienced an automation failure. 

\subsubsection{\textbf{Human-Machine-Interface (HMI)}}
The automated driving techniques make the design of HMI even more complex as the HMI system for ADVs relies on human-centered design approaches \cite{human-machine_27} to ensure safety awareness, mutual trust, pleasure, and comfort \cite{human-machine_28}. Currently, the HMI system becomes the main module that enables the collaboration between driver and vehicle. The design of the HMI system is a system engineering task \cite{human-machine_29}, and this section focuses on the introduction of in-cabin and out-cabin HMI design. 

For L4/L5, vehicle autonomy is expected to be fully responsible for the driving tasks, and the human drivers are even no longer required to maintain driving knowledge and skills. Hence, it is hard to require the human occupier to understand the context properly. Instead, only safety-related information for the vehicle behaviors and future planning has to be reported and displayed \cite{human-machine_30}. A well classification for various types of HMI on highly ADVs was proposed in \cite{human-machine_31}. Specifically, the onboard HMI system can be divided into five categories, namely, dynamic HMI, automation HMI, information HMI, vehicle HMI, and external HMI. Three recommended HMI design factors were introduced in \cite{human-machine_32}. First, a head-up display can avoid the distraction of the human driver. Second, HMI systems should assist with time-constrained maneuvers and decisions. Last, the driver monitoring system is needed to help understand the human states for high-quality visualization and explanation. An expert evaluation study for the design of HMI was discussed in \cite{human-machine_33}. According to the expert evaluation, the two most essential functions of HMI are 1) present the automation availability, navigation, and environmental information, and 2) improve the driver's attention through speech instruction, LED bar light, and seat oscillation. 

%The external HMI is designed to extend the cooperation of the ego-vehicle with multiple surrounding vehicles and to explicitly communicate the driving intentions among the multiple agents. Based on an international survey on how ADVs perform external communication and interaction with other road users, a general expectation of effective interaction and communication can be clarified \cite{human-machine_34}. Benderius et al. argued that a complex external HMI is needed for ADVs to indicate their intent \cite{human-machine_35}. Instead, they proposed a show, don’t tell principle for external HMI to explicitly demonstrate the plans with a more general-purpose light bar. When treating the interaction between different road users as a multi-agent interaction system, the mutual-understanding is critical to such a system, and the agents should explicitly communicate their intention. External HMI for ADVs is also expected to use multi-modal signals to integrate auditory, visual, and V2V communication systems for holistic HMI system design \cite{human-machine_36}. 

%\subsubsection{Conclusion and Future Works}
%In sum, the increase of vehicle autonomy for commercial passenger cars will not reduce the necessity of human behaviors and human factors issues but may increase the complexity of these problems. The responsibility of ensuring a safe, comfortable, and pleasant journey is extremely heavy for autonomous vehicles.  Future works for HMI systems on ADVs should further focus on the development of mutual understanding and mutual trust mechanisms, ensuring communication transparency and efficiency with both onboard and surrounding users. The personalized and human-centered design approach should be highlighted to guarantee the ADVs also able to understand user characteristics and personalities in case to interact with humans more effectively (especially vulnerable users \cite{human-machine_37, \cite{human-machine_38}}). Meanwhile, security \cite{human-machine_39}, privacy \cite{human-machine_40}, and ethics \cite{human-machine_41} issues are also expected to be carefully considered. 

==> body/methodology/planning.tex <==
\subsection{\textbf{Planning}}
%决策规划，统一称为planning module，在第一章扼要介绍该模块的一句话：
The planning module is responsible for finding a local trajectory for the low-level controller of the ego vehicle to track. 

%规划模块的详细文献回顾
The planning module is responsible for finding a local trajectory for the low-level controller of the ego vehicle to track. Herein, “local” means that the resultant trajectory is short in its spatial or temporal range; otherwise the ego vehicle cannot react to risks beyond the sensor ranges. The planning module typically contains three functions, namely global route planning, local behavior planning, and local trajectory planning \cite{planning_1,survey_planning_1, survey_planning_4}. Global route planning provides a road-level path from the start point to the destination on a global map; local behavior planning decides a driving action type (e.g., car-following, nudge, side pass, yield, and overtake) for the next several seconds while local trajectory planning generates a short-term trajectory based on the decided behavior type. This section reviews the techniques related to the three functions in the planning module.

\subsubsection{\textbf{Global Route Planning}}
Global route planning is responsible for finding the best road-level path in a road network, which is presented as a directed graph containing millions of edges and nodes. A route planner searches in the directed graph to find the minimal-cost sequence that links the starting and destination nodes. Herein, the cost is defined based on the query time, preprocessing complexity, memory occupancy, and/or solution robustness considered.


The development history of global route planning techniques is much longer than that of autonomous vehicle techniques because global route planning also serves manually driven vehicles. As indicated by \cite{planning_4}, the existing global route planning methods are classified as goal-directed methods, separator-based methods, hierarchical methods, bounded-hop methods, and their combinations. Details are provided in survey papers such as \cite{planning_4,planning_5}.

\subsubsection{\textbf{Local Behavior/Trajectory Planning}}
Local behavior planning and local trajectory planning functions work together to output a local trajectory along the identified global route. Since the resultant trajectory is local, the two functions have to be implemented in a receding-horizon way unless the global destination is not far away \cite{planning_6}. It deserves to emphasize that the output of the two functions should be a trajectory rather than a path \cite{planning_7}, otherwise extra efforts are needed for the ego vehicle to evade the moving obstacles in the environment.

Broadly speaking, the two functions would work in two different ways. One is the end-to-end way, i.e., to develop an integrated perception+planning system that receives the raw data from the on-board sensors and outputs a local trajectory directly. The other way is to implement the local behavior planning and local trajectory planning functions sequentially.

\textbf{\textit{2.1 End-to-end Methods} }: 
Compared with the sequential-planning solution reviewed I the next subsection, an end-to-end solution nominally deals with vehicle-environment interactions more efficiently because there is not an external gap between the perception and planning modules \cite{teng2}. The input of an end-to-end system is the large amount of raw data obtained by the on-board sensors whereas the output is a local trajectory. Since the relationship between the input and output is too intricate to be summarized as complete rules \cite{planning_9}, machine learning methods are commonly used, most of which are classified as imitation-learning-based and reinforcement-learning-based methods \cite{planning_10, smc_1, smc_2, smc_3, smc_8, smc_11, smc_13, smc_20, smc_23}.

An imitation-learning-based method builds a neuro network based on training samples [11]. Challenges lie in how to collect massive training samples that are consistent and how to guarantee learning efficiency (e.g., free from overfitting). Reinforcement-learning-based methods obtain knowledge by trial-and-error operations, thus they rely less on the quality and quantity of external training samples \cite{survey_e2e_1, planning_12, planning_13}.


End-to-end methods are still not mature, thus most of them are trained/tested in simulations rather than real-world scenarios \cite{planning_14}. Recent research efforts focus on how to enhance learning interpretability, security, and efficiency \cite{planning_15}.

\textbf{\textit{2.2 Sequential-planning-based Methods}}: 
As opposed to the aforementioned end-to-end solution, applying local behavior planning and trajectory planning functions sequentially has been a common and conventional choice in the past decade. However, the boundary between local behavior planning and trajectory planning is rather blurred \cite{survey_planning_1}, e.g., some behavior planners do more than just identify the behavior type. For the convenience of understanding, this paper does not distinguish between the two functions strictly and the related methods are simply regarded as trajectory planning methods.

Nominally, trajectory planning is done by solving an optimal control problem (OCP), which minimizes a predefined cost function with multiple types of hard constraints satisfied \cite{planning_16}. The solution to the OCP is presented as time-continuous control and state profiles, wherein the desired trajectory is reflected by (part of) the state profiles. Since the analytical solution to such an OCP is generally not available, two types of operations are needed to construct a trajectory. Concretely, the first type of operation is to identify a sequence of state grids while the second type is to generate primitives between adjacent state grids.


\textit{\textbf{2.2.1 State Grid Identification}}:  State grid identification can be done by search, selection, optimization, or potential minimization. Search-based methods abstract the continuous state space related to the aforementioned OCP into a graph and find a link of states there. Prevalent search-based methods include A* search \cite{planning_17, planning_18} and dynamic programming (DP) \cite{planning_19, planning_20, planning_21}. Selection-based methods decide the state grids in the next one or several steps by seeking the candidate with the optimal cost/reward function value. Greedy selection \cite{planning_22} and Markov decision process (MDP) series methods typically \cite{planning_23, planning_24} fall into this category. An optimization-based method discretizes the original OCP into a mathematical program (MP), the solution of which are high-resolution state grids \cite{planning_25, planning_26, planning_27, planning_28,planning_29, planning_30}. MP solvers are further classified as gradient-based and non-gradient-based ones;  gradient-based solvers typically solve nonlinear programs \cite{planning_16, planning_27, planning_29}, quadratic programs \cite{planning_21, planning_28, planning_31}, quadratically constrained quadratic programs \cite{planning_30} or mix-integer programs \cite{planning_32}; non-gradient-based solvers are typically represented by metaheuristics \cite{planning_33}. Potential-minimization-based methods adjust the state grid positions by simulating the process they are repelled or attracted by forces or in a heuristic potential field. Prevalent methods in this category include the elastic band (EB) series \cite{planning_35}, artificial potential field methods \cite{planning_7, planning_36}, and force-balance model \cite{planning_37}. 

The capability of each state grid identification method is different. For example, gradient-optimization-based and potential-minimization-based methods are generally more flexible and stable than typical search-/selection-based methods \cite{planning_38}, but search-/selection-based methods are more efficient to explore the entire state space globally \cite{planning_35, planning_39, planning_40}. Different methods could be combined jointly as a coarse-to-fine strategy, as has been implemented by many studies such as \cite{planning_16, planning_17, planning_21, planning_26, planning_28, planning_29, planning_30}.


\textit{\textbf{2.2.2 Primitive Generation}}:  Primitive generationis commonly done by closed-form rules, simulation, interpolation, and optimization. Closed-form rules refer to methods that generate primitives by analytical methods with closed-form solutions. Typical methods include the Dubins/Reeds-Shepp curves \cite{planning_41, planning_42}, polynomials \cite{planning_22, planning_43}, and theoretical optimal control methods \cite{planning_44}. Simulation-based methods generate trajectory/path primitives by forward simulation, which runs fast because it has no degree of freedom \cite{planning_17, planning_45}. Interpolation-based methods are represented by splines or parameterized polynomials. Optimization-based methods solve a small-scale OCP numerically to connect two state grids \cite{planning_47, planning_48}.

State grid identification and primitive generation are two necessary operations to construct a trajectory. Both operations may be organized in various ways. For example, \cite{planning_45} integrates both operations in an iterative loop; \cite{planning_47} builds a graph of primitives offline before online state grid identification; \cite{planning_21} identifies the state grids before generating connective primitives.

If a planner only finds a path rather than a trajectory, then a time course should be attached to the planned path as a post-processing step \cite{planning_49}. This strategy, denoted as path velocity decomposition (PVD), has been commonly used because it converts a 3D problem into two 2D ones, which largely facilitates the solution process. Conversely, non-PVD methods directly plan trajectories, which has the underlying merit to improve the solution optimality \cite{planning_19, planning_20, planning_50}.

Recent studies in this research domain include how to develop specific planners that fit specific scenarios/tasks particularly \cite{planning_6, planning_51, planning_52}, and how to plan safe trajectories with imperfect upstream/downstream modules \cite{planning_53, planning_54, planning_55}.

%规划模块的未来展望

==> body/methodology/system.tex <==

\subsection{\textbf{System Design}}
In this section, the system design of the autonomous vehicle will be described from three essential aspects of AVs, namely, the computing systems, sensor systems, and system design for various applications.

\subsubsection{\textbf{Computing System}}
The computing system plays a vital role in AVs to guarantee safety, security, energy and communication efficiency. For a typical AV which usually can be equipped with a large number of onboard sensors, including Lidar, cameras, Radar, communication module, and GPS, etc., the data generated per minute can be huge. To ensure the efficient processing and fusing of heterogeneous information, the computing system must be well designed to process the information in real-time and maintain safe autonomous driving. According to \cite{survey_8}, there are two basic types of computing architecture that are widely used in AVs, which are the modular design method and the end-to-end design method. The modular design approach decouples the functional units into separate modules which can be easier for system implementation, fault diagnosis, and module update. Based on the modular design approach, the computing architecture of AV can be separated into the following key modules (as shown in Fig. \ref{fig:system_fig_1}), including computation, communication, storage, security and privacy, and power management. While the end-to-end computing architecture is largely motivated by current artificial intelligence and mainly relay on learning-based approaches to process the sensing data and generate control output directly \cite{system_2, system_3}. Considering the modular design approach is much more widely used and mature for computing architecture design on AVs, the following parts will review the computing systems based on this branch.

\begin{figure}
\centering  %图片全局居中
\includegraphics[width=8.5cm]{picture/methodology/system.png}

\caption{Typical computing architecture for AVs\cite{survey_8, survey_system_1, survey_system_2} }
\label{fig:system_fig_1}
\end{figure}

\textbf{\textit{1.1 Computing Hardware}}: 
There is multiple powerful computing hardware to support the real-time computation capability of AVs. Typically, the Central Processing Unit (CPU), Graph Processing Unit (GPU), Field Programmable Gate Array (FPGA), Digital Signal Processor (DSP), Application Specific Processor Unit (ASIC) and its custom-developed deep learning-oriented Tensor Processing Unit (TPU) are the widely used computing hardware on AVs nowadays \cite{survey_system_2, survey_8, smc_22}. Specifically, Nvidia published the Nvidia Drive series to support AV technology with powerful GPU support \cite{system_9}. Xilinx released the Zynq UltraScale+MPSoC automotive-grade processor based on FPGA, which achieved more energy-saving performance (14 images/W) than Nvidia Tesla K40 GPU (4 images/W) \cite{system_10}. The Mobile EyeQ6 series and TPUv4 are the leading ASIC-based solution for AVs, which show significant improvement in the computation power and energy efficiency \cite{system_11}. 

\textbf{\textit{1.2 Operating System}}: 
Real-time operating system (RTOS) is key module for the computing systems on AVs which enable the resouces management and real-time perception, planning, decision-making, and control autonomously at a fast speed \cite{survey_system_2}. OS on AVs should support real-time resource allocation, networking, filing, communication, etc. Two common RTOS kernels are QNX and VxWorks \cite{system_12, system_13}. The QNX is widely used in the automotive industry that contains CPU scheduling, interprocess communication, interrupt redirection, and timer \cite{system_12}. VxWorks is a monolithic kernel and is designed for real-time embedded systems and also can be used for safety and security \cite{system_13}. It is designed with a shared memory architecture and it supports multiple architectures like Intel, POWER, and ARM. 

\textbf{\textit{1.3 Middleware}}： 
In the middle of RTOS and application layers, the middleware layer is needed to bind the multiple autonomous driving services together to manage the application communication and schedule the sensing and computing resources. In \cite{system_7}, three influential middleware architectures, namely Robot Operating System (ROS1), ROS2, and Cyber are evaluated regarding the communication latency for autonomous driving applications. The Inter-Process Communication mechanism in ROS1 provides high compatibility and extensibility \cite{system_15}. ROS2 shows efficient performance in real-time distributed systems based on the Data Distribution Service (DDS)-based communication scheme \cite{system_16}. Then, the Cyber is a recently published middleware architecture by Baidu Apollo, which is primarily designed for autonomous driving. 

\cite{system_7} summarised the three architectures based on a comparison study, it was found that 1) the communication through a shared memory mechanism is the optimal solution considering the performance and reliability of AVs; 2) Data copy and serialization/deserialization operation in the middleware layer are the main attributes of communication overhead. 3) Optimization in communication characteristics can bring significant benefits to computation efficiency. 4) the higher the performance of the platform, the more likely the communication becomes the bottleneck for processing speed. 5) Additional latency can be introduced if the publishing frequency and corresponding processing time are not well calibrated. 

In sum, middleware can be a contributor to the end-to-end latency and to avoid becoming the performance bottleneck for the overall computing system, the communication and management in the middleware should be carefully designed.

\textbf{\textit{1.4 Metrics for Computing Systems on AVs}}: 
In \cite{survey_system_1}, the authors identified seven evaluation metrics for the computing system on AV, which are accuracy, timelines, power, cost, reliability, privacy, and security. A brief summary of the characteristics of these metrics is demonstrated in Table \ref{table:system_table_1}. 

\input{tabels/methodology/system_tabel_1}

\textbf{\textit{1.5 Constraints for Computing Systems on AVs:}}
Though computing systems on AVs have achieved significant improvement in recent years, there are still several essential constraints exist which can delay the wide deployment of commercial AVs. In \cite{survey_system_1}, five major design constraints, namely, performance constraints, predictability constraints, storage constraints, thermal constraints, and power constraints for AVs are identified and analysed. 

Specifically, performance constraints mainly exist at the application level as shown in \ref{fig:system_fig_1}. In terms of the fundamental functions of AVs, including perception, planning and decision-making, and control, the gap between machine and human performance still exists. It is stated that the frame rate and processing latency are two main performance constraints for the AVs. The human driver can react to an event with the action within 100-150ms, therefore, for safety concerns, the vehicle should react even faster than the human driver within a latency of 100ms at a frequency of at least once every 100ms as well \cite{survey_system_1}. 

Predictability is another constraint which is defined from both the temporal aspects (meet the time deadline) and functional aspects (making the correct decision). Despite the conventional mean latency metric, the tail latency (99.99th-percentile latency) should also be used to satisfy the stringent predictability requirement \cite{survey_system_1}.

The storage constraint is an essential aspect and bottleneck for energy-saving and computing performance on AVs. It is shown that one AV can generate 2 to 40 TB of data per day \cite{survey_8}. The tens of TBs of storage space per day would require high storage speed and space for the vehicle. Besides, the real-time data storage and the transfer would also require a significant boost in energy and power usage. 

The thermal constraints of the AVs can be a serious consideration as well. There are two typical aspects of the thermal constraints which are 1) the temperature to keep the computing system working at operational range, and 2) the heat generated by the computing system should lead to limited impact on the vehicle thermal profile \cite{survey_system_1}. It is shown that without the cooling system, every 1 kW power consumption by the computing system would increase the in-cabin temperature up to 10℃ per minute \cite{system_17}. Therefore, usually, the computing system should be implemented in a climate-controlled area which means an additional cooling system is needed to mitigate the thermal impact of the computing system \cite{ system_17}. 

Last, power constraint is another critical aspect which can significantly influence the capability of AV. According to \cite{survey_system_1}, the power constraint of the computing system contains three major aspects which are power consumption of the computing system, consumption of the storage, and cooling overhead. The computing consumption and additional energy consumption for storage and cooling would dramatically decrease the millage of AVs, especially the electric AVs. For instance, the miles per gallon (MPG) rate can be reduced by one for every additional 400 W energy usage, and an energy-hungry system like GPUs can reduce the fuel efficiency by up to 11.5\% \cite{survey_system_1}. Therefore, more energy-efficient computing systems and green AI techniques are extremely expected for AVs in the future. 

\subsubsection{\textbf{Sensor Systems}}
Sensor systems on AVs provide essential sensing and detection data to the computation units. Common onboard sensors for AVs include Lidar, Radar, cameras, ultrasonic, GPS, IMU, and GNSS, etc. Dues to the large uncertainty properties during driving, AVs should rely on multiple sensor fusion to guarantee driving safety. Hence, in this part, the characteristics of common sensors and sensor fusion techniques are reviewed. 

\textbf{\textit{2.1 Sensors in AVs}}: 
De Jong et al. classified the sensors on AVs into smart sensors and non-smart sensors according to the internet-of-things concept in \cite{survey_hardware_3}. Smart sensors on AVs refer to those that can provide extra detection or perception information, such as object detection/tracking, and other event description from the camera, Lidar, or Radar systems. On the contrary, non-smart sensors are those which only provide raw data for processing. The study of the characteristics of on-board sensor systems has been widely studied in \cite{survey_hardware_3, system_20, system_21, survey_12}. A brief description of the different sensors and selected review studies are shown in Table \ref{table:system_table_2}. 

\input{tabels/methodology/system_tabel_2}

%\textbf{Sensor Fusion Technologies}
%Sensor fusion technologies have been widely studied for AVs \cite{system_8, system_20}. It improves the driving safety and detection robustness by reducing the detection uncertainties, false alarm rate, and overcoming the shortcomings of the individual sensor systems \cite{system_8}. It is shown that three primary sensor fusion methods for perception-purpose can be found in the literature, which are camera-Lidar, camera-Radar, and camera-Lidar-Radar \cite{system_8}. From the architectural point of view, sensor fusion can be divided into three levels, which are low-level fusion (LLF), mid-level fusion (MLF), and high-level fusion (HLF) (as shown in \ref{fig:system_fig_1}). Regarding the LLF, raw data are normally fused at an earlier stage to reduce the noise and uncertainty in the sensing results. However, precise sensor calibration is needed when applying LLF. The MLF is also known as feature fusion. It fuses abstracted feature information such as colour, location, and motion patterns from the corresponding sensors and further performs detection and recognition based on the fused features. Last, HLF is a framework to perform high-level information or decision fusion and make final results based on the individual results like detection and tracking from the corresponding sensors. In \cite{survey_static_3}, an algorithm fusion method for perception was also discussed based on the algorithm redundancy and parallel testing consideration. In \cite{system_20}, the sensor fusion strategies are systematically classified into four categories, which are fusion based on discernible units, fusion based on complementary features, fusion based on target attributes, and fusion based on a multi-source decision.

%Regarding the sensor fusion algorithms, currently, a large number of studies are based on deep learning methods. Deep learning networks such as convolutional neural networks (CNN) and visual transformers can be used as backbone networks to process the data from different sensors, extract the temporal-spatial patterns, and share information at either early-stage, mid-stage, or late-stage \cite{system_29, system_43}. Accordingly, the end-to-end learning processing can be developed for sensor fusion without hand-craft feature engineering. Despite the deep learning-based approach, conventional methods usually focus on knowledge-based methods, statistical and probabilistic methods, etc. The most successful methods including the Kalman filter, unscented Kalman filter, and particle filter has been broadly discussed in \cite{system_44, system_45, system_46}. In sum, it is shown that DL-based sensor fusion technologies are gaining great advantages nowadays in terms of accuracy, efficiency, and generalization, therefore, it is becoming one of the hottest research topics for AVs.

\textbf{\textit{2.2 System Design for Autonomous Vehicles with Various Application Scenarios}}: 
The system design of AVs is also heavily dependent on the application scenarios, policies, and regulations. Nowadays, the most commonly used standard for autonomous vehicles regarding safety, communication, and design can be found in \cite{system_47}. The standard roadmap in \cite{system_47} covers the current and ongoing standards for safety and assurance, perception, decision-making, data, security, infrastructures, and human factors. It should also be noticed that the design of the autonomous vehicle shall consider the specific application domains as well. For example, the autonomous mining truck and its testing techniques have been summarized in \cite{system_48}, which shows significantly different considerations compared to passenger cars. Other successful applications of autonomous vehicles at airports, harbours, and for logistic purposes can be found in \cite{ system_51}. Clearly, each specific autonomous vehicle requires significantly different concerns in the overall system design and should respect the specific real-world application environment. 

Another emerging research areas for system design in AVs are the design of the explainable interface for AVs. Explanation of the perception, localization, decision-making, and control to the human occupier is an essential design requirement for future AVs to enhance the human trust and acceptance of the AVs for worldwide commercialization \cite{survey_11}. The Explainability of AVs can be further divided into interpretability and completeness. Further, interpretability has two main branches, namely, transparency and post-hoc explanation \cite{survey_explainable}. Meanwhile, local explanation and global explanation also requires different system design for the AVs \cite{survey_explainable}. In sum, the design criteria for an explainable interface of AVs will contribute to the societal and legal requirements of the AVs, and more importantly enable safer, transparent, public-approved, and environmentally friendly AVs \cite{system_54}.

==> body/methodology/testing.tex <==

\subsection{Testing}
Vehicle testing has become a popular research topic in the field of intelligent vehicles since 2016. On one hand, several companies that produce intelligent vehicles encountered vehicle accidents during testing or running, which rises urgent demand to identify causes of accidents and fix complicated intelligent vehicle systems. On the other hand, researchers are increasingly interested in intelligence testing of generalized intelligent systems.  (Artificial Intelligence Test A Case Study of Intelligent Vehicles；Parallel Testing of Vehicle Intelligence via Virtual-Real Interaction).

As the research progresses, researchers gradually build a framework of conducting research. They summarize effective methods and focused on several key works \cite{sn_1, sn_2, sn_5, testing_tiv}.

%首先，研究者区分了业界提到的功能测试，性能测试和智能测试等几个概念。简而言之，性能测试关注在给定的特殊条件下，车辆或者车辆部件是否能针对特定的输入得到符合要求的输出（例如激光雷达是否能对于200m外的1m*1m的物体给出超过3个云点的输出）。功能测试关注在一定范围的条件下，车辆是否能针对一定范围的输入得到符合要求的输出。而智能测试则进一步要求车辆对于更为宽泛和抽象的驾驶场景进行合理的智能化的感知，决策和控制（Intelligence Testing for Autonomous Vehicles A New Approach）。
First of all, they clarified concepts of function testing, performance testing, intelligence testing and other testing concepts. In short, function testing focuses on whether vehicle or its component can obtain the required output for a specific input under given particular conditions (for example, can Lidar give output of more than 3 cloud points for a 1m*1m object located at 200m away). Performance testing focuses on whether vehicle can obtain the required output for a specific range of input under given range of conditions. Intelligence testing further requires vehicle to perform reasonable and intelligent perception, decision making and control strategy for a broader and more abstract driving scenario. (Intelligence Testing for Autonomous Vehicles A New Approach).

%其次，对于智能汽车的智能性测试问题，研究者目前多从人工智能的行为智能角度进行分析，认为如果智能汽车能顺畅驾驶通过给定的交通场景，则具备该类场景的驾驶智能。因此，如何确定需要测试的场景，是当前研究的热点。为此，国际标准化组织提出了功能安全国际标准（ISO 26262）试图指明对于哪些特定场景输入，车辆需要达到什么样的功能输出。为了进一步降低由于系统的预期功能不足（设计不足或性能局限）或可预见的人员误操作导致的不可接受风险造成的危险，国际标准化组织又提出了预期功能安全国际标准（ISO 21448），对于安全功能受外部环境影响的功能（例如AEB自动紧急制动系统、车道保持系统等高级驾驶辅助系统）进行功能测试（Finding Critical Scenarios for Automated Driving Systems A Systematic Literature Review）。然而，对于智能汽车的智能测试而言，需要考虑的驾驶场景千变万化，难以一一胜数。目前难以通过人类专家手工指定测试场景，确定理想的输入输出关系的方法来高效和可靠的测试智能汽车的智能性（Scenario-Based Test Automation for Highly Automated Vehicles A Review and Paving the Way for Systematic Safety Assurance）。

Secondly, for the intelligence testing of intelligent vehicle, currently most of researchers conduct analysis from the view of behavioral intelligence of artificial intelligence. They believe that if an intelligent vehicle drives successfully and smoothly under a given traffic scenario, then it is equipped with driving intelligence of such scenario. As a consequence, it is a hot research topic of how to determine the necessary scenarios for testing. Addressing this need, the International Organization for Standardization proposes an international standard for functional safety (ISO 26262) aiming to point out the functional output should vehicle obtain for a particular scenario and input. Furthermore, in order to reduce the dangers by unacceptable risks due to a lack of system estimated function (inadequate design or performance limitation) or foreseeable human error, the International Organization for Standardization proposes the estimated functional safety standard (ISO 21448) for functional testing of those functions that are affected by external environment, such as automatic emergency braking (AEB) system, lane keeping system and other advanced driving assistance systems. However, for the intelligence testing of intelligent vehicles, the necessary scenarios are numerous. So far, it is hard to efficiently and reliably test the intelligence of vehicle by the method of finding ideal relationship between input and output based on human expert specified testing scenarios. (Scenario-Based Test Automation for Highly Automated Vehicles A Review and Paving the Way for Systematic Safety Assurance).

%再者，考虑到场景构建的难题和当今主流智能系统依靠数据驱动的机器学习模型构建的现状，研究者们提出了多种算法，通过学习naturalistic driving data来实现半自动化或全自动化的场景生成。特别的，研究者高度关注两个问题。其一，如何快速寻找有难度的测试场景，避免在简单的测试场景中浪费时间，无助于提高车辆能力（Accelerated Evaluation of Automated Vehicles Safety in Lane-Change Scenarios Based on Importance Sampling Techniques；Testing Scenario Library Generation for Connected and Automated Vehicles, Part I: Methodology；Testing Scenario Library Generation for Connected and Automated Vehicles, Part II: Case Studies；Intelligent driving intelligence test for autonomous vehicles with naturalistic and adversarial environment）。其二，如何尽可能覆盖所有可能出现的场景，以免智能车辆遇到难以处理的未测试过的场景（A Theoretical Foundation of Intelligence Testing and Its Application for Intelligent Vehicles；Heterogeneous Driver Modeling and Corner Scenarios Sampling for Automated Vehicles Testing）。显然，如何合理平衡这两者具有很高难度，目前尚未找到大家公认的解决方案。特别是所谓Corner Case的寻找对于认知智能汽车的智能局限性很有帮助，值得深入思考（Corner Cases for Visual Perception in Automated Driving: Some Guidance on Detection Approaches）。

Thirdly, considering the difficulty of constructing scenarios and the trend of data-driven machine learning modelling in most of artificial intelligence systems, researchers propose several algorithms to generate scenarios semi-automated or fully automated by learning from naturalistic driving data. Especially, researchers are strongly interested in two problems. One of the problems is how to quickly identify difficult testing scenarios, so as to avoid wasting time in simple testing scenarios which does not help improve vehicle performance. (Accelerated Evaluation of Automated Vehicles Safety in Lane-Change Scenarios Based on Importance Sampling Techniques；Testing Scenario Library Generation for Connected and Automated Vehicles, Part I: Methodology；Testing Scenario Library Generation for Connected and Automated Vehicles, Part II: Case Studies；Intelligent driving intelligence test for autonomous vehicles with naturalistic and adversarial environment). The other problem is how to cover all possible scenarios as much as possible, so as to avoid intelligent vehicle encountering untested scenarios that are hard to deal. (A Theoretical Foundation of Intelligence Testing and Its Application for Intelligent Vehicles；Heterogeneous Driver Modeling and Corner Scenarios Sampling for Automated Vehicles Testing). Apparently, it is difficult to balance those two problems, and it remains unsolved. It is helpful to reveal intelligence limitation of intelligent vehicles by finding corner cases, which is worth to be studied further. (Corner Cases for Visual Perception in Automated Driving: Some Guidance on Detection Approaches)

%最后，由于实地测试需要花费大量的人力财力和时间，因此绝大多数研究者都集中精力进行基于仿真的虚拟测试（Creating a Digital-Vehicle Proving Ground；China 12-Year Quest of Autonomous Vehicular Intelligence The Intelligent Vehicles Future Challenge Program；Verification and Validation of Intelligent Vehicles Objectives and Efforts from China）。Waymore，nVidia等著名公司的尝试表明（Waymo Simulated Driving Behavior in Reconstructed Fatal Crashes within an Autonomous Vehicle Operating Domain；Towards Optimal Strategies for Training Self-Driving Perception Models in Simulation），精心设计的虚拟测试能有效的寻找受试车辆的薄弱环节，并提供有效的解决修改方案。目前，相关研究热点集中于仿真系统如何保证模拟对象的内在行为合理性和外在表现多样性。例如，一些研究者讨论了如何从日常收集的驾驶数据来学会模拟人类驾驶员的行为，以便在仿真系统中正确的复现有人驾驶车辆和无人驾驶车辆的互动（A Systematic Solution of Driving Behavior Modeling and Simulation for Automated Vehicle Studies）。如何通过深度学习模型进行图像变化，从日常驾驶采集到的场景图像变换得到日常难以出现的特殊场景图像就得到了很多研究者的青睐（Driving in the Matrix Can Virtual Worlds Replace Human-Generated Annotations for Real World Tasks；InstaFormer Instance-Aware Image-to-Image Translation with Transformer）。

Lastly, as it is cost and time consuming to conduct real tests, most of researchers focuses on virtual tests based on simulation. (Creating a Digital-Vehicle Proving Ground；China 12-Year Quest of Autonomous Vehicular Intelligence The Intelligent Vehicles Future Challenge Program；Verification and Validation of Intelligent Vehicles Objectives and Efforts from China). Experience of some famous companies such as Waymore and nVidia shows that (Waymo Simulated Driving Behavior in Reconstructed Fatal Crashes within an Autonomous Vehicle Operating Domain；Towards Optimal Strategies for Training Self-Driving Perception Models in Simulation) well-designed virtual tests can effectively identify the weakness of vehicles and provide useful modification solutions. Currently, relevant researches are focused on how to ensure the intrinsic behavioral rationality and external manifestation variety of simulated object in simulation systems. For example, some researchers discuss how to mimic human driver’s behavior by learning from daily collected driving data, so that interactions between manned vehicle and unmanned vehicle can be correctly reproduced in simulation systems. (A Systematic Solution of Driving Behavior Modeling and Simulation for Automated Vehicle Studies). How to transform images by deep learning models, and obtain rarely seen special scene images from transforming daily driving collected scene images has been favored by many researchers. (Driving in the Matrix Can Virtual Worlds Replace Human-Generated Annotations for Real World Tasks；InstaFormer Instance-Aware Image-to-Image Translation with Transformer)

%目前智能汽车的测试尚有很多难点有待解决。可以预见，未来十年是该研究方向进一步飞速发展的重要阶段。

So far there are still many difficulties need to be solved in the field of intelligent vehicle testing. It can be forecasted that the next decade will be an important stage of further rapid development of this field.

==> tabels/introduction/levels.tex <==



\begin{table}[h!]
\centering
\caption{autonomous driving level definition}
\begin{tabular}{ccccccc} \hline
Level & Name                          & Control & Perception & Accidents & Cases \\ \hline
L0    & Artificial            & Driver  & Driver     & Driver               & No               \\
L1    & Assistance                & Driver  & Driver     & Driver               & Part             \\
L2    & Partial      & System  & Driver     & Driver               & Part             \\
L3    & Conditional       & System  & System     & Driver               & Part             \\
L4    & High & System  & System     & System               & Part             \\
L5    & Full       & System  & System     & System               & All        
\\ \hline
\end{tabular}
\label{tab:introduction_levels}
\end{table}

==> tabels/methodology/system_tabel_1.tex <==
\begin{table}[]
\caption{Metrics for Computing Systems for AVs \cite{survey_8}}
\begin{tabular}{cm{6.7cm}}\toprule

\hline

Metric      & Description                                                                                                             \\ \hline
Accuracy    & Usually evaluate the difference between the predicted value and ground truth regarding the precision, recall, and other metrics.                                                                 \\ \hline
Timelines   & Evaluate the inference and processing speed of the computing system to ensure the computation can be finished before the deadline and minimize latency and tail latency, etc.                     \\\hline
Power       & Evaluate the power usage of the computing system and analysis its impact on the energy, mileage, and comfort issues for AVs.                                                                      \\\hline
Cost        & Mainly refer to the financial cost for the computing system toward board deployment.                                                                                                              \\\hline
Reliability & To guarantee the safety of the AVs, the worst-case execution time, interruption or emergency stop capabilities, and fault-tolerant should be considered.                                          \\\hline
Privacy     & To protect the privacy of all the road users including both in-cabin and surrounding users’ private data. Also, the acquisition, storage, and communication privacy should be further considered. \\\hline
Security    & The onboard security can be mainly divided into sensing security, communication security, data security, and control security.        
\\ \hline
\end{tabular}
\label{table:system_table_1}
\end{table}

==> tabels/methodology/system_tabel_2.tex <==
\begin{table*}[]
\caption{Comparative Study for Common Sensor Systems on Autonomous Vehicle.}
\begin{tabular}{cp{5cm}p{5cm}p{5cm}}\toprule
\hline
Sensors    & Advantages                                                                                                                                                                     & Disadvantages                                                                                                                                                                           & Review Studies                                                                                                           \\ \hline
Lidar      & \begin{tabular}[l]{@{}l@{}}1.Support high-resolution 3D point cloud\\ 2.Larger and wider sensing range\\ 3.Accurate object and distance detection\\ 4.Robust to lightning\end{tabular} & \begin{tabular}[p{5cm}]{@{}l@{}}1.High Cost\\ 2.Poor performance to harsh weather\\ 3.A large amount of data stream\end{tabular}                                      & \begin{tabular}[p{5cm}]{@{}l@{}}1.Point Cloud and networks \cite{survey_dynamic_16}\\ 2.SLAM \cite{ system_27, system_28}\\ 3.Sensor design \cite{system_24, system_25}\end{tabular} \\ \hline

Camera     & \begin{tabular}[p{5cm}]{@{}l@{}}1.Cost-effective\\ 2.Visual recognition and texture extraction\end{tabular}                                             & \begin{tabular}[p{5cm}]{@{}l@{}}1.Easily affected by lighting and weather.\end{tabular}                                                       & \begin{tabular}[p{5cm}]{@{}l@{}}1.Perception and networks \cite{survey_dynamic_21, survey_dynamic_5}\\ 2.Fusion \cite{survey_dynamic_15, survey_loca_10}\end{tabular}                         \\ \hline

Radar      & \begin{tabular}[p{5cm}]{@{}l@{}}1.Support extreme long sensing range\\ 2.Resilient to various environmental conditions\end{tabular}                                          & \begin{tabular}[p{5cm}]{@{}l@{}}1.Smaller data size \\ 2.Indistinguishable from static targets\end{tabular} & \begin{tabular}[p{5cm}]{@{}l@{}}1.Detection and perception \cite{survey_hardware_2, survey_dynamic_28}\\ 2.Radar Communication \cite{system_35, system_36, system_37}\end{tabular}           \\ \hline

GPS        & \begin{tabular}[p{5cm}]{@{}l@{}}1.Low cost and stable\\ 2.Non-accumulation error for GPS\end{tabular}                                                                                   & \begin{tabular}[p{5cm}]{@{}l@{}}1.Relative low accuracy for GPS and IMU\\ 2.Slow update frequency \\3. Requiring an unobstructed view\end{tabular}                                      & \begin{tabular}[p{5cm}]{@{}c@{}}1.Localization \& navigation \cite{system_38, system_39}\end{tabular}                                                                   \\ \hline

Ultrasound & \begin{tabular}[p{5cm}]{@{}l@{}}1.Low cost\\ 2.High accuracy for close range\\ 3.Resilient to adverse weather conditions\end{tabular}            & \begin{tabular}[p{5cm}]{@{}l@{}}1.Short-range detection\\ 2.Inapplicable for high speed\end{tabular}  & \begin{tabular}[p{5cm}]{@{}l@{}}1.A systematic review \cite{system_40}\\ 2.All-weather conditions \cite{system_41}\end{tabular} 
\\ \hline
\end{tabular}
\label{table:system_table_2}
\end{table*}
